A HAT Trick: Automatically Verifying Representation Invariants Using Symbolic Finite Automata

Functional programs typically interact with stateful libraries that hide state behind typed abstractions. One particularly important class of applications are data structure implementations that rely on such libraries to provide a level of efficiency and scalability that may be otherwise difficult to achieve. However, because the specifications of the methods provided by these libraries are necessarily general and rarely specialized to the needs of any specific client, any required application-level invariants must often be expressed in terms of additional constraints on the (often) opaque state maintained by the library. In this paper, we consider the specification and verification of such representation invariants using symbolic finite automata (SFA). We show that SFAs can be used to succinctly and precisely capture fine-grained temporal and data-dependent histories of interactions between functional clients and stateful libraries. To facilitate modular and compositional reasoning, we integrate SFAs into a refinement type system to qualify stateful computations resulting from such interactions. The particular instantiation we consider, Hoare Automata Types (HATs), allows us to both specify and automatically type-check the representation invariants of a datatype, even when its implementation depends on stateful library methods that operate over hidden state. We also develop a new bidirectional type checking algorithm that implements an efficient subtyping inclusion check over HATs, enabling their translation into a form amenable for SMT-based automated verification. We present extensive experimental results on an implementation of this algorithm that demonstrates the feasibility of type-checking complex and sophisticated HAT-specified OCaml data structure implementations.

==> Makefile <==
# create pdf

.PHONY: marple marple-diff marple-sm

all: marple

marple: main.tex sections/intro.tex sections/overview.tex sections/lang.tex \
	sections/typing.tex sections/algo.tex sections/evaluation.tex \
	sections/related.tex
	pdflatex -jobname="marple" -shell-escape main
	bibtex marple
	clear
	pdflatex -jobname="marple" -shell-escape main
	clear
	pdflatex -jobname="marple" -shell-escape main

marple-diff: main.tex sections/intro.tex sections/overview.tex sections/lang.tex \
	sections/typing.tex sections/algo.tex sections/evaluation.tex \
	sections/related.tex \
	commands.sty refinementtydef.sty
	pdflatex -jobname="marple-diff" -shell-escape "\def\diffmode{}\input main.tex"
	bibtex marple-diff
	clear
	pdflatex -jobname="marple-diff" -shell-escape "\def\diffmode{}\input main.tex"
	clear
	pdflatex -jobname="marple-diff" -shell-escape "\def\diffmode{}\input main.tex"

marple-sm: main.tex sections/intro.tex sections/overview.tex sections/lang.tex \
	sections/typing.tex sections/algo.tex sections/evaluation.tex \
	sections/related.tex \
	commands.sty refinementtydef.sty
	pdflatex -jobname="marple-sm" -shell-escape "\def\appendixmode{}\input main.tex"
	bibtex marple-sm
	clear
	pdflatex -jobname="marple-sm" -shell-escape "\def\appendixmode{}\input main.tex"
	clear
	pdflatex -jobname="marple-sm" -shell-escape "\def\appendixmode{}\input main.tex"

marple-tech: supplemental.tex tech/outlines.tex tech/semantics.tex \
	tech/basictyping.tex tech/typing.tex tech/srl.tex \
	tech/algo.tex tech/proof.tex tech/evaluation.tex \
	commands.sty refinementtydef.sty
	pdflatex -jobname="marple-tech" -shell-escape supplemental
	bibtex marple-tech
	clear
	pdflatex -jobname="marple-tech" -shell-escape supplemental
	clear
	pdflatex -jobname="marple-tech" -shell-escape supplemental

# create pdf without bibs (fast)
haste:
	pdflatex -shell-escape main

# remove tex objects
clean:
	rm -f *.cb *.cb2 *.log *.aux *.blg *.bbl *.out *~ *.cut sections/*.aux sections/tech/*.aux

# remove objects, including the pdf file
cleanall:
	 rm -f *.cb *.cb2 *.log *.aux *.blg *.bbl *.out *~ *.cut sections/*.aux sections/tech/*.aux *.pdf


==> draft/automata-type.tex <==
\section{Logic}

The events $a$ (or in the context of the automata, we call it characters) are encoded as datatypes, the unary formula $\phi(a)$ over charater $a$ can be used as the ``symbolic alphabets $\Sigma$'' (i.g., the formula appears on the edges, the transition function is a relation over $S \times \Sigma \times S$). For example:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\phi$&(a) :=
match' a with
| Put (i, j) => &$0 \leq n \land i \not= j$&
| Get _ => &$\top$&
\end{minted}

\section{Type Check}

\subsection{Input}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
val[@effect] put: int * int -> unit
val[@effect] get: int -> int

fix (gen: int -> unit) (n: int) =
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let () = gen n' in
    let (m: int) = anynot n in
    () &$\oplus$& perform Put (n, m)
\end{minted}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall$& n, get n; () == ()
&$\forall$& n, (get n == m) &$\impl$& (put (n, m) == ())
&$\forall$& n m, put (n, m); get n == put (n, m); m
&$\forall$& n n' m, &$n \not= n' \impl$& put (n, m); get n' == let x = get n' in put (n, m); x
\end{minted}

It is difficult to reconstruct an automata from a formula, thus consider using the automata directly.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* Ideal type *)
&$\vdash$& gen : &$\nuotxarr{s}{s}{\top}\nuotxarr{n}{int}{0 \leq \vnu } \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}$&
&$\phi$&:
&$\forall i, 0 \leq i < n \impl \neg$& (gen n; get i == i) &$\lor$& (gen n; get i == get i)
&$\forall i, n \leq i \impl$& gen n; get i == get i
(* The type explicit encodes the regular expression *)
&$\vdash$& gen : &$\nuotxarr{n}{int}{0 \leq \vnu } \bcol{s}[.^*]\sarr[R]\tprod{\nuut{unit}{\top}}$&
\end{minted}
However, even this $R$ is kind of hard to get. Consider the expect language of $\mathcal{L}(R)$, that is
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\mathcal{L}(R):$&
[]
[Put (1, 2)]
[Put (1, 3)]
[Put (3, 2); Put (1, 2);]
...
\end{minted}
for a specific $n = 2$:

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (3.2,-5.8) circle (3);
\draw (3.2,-5.8) node {$S_0$};
\draw [black] (25.9,-5.8) circle (3);
\draw (25.9,-5.8) node {$S_1$};
\draw [black] (48.5,-5.8) circle (3);
\draw (48.5,-5.8) node {$S_2$};
\draw [black] (48.5,-5.8) circle (2.4);
\draw [black] (5.829,-4.359) arc (114.6206:65.3794:20.934);
\fill [black] (23.27,-4.36) -- (22.75,-3.57) -- (22.34,-4.48);
\draw (14.55,-1.96) node [above] {\tiny $Put\mbox{ }(2,\mbox{ }\nuut{int}{\vnu\not=2})$};
\draw [black] (28.513,-4.331) arc (115.14642:64.85358:20.444);
\fill [black] (45.89,-4.33) -- (45.38,-3.54) -- (44.95,-4.44);
\draw (37.2,-1.89) node [above] {\tiny $Put\mbox{ }(1,\mbox{ }\nuut{int}{\vnu\not=1})$};
\draw [black] (23.372,-7.409) arc (-62.09298:-117.90702:18.848);
\fill [black] (23.37,-7.41) -- (22.43,-7.34) -- (22.9,-8.23);
\draw [black] (45.886,-7.267) arc (-64.89521:-115.10479:20.473);
\fill [black] (45.89,-7.27) -- (44.95,-7.15) -- (45.37,-8.06);
\end{tikzpicture}
which is not an automata whose shape is depended on the $n$ -- notice that, it is not a symbolic automata whose transition condition can be a formula depends on $n$. It is also not realistic to ask the user to write down this (family of) automata as specification. However, we can get the underapproximation by quotation. Consider the following regular expression
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n}, \nuut{int}{\vnu \not= i})^*$&
\end{minted}
which describe the following automata $A$:

\newcommand{\putnoteq}[1]{\Code{Put}\ (\bcol{i}\nuut{int}{1 \leq \vnu \leq {#1}}, \nuut{int}{\vnu \not= i})}
\newcommand{\getzton}{\Code{Get}\ \nuut{int}{1 \leq \vnu \leq n}}
\newcommand{\mpret}[1]{\I{ret}(#1)}


\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (3.2,-9.1) circle (3);
\draw (3.2,-9.1) node {$S_0$};
\draw [black] (3.2,-9.1) circle (2.4);
\draw [black] (1.877,-6.42) arc (234:-54:2.25);
\draw (3.2,-1.85) node [above] {\tiny $\putnoteq{n}$};
\fill [black] (4.52,-6.42) -- (5.4,-6.07) -- (4.59,-5.48);
\end{tikzpicture}

which is an underapproximation of the behaviours of the generator. Moreover, this automata $A$ satisfies that
\begin{align*}
    \forall \pi, \forall s \in \mathcal{L}(.^*), (\forall x, 0 \leq x \leq n \impl \mpret{s; \pi; \Code{Get\ x}} \not= x \lor \mpret{s; \pi; \Code{Get\ x}} = \mpret{s; \Code{Get\ x}}) \impl \pi \in \mathcal{L}(A)
\end{align*}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (3.2,-9.1) circle (3);
\draw (3.2,-9.1) node {$S_0$};
\draw [black] (3.2,-9.1) circle (2.4);
\draw [black] (22.8,-9.1) circle (3);
\draw (22.8,-9.1) node {$S_1$};
\draw [black] (22.8,-9.1) circle (2.4);
\draw [black] (1.877,-6.42) arc (234:-54:2.25);
\draw (3.2,-1.85) node [above] {\tiny $\putnoteq{n{-}1}$};
\fill [black] (4.52,-6.42) -- (5.4,-6.07) -- (4.59,-5.48);
\draw [black] (5.646,-7.371) arc (119.49889:60.50111:14.935);
\fill [black] (20.35,-7.37) -- (19.9,-6.54) -- (19.41,-7.41);
\draw (13,-4.94) node [above] {\tiny $\epsilon$};
\draw [black] (20.311,-10.766) arc (-61.76239:-118.23761:15.452);
\fill [black] (20.31,-10.77) -- (19.37,-10.7) -- (19.84,-11.59);
\draw (13,-13.11) node [below] {\tiny $\Code{Put}\ (n, \nuut{int}{\vnu \not= n})$};
\end{tikzpicture}

There is a equivalence relation (forward bisimulation?) between these two automata, since
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
...; Put (n, m); Put (n, m') &$\simeq$& ...; Put (n, m')
n != n' &$\impl$& ...; Put (n, m); Put (n', m') &$\simeq$& ...; Put (n', m'); Put (n, m) 
\end{minted}
Thus
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
   &$\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n}, \nuut{int}{\vnu \not= i})^*$&
=  &$(\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n{-}1}, \nuut{int}{\vnu \not= i})\ |\ \Code{Put} (n, \nuut{int}{\vnu \not= n}))^*$&
since &$1 \leq \vnu \leq n{-}1 \land \vnu = n \impl n != n'$& is true
&$\simeq$& &$(\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n{-}1}, \nuut{int}{\vnu \not= i})^*\ |\ (\Code{Put} (n, \nuut{int}{\vnu \not= n})^*)$&
= &$(\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n{-}1}, \nuut{int}{\vnu \not= i})^*\ |\ (\epsilon\ |\ \Code{Put} (n, \nuut{int}{\vnu \not= n})^*\Code{Put} (n, \nuut{int}{\vnu \not= n}))$&
since there are adjacent Put (n, _)
&$\simeq$& &$(\Code{Put} (\bcol{i}\nuut{int}{1 \leq \vnu \leq n{-}1}, \nuut{int}{\vnu \not= i})^*\ |\ (\epsilon\ |\ \Code{Put} (n, \nuut{int}{\vnu \not= n}))$&
\end{minted}

Here we use a special case where all events in the $\mathcal{L}(R)$ is valid -- lead to a state satisfies the user defined specification. Consider another spec:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* Ideal type *)
&$\vdash$& gen : &$\nuotxarr{s}{s}{\top}\nuotxarr{n}{int}{0 \leq \vnu } \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}$&
&$\phi$&:
&$\forall i, 0 \leq i < n \impl \neg$& (gen n; get i == i)
&$\forall i, n \leq i \impl$& gen n; get i == get i
(* The type explicit encodes the regular expression *)
&$\vdash$& gen : &$\nuotxarr{n}{int}{0 \leq \vnu } \bcol{s}[.^*]\sarr[R]\tprod{\nuut{unit}{\top}}$&
\end{minted}
which is hard to encode into a regular expression. Now we try to use the equality relation to filter out the invalid cases.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* Assert Equality *)
... ; Put (n, m); Get n; Assert m &$\simeq$& ... ; Put (n, m)
m != m' &$\impl$& ... ; Put (n, m); Get n; Assert m' &$\simeq$& ... ; Put (n, m); Err
n != n' &$\impl$& ... ; Put (n, m); Get n'; Assert m' &$\simeq$& ... ; Get n'; Assert m'; Put (n, m)
...; Err &$\simeq$& Err
\end{minted}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (3.2,-9.1) circle (3);
\draw (3.2,-9.1) node {$S_0$};
\draw [black] (25,-8.8) circle (3);
\draw (25,-8.8) node {$S_1$};
\draw [black] (45.7,-8.8) circle (3);
\draw (45.7,-8.8) node {$S_2$};
\draw [black] (45.7,-8.8) circle (2.4);
\draw [black] (1.877,-6.42) arc (234:-54:2.25);
\draw (3.2,-1.85) node [above] {\tiny $\Code{Put}(\nuut{int}{\top}, \nuut{int}{\top})$};
\fill [black] (4.52,-6.42) -- (5.4,-6.07) -- (4.59,-5.48);
\draw [black] (6.2,-9.06) -- (22,-8.84);
\fill [black] (22,-8.84) -- (21.19,-8.35) -- (21.21,-9.35);
\draw (14.09,-8.42) node [above] {\tiny $\Code{Get}\ i$};
\draw [black] (4.523,-11.78) arc (54:-234:2.25);
\draw (3.2,-16.35) node [below] {\tiny $\Code{Get}\ \nuut{int}{\top}$};
\fill [black] (1.88,-11.78) -- (1,-12.13) -- (1.81,-12.72);
\draw [black] (28,-8.8) -- (42.7,-8.8);
\fill [black] (42.7,-8.8) -- (41.9,-8.3) -- (41.9,-9.3);
\draw (35.35,-9.3) node [below] {\tiny $\Code{Assert}\ \nuut{int}{\vnu \not= i}$};
\end{tikzpicture}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (3.2,-9.1) circle (3);
\draw (3.2,-9.1) node {$S_0$};
\draw [black] (16.1,-9.1) circle (3);
\draw (16.1,-9.1) node {$S_1$};
\draw [black] (31.5,-9.1) circle (3);
\draw (31.5,-9.1) node {$S_2$};
\draw [black] (49.5,-9.1) circle (3);
\draw (49.5,-9.1) node {$S_3$};
\draw [black] (61.7,-9.1) circle (3);
\draw (61.7,-9.1) node {$S_4$};
\draw [black] (74.4,-9.1) circle (3);
\draw (74.4,-9.1) node {$S_5$};
\draw [black] (1.877,-6.42) arc (234:-54:2.25);
\draw (3.2,-1.85) node [above] {\tiny $\Code{Put}(\nuut{int}{\top}, \nuut{int}{\top})$};
\fill [black] (4.52,-6.42) -- (5.4,-6.07) -- (4.59,-5.48);
\draw [black] (6.2,-9.1) -- (13.1,-9.1);
\fill [black] (13.1,-9.1) -- (12.3,-8.6) -- (12.3,-9.6);
\draw (9.65,-8.6) node [above] {\tiny $\Code{Get}\ i$};
\draw [black] (4.523,-11.78) arc (54:-234:2.25);
\draw (3.2,-16.35) node [below] {\tiny $\Code{Get}\ \nuut{int}{\top}$};
\fill [black] (1.88,-11.78) -- (1,-12.13) -- (1.81,-12.72);
\draw [black] (19.1,-9.1) -- (28.5,-9.1);
\fill [black] (28.5,-9.1) -- (27.7,-8.6) -- (27.7,-9.6);
\draw (23.8,-9.6) node [below] {\tiny $\Code{Assert}\ \nuut{int}{\vnu \not= i}$};
\draw [black] (34.5,-9.1) -- (46.5,-9.1);
\fill [black] (46.5,-9.1) -- (45.7,-8.6) -- (45.7,-9.6);
\draw (40.5,-9.6) node [below] {\tiny $\Code{Put}(n, \nuut{int}{\vnu \not= n})$};
\draw [black] (52.5,-9.1) -- (58.7,-9.1);
\fill [black] (58.7,-9.1) -- (57.9,-8.6) -- (57.9,-9.6);
\draw (55.6,-9.6) node [below] {\tiny $\Code{Get}\ i$};
\draw [black] (64.7,-9.1) -- (71.4,-9.1);
\fill [black] (71.4,-9.1) -- (70.6,-8.6) -- (70.6,-9.6);
\draw (68.05,-9.6) node [below] {\tiny $\Code{Assert}\ \nuut{int}{\vnu \not= i}$};
\end{tikzpicture}


\subsection{Type Check}

\newcommand{\genrty}{\nuotxarr{n}{int}{0 \leq \vnu } \bcol{s}[.^*]\sarr[\putnoteq^*]\tprod{\nuut{unit}{\top}}}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* type judgement *)
&$\mathcal{D} := \Code{Event}$&
&$\vdash$&
fix (gen: int -> unit) (n: int) =
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$: \genrty$&
\end{minted}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TFix *)
&$\mathcal{D} := \Code{Event}$&
gen: &$\genrty$& 
&$\vdash$&
fun (n: int) =
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$: \genrty$&
\end{minted}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLam *)
&$\mathcal{D} := int \times \Code{Event}$&
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&
&$\vdash$&
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$: \bcol{s}[.^*]\sarr[\putnoteq^*]\tprod\nuut{unit}{\top}$&
\end{minted}
Here the domain of the symbolic automata is now a pair, which means the valid events are in the following form:
\begin{align*}
    \Code{(3, Get 3); (4, Put (1, 2)); ...}
\end{align*}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (26,-3.2) circle (2.4);
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\footnotesize $(\nuut{int}{0 \leq \vnu}, .)^*$};
\end{tikzpicture}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TIntroS *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&
&$\vdash$&
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$: [\putnoteq^*]\tprod\nuut{unit}{\top}$&
\end{minted}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (26,-3.2) circle (2.4);
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\footnotesize $(\nuut{int}{0 \leq \vnu}, .)^*$};
\end{tikzpicture}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLet and TOp *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&, b: &$\nuut{bool}{\vnu = (n = 0)}$&
&$\vdash$&
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$: [\putnoteq^*]\tprod\nuut{unit}{\top}$&
\end{minted}

The type of the true branch can be easily inferred as

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (26,-3.2) circle (2.4);
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\footnotesize $(\nuut{int}{0 \leq \vnu}, .)^*$};
\end{tikzpicture}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLet and TOp *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&, b: &$\nuut{bool}{\vnu = (n = 0) \land \textcolor{red}{\vnu}}$&
&$\vdash$&
    ()
&$\typeinfer [\epsilon]\tprod\nuut{unit}{\top}$&
\end{minted}
notice that the condition of this branch, it constraints the first element of the pair, such that
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (26,-3.2) circle (2.4);
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\tiny $(\nuut{int}{0 \leq \vnu \land 0 = \vnu}, .)^*$};
\end{tikzpicture}

The type of the false branch can inferred as

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (26,-3.2) circle (2.4);
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\footnotesize $(\nuut{int}{0 \leq \vnu}, .)^*$};
\end{tikzpicture}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLet and TOp *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&, b: &$\nuut{bool}{\vnu = (n = 0) \land \neg \vnu}$&, n': &$\nuut{int}{\vnu = n - 1}$&
&$\vdash$&
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$\typeinfer ?$&
\end{minted}

In order to apply $\Code{gen}$, we check the inclusion relation of the current automata $A$ and the argument type $[.^*]$, that is $\mathcal{L}(.^*) \subseteq \mathcal{L}(A)$, which is decidable. Since $A$ is just $.^*$, thus easily know it is true. Then we can append the events of the recursive function call:

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (26,-3.2) circle (3);
\draw (26,-3.2) node {$S_1$};
\draw [black] (3.2,-3.2) circle (3);
\draw (3.2,-3.2) node {$S_0$};
\draw [black] (59.6,-3.2) circle (3);
\draw (59.6,-3.2) node {$S_2$};
\draw [black] (59.6,-3.2) circle (2.4);
\draw [black] (6.2,-3.2) -- (23,-3.2);
\fill [black] (23,-3.2) -- (22.2,-2.7) -- (22.2,-3.7);
\draw (14.6,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n}, .)^*$};
\draw [black] (29,-3.2) -- (56.6,-3.2);
\fill [black] (56.6,-3.2) -- (55.8,-2.7) -- (55.8,-3.7);
\draw (42.8,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n'}, \Code{Put}\ (\bcol{i}\nuut{0 \leq \vnu \leq n'}, ...))^*$};
\end{tikzpicture}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLet and TOp *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&, b: &$\nuut{bool}{\vnu = (n = 0) \land \neg \vnu}$&, n': &$\nuut{int}{\vnu = n - 1}$&,
m: &$\nuut{int}{\vnu \not= n}$&
&$\vdash$&
    perform Put (n, m')
&$\typeinfer A' \times \nuut{unit}{\top}$&
\end{minted}

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23.4,-3.2) circle (3);
\draw (23.4,-3.2) node {$S_1$};
\draw [black] (3.1,-3.2) circle (3);
\draw (3.1,-3.2) node {$S_0$};
\draw [black] (54.2,-3.2) circle (3);
\draw (54.2,-3.2) node {$S_2$};
\draw [black] (86.4,-3.2) circle (3);
\draw (86.4,-3.2) node {$S_3$};
\draw [black] (86.4,-3.2) circle (2.4);
\draw [black] (6.1,-3.2) -- (20.4,-3.2);
\fill [black] (20.4,-3.2) -- (19.6,-2.7) -- (19.6,-3.7);
\draw (13.25,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n}, .)^*$};
\draw [black] (26.4,-3.2) -- (51.2,-3.2);
\fill [black] (51.2,-3.2) -- (50.4,-2.7) -- (50.4,-3.7);
\draw (38.8,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n'}, \Code{Put}\ (\bcol{i}\nuut{0 \leq \vnu \leq n'}, ...))^*$};
\draw [black] (57.2,-3.2) -- (83.4,-3.2);
\fill [black] (83.4,-3.2) -- (82.6,-2.7) -- (82.6,-3.7);
\draw (70.3,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n}, \Code{Put}\ (n, \nuut{int}{\vnu \not= n}))$};
\end{tikzpicture}

now exists the bindings in the type context.

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23.4,-3.2) circle (3);
\draw (23.4,-3.2) node {$S_1$};
\draw [black] (3.1,-3.2) circle (3);
\draw (3.1,-3.2) node {$S_0$};
\draw [black] (54.2,-3.2) circle (3);
\draw (54.2,-3.2) node {$S_2$};
\draw [black] (86.4,-3.2) circle (3);
\draw (86.4,-3.2) node {$S_3$};
\draw [black] (86.4,-3.2) circle (2.4);
\draw [black] (6.1,-3.2) -- (20.4,-3.2);
\fill [black] (20.4,-3.2) -- (19.6,-2.7) -- (19.6,-3.7);
\draw (13.25,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n \land 0 < \vnu}, .)^*$};
\draw [black] (26.4,-3.2) -- (51.2,-3.2);
\fill [black] (51.2,-3.2) -- (50.4,-2.7) -- (50.4,-3.7);
\draw (38.8,-3.7) node [below] {\tiny $(n {-} 1, \Code{Put}\ (\bcol{i}\nuut{0 \leq \vnu \leq n {-} 1}, ...))^*$};
\draw [black] (57.2,-3.2) -- (83.4,-3.2);
\fill [black] (83.4,-3.2) -- (82.6,-2.7) -- (82.6,-3.7);
\draw (70.3,-3.7) node [below] {\tiny $(n, \Code{Put}\ (n, \nuut{int}{\vnu \not= n}))$};
\end{tikzpicture}

Now merge the automata. Here is a simple case where the true branches has the same return value, thus we can merge the automata directly:

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23.4,-3.2) circle (3);
\draw (23.4,-3.2) node {$S_1$};
\draw [black] (3.1,-3.2) circle (3);
\draw (3.1,-3.2) node {$S_0$};
\draw [black] (54.2,-3.2) circle (3);
\draw (54.2,-3.2) node {$S_2$};
\draw [black] (76.4,-3.2) circle (3);
\draw (76.4,-3.2) node {$S_3$};
\draw [black] (76.4,-3.2) circle (2.4);
\draw [black] (23.4,-13.3) circle (3);
\draw (23.4,-13.3) node {$S_1'$};
\draw [black] (23.4,-13.3) circle (2.4);
\draw [black] (6.1,-3.2) -- (20.4,-3.2);
\fill [black] (20.4,-3.2) -- (19.6,-2.7) -- (19.6,-3.7);
\draw (13.25,-3.7) node [below] {\tiny $(\nuut{int}{\vnu = n \land 0 \not= \vnu}, .)^*$};
\draw [black] (26.4,-3.2) -- (51.2,-3.2);
\fill [black] (51.2,-3.2) -- (50.4,-2.7) -- (50.4,-3.7);
\draw (38.8,-3.7) node [below] {\tiny $(n {-} 1, \Code{Put}\ (\bcol{i}\nuut{0 \leq \vnu \leq n {-} 1}, ...))^*$};
\draw [black] (57.2,-3.2) -- (73.4,-3.2);
\fill [black] (73.4,-3.2) -- (72.6,-2.7) -- (72.6,-3.7);
\draw (65.3,-3.7) node [below] {\tiny $(n, \Code{Put}\ (n, \nuut{int}{\vnu \not= n}))$};
\draw [black] (5.79,-4.54) -- (20.71,-11.96);
\fill [black] (20.71,-11.96) -- (20.22,-11.16) -- (19.78,-12.05);
\draw (12.32,-8.75) node [below] {\tiny $(\nuut{int}{\vnu = n \land 0 = \vnu}, .)^*$};
\end{tikzpicture}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TMerge *)
&$\mathcal{D} := int \times \Code{Event}$&, A : (* figure above *)
gen: &$\genrty$&,
n: &$\nuot{int}{0 \leq \vnu}$&
&$\vdash$&
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let (_: unit) = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m')
&$\typeinfer A\tprod\nuut{unit}{\top}$&
\end{minted}

This automata is not exactly consistent with the return type of the $\Code{gen}$ where the domain is contains an auxiliary filed $n$ which is used to label the control flows in the automata. Now we drop it:

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23.4,-3.2) circle (3);
\draw (23.4,-3.2) node {$S_1$};
\draw [black] (3.1,-3.2) circle (3);
\draw (3.1,-3.2) node {$S_0$};
\draw [black] (54.2,-3.2) circle (3);
\draw (54.2,-3.2) node {$S_2$};
\draw [black] (76.4,-3.2) circle (3);
\draw (76.4,-3.2) node {$S_3$};
\draw [black] (76.4,-3.2) circle (2.4);
\draw [black] (23.4,-13.3) circle (3);
\draw (23.4,-13.3) node {$S_1'$};
\draw [black] (23.4,-13.3) circle (2.4);
\draw [black] (6.1,-3.2) -- (20.4,-3.2);
\fill [black] (20.4,-3.2) -- (19.6,-2.7) -- (19.6,-3.7);
\draw (13.25,-3.7) node [below] {\tiny $.^*$};
\draw [black] (26.4,-3.2) -- (51.2,-3.2);
\fill [black] (51.2,-3.2) -- (50.4,-2.7) -- (50.4,-3.7);
\draw (38.8,-3.7) node [below] {\tiny $\Code{Put}\ (\bcol{i}\nuut{0 \leq \vnu \leq n {-} 1}, \nuut{int}{\vnu 
\not= i})^*$};
\draw [black] (57.2,-3.2) -- (73.4,-3.2);
\fill [black] (73.4,-3.2) -- (72.6,-2.7) -- (72.6,-3.7);
\draw (65.3,-3.7) node [below] {\tiny $\Code{Put}\ (n, \nuut{int}{\vnu \not= n})$};
\draw [black] (5.79,-4.54) -- (20.71,-11.96);
\fill [black] (20.71,-11.96) -- (20.22,-11.16) -- (19.78,-12.05);
\draw (12.32,-8.75) node [below] {\tiny $.^*$};
\end{tikzpicture}

Now we prove the automata above can include the user provided 

\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23.4,-3.2) circle (3);
\draw (23.4,-3.2) node {$S_1$};
\draw [black] (3.1,-3.2) circle (3);
\draw (3.1,-3.2) node {$S_0$};
\draw [black] (57.2,-3.2) circle (3);
\draw (57.2,-3.2) node {$S_2$};
\draw [black] (57.2,-3.2) circle (2.4);
\draw [black] (6.1,-3.2) -- (20.4,-3.2);
\fill [black] (20.4,-3.2) -- (19.6,-2.7) -- (19.6,-3.7);
\draw (13.25,-3.7) node [below] {\tiny $.^*$};
\draw [black] (26.4,-3.2) -- (54.2,-3.2);
\fill [black] (54.2,-3.2) -- (53.4,-2.7) -- (53.4,-3.7);
\draw (40.3,-3.7) node [below] {\tiny $\putnoteq^*$};
\end{tikzpicture}

==> draft/dttrace.tex <==
\section{Novelty}

In our discussion on Wednesday, we notice that we can reuse ``Poirot'' to solve track the trace of the effectful program, simply shifting from constraint a value $\vnu$ with type $\nuut{b}{\phi}$ to a type $\nuut{b \times tr}{\phi}$ where $tr$ is a built-in type indicating the traces that is a list of events, where event is a effectful operator call. The new type system needs slight changes, but following the same idea. For example, as I showed this Wednesday, when we eliminate the bindings in the type context, the new exists function not only existing the hidden variables (i.g., the left-hand-side of the let binding), but also concatenate the trace of the hidden variables to the trace of the body expression of the let binding.

It somehow solves the problem, but not perfectly. Although we can track the trace of the expression, say $\vnu.h{:}tr$, by treating the traces as a list (or a steam), this abstraction is not precise and the logic of the qualifier is not rich enough for the users to express the desired protocol. Consider the following variant of the put/get example, which has an additional operator ``clear''.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=240pt]{image/recursive-put-get.drawio.png}
    \caption{Protocol of the put/get example with ``clear'' operator.}
    \label{fig:recursive-put-get}
\end{figure}

As we shown in \autoref{fig:recursive-put-get}, the protocol assume there is a hidden cell that has two states: uninitialized or storing some integer. Then, the ``set'' operation save a integer to the cell; the ``clear'' operation reset the cell to uninitialized; the ``getI'' operator read the cell while the ``getU'' always returns some default value (i.g., $0$). Notice that, although there are two arrows ``getI'' and ``getU'' in \autoref{fig:recursive-put-get}, there is a only single effectful operator ``get'' whose behaviours dependent on the current state.

It is hard for the users to express a property only using the plain list data type in ``Poirot''. For example, a safety (overapproximate) property ``all traces generated by the generator $\S{gen}$ should be consistent the protocol above'' needs to say there is no adjacent ``set'' or ``clear''. The user needs to 1) define the meaning of ``adjacent'' 2) distinguish the ``set'' event and ``clear'' event. On the other hand, the coverage (underapproximate) property can be even harder. For example, the user believes that the it is enough to perform only one ``get'' operation when the cell is uninitialized since it just returns the default value, on the other hand, the user want to perform arbitrary many ``get'' when the cell is initialized. In this case, the ``adjacent'' doesn't work here, because if we know the previous event is a ``get'' event returning value $0$, we cannot decide if we should perform another ``get'' operation. The only solution is to define a new method predicate to record the state of all prefixes of the traces.

These additional user efforts over the method predicate are caused by the fact that the expressive power of the plain list data type in ``Poirot'' is too weak to capture the ``stateful natural'' of the trace. In the traditionally refinement type system, the list/stream data type is a ``base type'' whose details are hidden from the qualifiers. More precisely, the constructor of the list/stream is hidden, which lead there is no way to naturally describe the relation between new adding event and previous trace. Moreover, when there are multiple effect operators (e.g., $put$, $get$, $clear$), the event is equal to the sum (type) of these operations. There is no natural way in ``Poirot'' to describe the relation of two events who has the sum type since the sum type is also a base type.

I am inspired the recursive type which has type level fixpoint functions and describe the algebraic data type more precisely. There is also a correspondence between the recursive type (with an co-inductive interpretation) and the process following the some protocols \cite{TAPL}. I am also inspired by the defunctionalization, which is a replacement of the closure conversion, that convert the functions (e.g., perform an effectful operation) calls into datatypes. The defunctionalization realizes a data type of the continuation\cite{defunc-at-work}, which is is a better data type form for the traces we consider. Then, I introduce the following definition:
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
type b' uninit = Clear of 'a init
            | GetU of b' uninit
and 'a init = Set of int * b' uninit
            | GetI of 'a init 
and 'a tr = Uninit of b' uninit | Init of 'a init
\end{minted}
The type $tr$ (I will explain the $'a$ later) is the sum type of the mutual recursive types $uninit$ and $init$ that indicates two states. On the other hand, the definition of these two types exactly encode the protocol shown in \autoref{fig:recursive-put-get}. Notable, these recursive types are interpreted as an inductive (lfp) definitions. For example, the $\Code{Set}$ constructor means that ``a trace ends up with a state $\Code{init}$ can be constructed from a trace ends up with state $\Code{uninit}$ and an event of setting an interger''. Alternatively, we can also have an co-inductive (gfp) style definition by swapping the constructor $\Code{Set}$ and $\Code{Clear}$ :
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
type b' uninit = Set of int * 'a init
            | GetU of b' uninit
and 'a init = Clear of b' uninit
            | GetI of 'a init 
and 'a tr = Uninit of b' uninit | Init of 'a init
\end{minted}
Now the definition of $\Code{Set}$ means that ``a trace ends up with a state $\Code{uninit}$ can be destructed as a trace ends up with state $\Code{init}$ and an event of setting an interger''. Precisely, The type above is defined as the following type level fixpoint function (with sum type $+$ and record type $\{...:...\}$):
\begin{align*}
    tr ::= \mu\alpha. &\Code{match}~\alpha~\Code{ with} \\
                      &|~\Code{Left}~\Code{uninit} -> \{\Code{GetU}:\Code{uninit}\} + \{\Code{Clear}:\Code{uninit}\} \\
                      &|~\Code{Right}~\Code{init} -> \{\Code{Set}:\Code{int}\times\Code{init}\} + \{\Code{GetI}:\Code{init}\}
\end{align*}
\ZZ{One idea: the overapproximate type use induction definition and the underapproximate type use the co-induction definition.}

\paragraph{Why we define the trace in the form above} The reason is simple, that is to enable to refinement type and the qualifiers the trace (precisely, the prefix of the trace) and the new adding event via the equation. Consider the following example where we instantiate the type variable $'a$ as bool which indicate the sign of the value stored in the hidden cell; on the other hand, the initialized cell saved nothing thus the type variable $'b$ is instantiated as unit (we omit it for concision).
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
type uninit = Clear of &$\nuot{bool}{\top}$& init
                | GetU of uninit
and &$x{:}\nuot{bool}{\top}$& init = Set of &$\nuot{int}{x \iff \vnu \geq 0}$& * uninit
                | GetI of &$\nuot{bool}{x \iff \vnu}$& init 
and &$x{:}\nuot{bool}{\top}$& tr = Uninit of uninit | Init of &$\nuot{bool}{x \iff \vnu}$& init
\end{minted}
The meaning of this type is obvious. For example, the first constructor \Code{Clear} means that ``a trace ends up with an uninitialized hidden cell can be constructed from a trace ends up with a hidden cell saving integer with positive or negative sign''. On the other hand, the constructor \Code{Set} mean that ``a trace ends up with an initialized hidden cell saving integer with sign $x{:}bool$ can be constructed from a trace ends up with an uninitialized hidden cell and an integer who is greater equal than $0$ iff $x$ is true''. Here is another interesting example, as we mentioned above, try to find trace with arbitrary many adjacent \Code{GetI} but no adjacent \Code{GetU}.
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
type &$x{:}\nuot{nat}{\top}$& uninit = Clear of &$\nuot{nat}{\vnu = 0}$& init
                | GetU of &$\nuot{nat}{\vnu = x + 1}$& uninit
and &$x{:}\nuot{nat}{\top}$& init = Set of &$\nuot{nat}{\top}$& * &$\nuot{nat}{\vnu = 0}$& uninit
                | GetI of &$\nuot{nat}{\vnu = x + 1}$& init 
and tr = Uninit of &$\nuot{nat}{\vnu \leq 1}$& uninit | Init of &$\nuot{nat}{\top}$& init
\end{minted}
Here we assume both \Code{init} and \Code{uninit} is bound with a natural number that counts of the adjacent \Code{get} preformed. The operation \Code{Set} and \Code{Clear} will reset the counter to zero and operation \Code{GetU} and \Code{GetI} will increase the counter by $1$. The constructor \Code{Uninit} on the last line constraints that a valid trace that ends up with an uninitialized state can only has counter that is less equal than $1$, which express the protocol we want. We can imagine that the type above is the subtype of the following type
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
...
and tr = Uninit of &$\nuot{nat}{\vnu \leq 2}$& uninit | Init of &$\nuot{nat}{\top}$& init
\end{minted}
which requires there are at most two adjacent ``get'' if the state is uninitialized.

Notable, there are two things to be clarified:
\begin{enumerate}
    \item The type of $'a$ and $'b$ is independent with the argument type of the effectful operators. For example, although the ``set'' operation takes integer as input, the state can be parameterized as bool type or nat type. This fact means that the type (specification of the use defined protocol and states) independent from the implementation details (the program we want to type check). Moreover, the granularity of the abstraction of the trace (e.g., using bool type or nat type) can be controlled by the user. 
    \item The type above
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
        type &$\tau$& NAME = NAME of &$\tau$& NANE | ...
\end{minted}
is a new kind of refinement type, same as the base refinement type and function refinement type. Thus the syntax of the refinement type is
\begin{align*}
    \tau ::= \ &\nuot{t}{\phi} \\
               &|\ x{:}\tau{\shortrightarrow}\tau \\
               &|\ \Code{type}\ \tau\ x\ =\ \overline{ x\ \Code{of}\ \overline{ \tau }}
\end{align*}
Indeed, a type above is kind of too complicate for the user to write it down. I am considering somehow to simplify it, since the ``shape'' of the mutual recursive definition doesn't change, the user just need to provide the qualifiers distributed in the definition, which can be reduced to some special function types (notated as $\Rightarrow$) in the counter example:
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
Clear: &$x{:}\nuot{nat}{\top}{\Rightarrow}\nuot{nat}{\vnu = 0}$&
GetU: &$x{:}\nuot{nat}{\top}{\Rightarrow}\nuot{nat}{\vnu = x + 1}$&
Set: &$x{:}\nuot{nat}{\top}{\Rightarrow}\nuot{nat}{\top}\times\nuot{nat}{\vnu = 0}$&
GetI: &$x{:}\nuot{nat}{\top}{\Rightarrow}\nuot{nat}{\vnu = x + 1}$&
Uninit: &$unit{\Rightarrow}\nuot{nat}{\vnu \leq 1}$&
Init: &$unit{\Rightarrow}\nuot{nat}{\top}$&
\end{minted}
Here the user will not change the specification of $\Code{Clear}$ or $\Code{GetI}$ which simply counts the number of preformed ``get''. The user (and during the type checking, the type of traces) may change the qualifiers of the states, that is \Code{Uninit} and \Code{Init}.
\end{enumerate}

==> draft/language.tex <==
\section{Language}
\label{sec:lang}
%\subsection{Syntax}

\begin{figure}[t!]
{\small
    \begin{alignat*}{2}
    \text{\textbf{Variables }}& \quad &\quad& x, f, u, X, ... \\
    \text{\textbf{Operations }}& \quad &\quad& op \\
    \text{\textbf{Constants }}& \quad &c ::= \quad & () ~|~ \mathbb{B} ~|~ \mathbb{N} \\
    \text{\textbf{Primitive Operations}}& \quad & primop ::= \quad &{+} ~|~ {==} ~|~ {<} \\
    \text{\textbf{Values }}& \quad  & v ::= \quad & c ~|~ x ~|~ \zlam{x}{t}{e} ~|~ v\#op ~|~ h \\
    % \text{\textbf{Handlers }}& \quad  & h ::= \quad & \handler{v}{\overline{ op_i \to v_i }} \\
    \text{\textbf{Expression (Computation)}}& \quad & e ::=\quad & v
    ~|~ \zlet{x}{e}{e}
    ~|~ \zlet{x}{primop\ \overline{v}}{e}
    ~|~ \zlet{x}{v\ v}{e}\\
    &\quad&\quad& |~ \perform{x}{op}{v}{e} ~|~ \handle{e}{v}{\overline{ op_i \to v_i }}\\
    % &\quad&\quad&
    % ~|~ \zlet{x}{d\ \overline{v}}{e}
    % \ite{v}{e}{e}
    % ~|~ \match{x}{d\ \overline{y}}{e} \\
    \text{\textbf{Base Types}}& \quad & b  ::= \quad &  unit ~|~ bool ~|~ nat \\
    \text{\textbf{Basic Types}}& \quad & t  ::= \quad & b ~|~ t \sarr t ~|~ t \sarr^{\kappa} t  \\
    \text{\textbf{Propositions}}& \quad & \phi ::= ... \\
    % \text{\textbf{Pure Refinement Types}}& \quad &\tau  ::= \quad &  \nuut{\textit{b}}{\phi}~|~ \nuot{\textit{b}}{\phi} ~|~  x{:}\tau{\shortrightarrow}\tau \\
    \text{\textbf{(Effectful) Refinement Types}}& \quad &\tau ::= \quad &  \nuut{\textit{b}}{\phi} \otttail{\psi} ~|~ \nuott{\psi}{\textit{b}}{\phi} ~|~  (\mu_x, x){:}\tau{\shortrightarrow}\tau ~|~  \tau \sarr^{\kappa} \tau  \\
    \text{\textbf{(Effectful) Type Contexts}}& \quad &\Gamma ::= \quad & \emptyset ~|~ \Gamma, (\mu_x, x){:}\tau ~|~ \Gamma, \hat{(\mu_x, x)}{:}\tau
  \end{alignat*}
}
    \caption{\langname{} syntax.}\label{fig:syntax}
\end{figure}
\begin{enumerate}
    \item $t \sarr t$ is the function type, $t \sarr^{kappa} t$ is the delimited continuation type.
    \item the type $\nuott{\psi}{\textit{b}}{\phi}$ indicates that ``a computation may reduce to a value $\nu$ with along an event trace $\mu$ such that $\psi(\mu) \land \phi(\mu, \nu)$''. For example,
    \begin{align*}
        &\vdash 3 : \nuott{\mu = \emptyset}{nat}{\nu = 3} \\
        &\vdash Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)} \\
        &\vdash \lambda x. Get\ x: \nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu  }{unit}{\top} \sarr \nuott{\mu = Get\ \nuot{unit}{\top}}{nat}{last(\mu_a, Put)}
    \end{align*}
    which indicates that the trace before we perform $Get$ should contain at least $1$ $Put$ event, and we exactly returns the value consistent with the argument of that $Put$. Additionally, $Get$ is an operation which indicates that the application (perform the $Get$) will generate a new event $Get$; the $\mu = \emptyset$ in the return type indicate the the handler of $Get$ should not perform new effects. Notice that, only the effect function type can generate new event, the normal function type is pure -- although it may require event traces in the argument type and its return type will describe the generated effect events of the function body (e.g., $\lambda x. Get\ x$).
\end{enumerate}

\begin{figure}[!t]
{\small
{\normalsize
\begin{flalign*}
 &\text{\textbf{Typing }} & % \fbox{$\Gamma \vdashover \tau$} \text{ and }
 \fbox{$\Gamma \vdash \tau$}
\end{flalign*}
}
\\ \
\begin{prooftree}
\hypo{
}
\infer1[\textsc{TConst}]{
\Gamma \vdash c : \nuott{\mu = \emptyset}{ty(c)}{\nu = c}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{ \Gamma(\_, x) = \tau
}
\infer1[\textsc{TVar}]{
\Gamma \vdash x : \nuott{\mu = \emptyset}{\eraserf{\tau}}{\nu = x}
}
\end{prooftree}
\\ \ \\ \ \\
\begin{prooftree}
\hypo{
\parbox{110mm}{\center
$\hat{\Gamma}, \hat{(\mu_a, a)}{:}\nuott{\psi_a}{A}{\phi_a} \vdash e : \tau$
}
}
\infer1[\textsc{TLam}]{
\Gamma \vdash \zlam{a}{A}{e}\ : (\mu_a, a){:}\nuott{\psi_a}{A}{\phi_a} \sarr \tau
}
\end{prooftree}
\\ \ \\ \ \\
\begin{prooftree}
\hypo{
\parbox{110mm}{\center
$\Gamma \vdash v : (\mu_a, a){:}\nuott{\psi_a}{A}{\phi_a} \sarr \nuott{\psi_b}{B}{\phi_b}$ \quad
$\Gamma \vdash v_a : \nuott{\mu = \emptyset}{A}{\phi_{v_a}}$ \quad
$\Gamma \vdash \nuott{\listconcat \Gamma}{A}{\phi_{v_a}} <: \nuott{\psi_a}{A}{\phi_a}$ \quad
$\Gamma, (\mu_x, x){:}\nuott{\psi_b[a\mapsto v_a]}{B}{\phi_b[a\mapsto v_a]} \vdash e : \tau$
}
}
\infer1[\textsc{TApp}]{
\Gamma \vdash \zlet{x}{v\ v_a}{e}\ : \tau
}
\end{prooftree}
\\ \ \\ \ \\
\begin{prooftree}
\hypo{
\parbox{110mm}{\center
$\Gamma(op) = a{:}\nuott{\psi_a}{A}{\phi_a} \sarr \nuott{\psi_b}{B}{\phi_b}$ \quad $\Gamma \vdash v : \nuott{\mu = \emptyset}{A}{\phi_{v_a}}$ \quad 
$\Gamma \vdash \nuott{\listconcat \Gamma}{A}{\phi_{v_a}} <: \nuott{\psi_a}{A}{\phi_a}$ \quad
$\Gamma, (\mu_x, x){:}(\nuott{ op\ \nuot{A}{\phi_a} ;\psi_b [a\mapsto v]}{B}{\phi_b [a\mapsto v]}) \vdash e : \nuott{\psi}{C}{\phi}$
}
}
\infer1[\textsc{TPerform}]{
\Gamma \vdash \perform{x}{op}{v}{e}\ : \nuott{op\ \nuot{A}{\phi_a} ;\psi_b [a\mapsto v];\psi}{C}{\phi}
}
\end{prooftree}
\\ \ \\ \ \\
\begin{prooftree}
\hypo{
\parbox{110mm}{\center
$\hat{\Gamma}, op_i : (\mu_a,a){:}\tau_a \sarr \nuott{\psi_b}{B}{\phi_b} \vdash e : \tau_e$ \quad $\hat{\Gamma}\vdash v_i : ((\mu_a,a){:}\tau_a \sarr (\nuott{\psi_b}{B}{\phi_b} \sarr^{\kappa} \tau) \sarr \tau)$ \quad
$\Gamma\vdash v : \tau_e \sarr \tau$ \quad
}
}
\infer1[\textsc{THandle}]{
\Gamma \vdash \handle{e}{v}{\overline{ op_i \to v_i }}\ : \tau
}
\end{prooftree}
}
\caption{typing rules}\label{fig:typing-rules}
\end{figure}

\begin{example}Consider

\begin{minted}[fontsize = \footnotesize,xleftmargin = 10pt,escapeinside=<>]{ocaml}
let x = perfrom Put 3 in
let y = perfrom Get () in
y
\end{minted}
We have
\end{example}

\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &\vdash \perform{x}{Put}{3}{...} : ...
\end{align*}

\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr^{E} \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &\vdash 3 : \nuott{\mu = \emptyset}{nat}{\nu = 3}
\end{align*}

Subtyping:
\begin{align*}
    &\vdash \nuott{\mu = \emptyset}{nat}{\nu = 3} <: \nuott{\top}{nat}{\top}
\end{align*}

\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr^{E} \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &(\mu_x,x){:}\nuott{\mu = Put\ \nuot{nat}{\nu = 3} }{unit}{\top} \vdash \perform{x}{Get}{()}{y} : ...
\end{align*}

\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr^{E} \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &(\mu_x,x){:}\nuott{\mu = Put\ \nuot{nat}{\nu = 3} }{unit}{\top} \vdash () :\nuott{\emptyset }{unit}{\top}
\end{align*}

Subtyping:
\begin{align*}
    & \vdash \nuott{\mu = Put\ \nuot{nat}{\nu = 3} }{unit}{\top} <: \nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu  }{unit}{\top}
\end{align*}

\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr^{E} \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &(\mu_x,x){:}\nuott{\mu = Put\ \nuot{nat}{\nu = 3} }{unit}{\top}, (\mu_y,y){:}\nuott{\mu = Get\ \nuot{unit}{\top}}{nat}{\nu = 3}\\
    & \vdash y : \nuott{\emptyset}{nat}{\nu = y}
\end{align*}

Pop the bindings from the type context.
\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr^{E} \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    &(\mu_x,x){:}\nuott{\mu = Put\ \nuot{nat}{\nu = 3} }{unit}{\top}\\
    & \vdash \perform{x}{Get}{()}{y} : \nuott{\mu = Get\ \nuot{unit}{\top}}{nat}{\exists y, y = 3 \land \nu = y}
\end{align*}

Pop the bindings from the type context.
\begin{align*}
    &Get: (\mu_a,\_){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr \nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)}\\
    &Put{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu = \emptyset}{unit}{\top}\\
    & \vdash \perform{x}{Put}{3}{\perform{x}{Get}{()}{y}} : \\
    &\nuott{\mu = Put\ \nuot{nat}{\nu = 3};Get\ \nuot{unit}{\top}}{nat}{\exists y, y = 3 \land \nu = y}
\end{align*}

\begin{minted}[fontsize = \footnotesize,xleftmargin = 10pt,escapeinside=<>]{ocaml}
handle ... with {
  fun (x:nat) -> (fun (s: nat) -> (s, x));
  Put : fun (a:nat) (k: cont (unit, nat -> nat * nat)) -> (fun (_: nat) -> k () a);
  Get : fun (a:unit) (k: cont (nat, nat -> nat * nat)) -> (fun (s: nat) -> k s s);
}
\end{minted}

\begin{align*}
    &\emptyset \vdash \zlam{x}{nat}{\zlam{s}{nat}{(s, x)}} : \\
    &x{:}\nuott{\top}{nat}{\top} \sarr s{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu=\emptyset}{nat\times nat}{\nu.1 = s \land \nu.2 = x}
\end{align*}

Put:
\begin{align*}
    &\emptyset \vdash \zlam{a}{unit}{\zlam{k}{(nat \sarr^{\kappa} nat \times nat)}{\zlam{s}{nat}{k\ ()\ a}}} : \\
    &(\mu_a,a){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr \\
    &(\nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)} \sarr^{\kappa} s{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu=\emptyset}{nat\times nat}{\nu.1 = s \land \nu.2 = a}) \sarr \\
    &\nuott{\mu=\emptyset}{nat\times nat}{\nu.1 = s \land \nu.2 = a}
\end{align*}

Get:
\begin{align*}
    &\emptyset \vdash \zlam{a}{nat}{\zlam{k}{(unit \sarr^{\kappa} nat \times nat)}{\zlam{s}{nat}{k\ s\ s}}} : \\
    &(\mu_a,a){:}\nuott{ \exists p\ \tau, (p; Put\ \tau)  \sqsubseteq \mu }{unit}{\top} \sarr \\
    &(\nuott{\mu = \emptyset}{nat}{last(\mu_a, Put)} \sarr^{\kappa} s{:}\nuott{\top}{nat}{\top} \sarr \nuott{\mu=\emptyset}{nat\times nat}{\nu.1 = s \land \nu.2 = a}) \sarr \\
    &\nuott{\mu=\emptyset}{nat\times nat}{\nu.1 = s \land \nu.2 = a}
\end{align*}


==> draft/meta-theory.tex <==
\section{Meta Theory}

Now we introduce the formalization and the corresponding soundness and completeness theorems for the ``stateful property-based testing'' and corresponding generator.

From the user perspective, the test generator actually generate traces in the labeled transition system (LTS) from the initial states to the states specified the users.

\begin{definition}[Labeled transition system] A labeled transition system (LTS) is a tuple $\mathcal{L} = (S, Act, \sarr)$ such that
\begin{enumerate}
    \item $S$ is a set of states (the state space).
    \item $Act \cup \{\epsilon\}$ is a set of actions (Act is the label space), where $\epsilon$ indicate a silent action.
    \item $\sarr \subseteq S \times Act \times S$ is a transition relation, $(s, \alpha, s') \in \sarr$ is denoted by $\action{s}{\alpha}{s'}$. Specifically, $\action{s}{\epsilon}{s'}$ indicate a transition with a silent action.
\end{enumerate}
\end{definition}

\begin{definition}[LTS $\mathcal{L}_{\Lambda}$ ] A LTS derived from the operational semantics of the lambda calculus with algebraic effects $\Lambda$ is $\mathcal{L}_{\Lambda} = $ $(\Lambda^0, Act, \harr)$ where
\begin{enumerate}
    \item $\Lambda^0$ indicates all closed terms in the calculus $\Lambda$.
    \item $Act$ is the set of effects calling (name of effects and corresponding arguments).
    \item $\harr$ is based on the reduction relation such that
    \begin{align*}
        &\action{e}{\alpha}{e'} \iff e \hookrightarrow e' \quad \text{ with rule } \S{STPerform} \land \alpha \in E \\
        &\action{e}{\epsilon}{e'} \iff e \hookrightarrow e' \quad \text{ with other rules }
    \end{align*}
\end{enumerate}
\end{definition}

\begin{definition}[Paths and Traces] For given $\mathcal{L} = (S, Act, \sarr)$, a path $\pi$ is a sequence of states $s_0;s_1;s_2;...;s_n$ such that
\begin{enumerate}
    \item The sequence is not empty.
    \item The sequence is finite.
    \item For all $s_i$ and $s_{i+1}$, there is a transition $\action{s_i}{}{s_{i+1}}$ (include unlabelled transition $\epsilon$).
\end{enumerate}
A trace $L(\pi)$ is the labels of a path $\pi$.
If there is path $\pi = s_0;s_1;s_2;...;s_n$, we say $s_0$ can reach $s_n$ via trace $L(\pi)$, denoted as $\maction{s_0}{L(\pi)}{s_n}$.
\end{definition}

\begin{definition}[Free LTS ] The free category of the LTS $\mathcal{L} = (S, Act, \sarr)$ is a LTS $\hat{\mathcal{L}} = (\Pi, Act, \sarr^{\#})$ where
\begin{enumerate}
    \item $\Pi$ indicates the set of the paths in the $\mathcal{L}$.
    \item $\sarr^{\#}$ is lift from $\sarr$ such that
    \begin{align*}
        \action{\pi_1}{\alpha}{\pi_2} \iff \exists \pi_0 \ s_1\ s_2, \pi_1 = \pi_0; s_1 \land \pi_2 = \pi_0; s_1; s_2 \land \action{s_1}{\alpha}{s_2}
    \end{align*}
\end{enumerate}
\end{definition}

\begin{definition}[Weak Bisimulation] For given LTS $\mathcal{L} = (S, Act, \sarr)$, the weak bisimulation is a relation $R\subseteq S \times S$ such that
\begin{align*}
    &\forall s_1\ s_2, (s_1, s_2) \in R \impl \action{s_1}{\epsilon}{s_1'} \impl \exists s_2', \maction{s_2}{\epsilon^*}{s_2'} \land (s_1', s_2') \in R \\
    &\forall s_1\ s_2, (s_1, s_2) \in R \impl \action{s_1}{\alpha}{s_1'} \impl \exists s_2', \maction{s_2}{\epsilon^*\alpha\epsilon^*}{s_2'} \land (s_1', s_2') \in R
\end{align*}
where $\epsilon^*$ indicate traces that only contains the silent actions.
\end{definition}

\begin{definition}[Language Formalization] For the free LTS $\hat{\mathcal{L}}_{\Lambda} = (\Pi, Act, \harr^{\#})$ and a LTS $\mathcal{L} = (S, Act, \sarr)$ that share the same action space, we define the language we consider is the union of them $\hat{\mathcal{L}}_{\Lambda} + \mathcal{L} = (\Pi \cup S, Act, \sarr^{\#\#})$.
\end{definition}

\begin{definition}[Soundness and Completeness] For given $\hat{\mathcal{L}}_{\Lambda} + \mathcal{L} = (\Pi \cup S, Act, \sarr^{\#\#})$, the initial state $s_I \in S$ and a set of terminal states $Q$ in $\mathcal{L}$, the reduction of a term $e$
\begin{enumerate}
    \item (Soundness) only performs traces from $s_I$ to $Q$ in $\mathcal{L}$ iff exists a weak bisimulation $\sim$ such that
    \begin{align*}
        & [e] \sim s_I \\
        & \forall \pi\ v, \maction{e}{L(\pi)}{v} \impl \exists s' \in Q, e;\pi;v \sim s'
    \end{align*}
    \item (Completeness) performs all traces from $s_I$ to $Q$ in $\mathcal{L}$ iff exists a weak bisimulation $R$ such that
    \begin{align*}
        & s_I \sim [e] \\
        & \forall \pi\ s'\in Q, e;\pi;v \sim s' \impl \exists v, \maction{e}{L(\pi)}{v}
    \end{align*}
\end{enumerate}
\end{definition}

% \item $s_I$ is the initial state. Here we have a single initial state, which is consistent with the reduction of the test generator -- the reduction always start from a single term.

\begin{definition}[State Predicate] For given LTS $\mathcal{L} = (S, Act, \sarr)$, $\Theta$ is a set of predicates over the states.
\end{definition}

Consider a simple algebraic effect $\S{Put}{:}\mathrm{N}\sarr 1$ and $\S{Get}{:}1 \sarr\mathrm{N}$, the test generator will use two operations to simulate them
\begin{align*}
    &\S{MkPut}{:}\mathrm{N}\times 1 \sarr 1 \\
    &\S{MkGet}{:}1\times \mathrm{N} \sarr 1
\end{align*}
we provide two LTS as examples for this setting.

\begin{example} [Hidden Store] A state can be the value saved in the hidden store, thus $S$ is the natural number $\mathrm{N}$. The $Act$ is $\{\S{MkGet}\ ((), 0);\S{MkGet}\ ((), 1);... \S{MkPut}\ (0, ()); \S{MkPut}\ (1, ());... \}$, which is all possible events in the put\&get model.  The transition relation defined as the following
\begin{align*}
    &\action{s}{\S{MkGet}\ ((), m)}{s'} \iff s = s' \land s = m \\
    &\action{s}{\S{MkPut}\ (m, ())}{s'} \iff s' = m
\end{align*}
The $\Theta$ contains a single predicate $lookup(s,n)$, which is defined inductively
\begin{align*}
\text{Base Case: }& lookup(s_I, n) \iff n = m \\
\text{Inductive Case: }& lookup(s, n) \iff \exists s', (\action{s'}{\S{MkGet}\ ((), n)}{s} \land lookup(s', n)) \lor \action{s'}{\S{MkPut}\ ((), n)}{s}
\end{align*}
\AM{$S_I$ can be defined as a part of the definition of the transition system. }
which means that initially the hidden store is initialized as some natural number $m$ (here, of course we additionally require $m = s_I$). Here is a simpler definition
\begin{align*}
    lookup(s, n) \iff s = n
\end{align*}
which is equivalent. We define $lookup$ in a more complicate way to make sure it is consistent with the second example.
\end{example}
\AM{I am having a problem trying to understand this relation. Let us take an example, suppose I have an effectful language; I am not able to model the operational semantics of the calculus to this form.  }

\begin{example} [Reduction Relation] The state $S$ can be a set of reduction paths $p \doteq e_I \harr e_1 \harr ...$ from a fixed term $e_I$ in a effectful language, $Act$ defined as above. The transition relation can be defined based on the operational semantics over terms. For a single reduction step $\step{e}{e'}$, we have transition $\action{p;e}{op\ \overline{v}}{p;e;e'}$ iff $e$ can reduce to $e'$ with the small-step reduction rule $\S{STPerform}$ (the rule evaluate the effectful operation calling) over the operation $op$ and arguments $\overline{v}$; otherwise the transition is unlabelled: $\action{p;e}{\epsilon}{p;e;e'}$. The $\Theta$ contains a single predicate $lookup(s,n )$, which is defined inductively
\begin{align*}
\text{Base Case: }& lookup(s_I, n) \iff n = m \\
\text{Inductive Case: }& lookup(s, n) \iff \exists s', (\action{s'}{\S{MkGet}\ ((), n)}{s} \land lookup(s', n)) \lor \action{s'}{\S{MkPut}\ ((), n)}{s}
\end{align*}
which means that initially the hidden store is initialized as some natural number $m$.
\end{example}
% \AM{This is not clear, I thought user is not writing these LTS, rather, user writes a test generator program in an effectful language, and we interpret the given program in something similar to the second LTS, same as we would do with any operational semantics.}

\ZZ{Details example} Consider a random test generator $\S{gen}$ and trivial handler $\S{h}$.
\begin{minted}[fontsize = \footnotesize,xleftmargin = 10pt,escapeinside=<>]{ocaml}
let gen () : unit=
    let n = random_nat () in
    MkPut (n, ()); MkGet ((), n)
let h (gen: unit -> unit): unit =
    match gen () with {
        retc = fun _ -> ();
        effc = function
            | MkPut (_, _) k -> k ()
            | MkGet (_, _) k -> k ()
    }
\end{minted}
Now we define the term $e_I$ as $\S{h}\ \S{gen}$. Then we have reduction relation shown below

\adjustbox{max width=\textwidth}{
\begin{tikzcd}
{\S{h}\ (\S{MkPut}\ (1, ()); \S{MkGet}\ ((), 1))} \arrow[r, "{\S{MkPut}\ (1, ())}"] & {\lambda \_.\S{h}\ \S{MkGet}\ ((), 1))\ () } \arrow[r,] & {\S{h}\ (\S{MkGet}\ ((), 1))} \arrow[r, "{\S{MkGet}\ ((), 1)}"] & \lambda \_.\S{h}\ ())\ () \arrow[r,] & \S{h}\ () \arrow[r,] & \lambda \_.()\ () \arrow[r,] & () \\
\S{h}\ \S{gen} \arrow[u,] \arrow[d,] \arrow[r,]    & ...                                                                &                                                                 &                                                 &                                 &                                         &    \\
{\S{h}\ (\S{MkPut}\ (2, ()); \S{MkGet}\ ((), 2))} \arrow[r]                         & ...                                                                &                                                                 &                                                 &                                 &                                         &   
\end{tikzcd}
}
Then states are paths
\begin{align*}
    &\S{h}\ \S{gen} \\
    &\S{h}\ \S{gen}; \S{h}\ (\S{MkPut}\ (1, ()); \S{MkGet}\ ((), 1)) \\
    &\S{h}\ \S{gen}; \S{h}\ (\S{MkPut}\ (1, ()); \S{MkGet}\ ((), 1)); \lambda \_.\S{h}\ \S{MkGet}\ ((), 1))\ (); \S{h}\ (\S{MkGet}\ ((), 1) \\
    &\S{h}\ \S{gen}; \S{h}\ (\S{MkPut}\ (2, ()); \S{MkGet}\ ((), 2))
\end{align*}



In general, the user will write down the LTS as in the first example; on the other hand, we will derive the LTS from the impelementation of the test generator similar with the second example. The soundness and completeness of will be phrased as the relation of these two LTS. Precisely, the relation are about the ``traces'' in these two LTS.

\begin{definition}[Paths and Traces] A path $\pi$ is a finite sequence of states $s_0;s_1;s_2;...;s_n$ such that
\begin{enumerate}
    \item $s_0$ is the initial state $s_I$
    \item for all $s_i$ and $s_{i+1}$, there is a transition $\action{s_i}{}{s_{i+1}}$ (include unlabelled transition $\epsilon$).
\end{enumerate}
A path is maximal iff $s_n$ is a terminal state (no transition starts from $s_n$).
We say a path $s_0;s_1;s_2;...;s_n$ can reach a set of states $\Phi \subseteq S$, when $s_n \in \Phi$.
The trace is the labels of a path $\pi$, denoted as $L(\pi)$ such that
\begin{align*}
    &L(s_I) = \emptyset \\
    &L(...;s_n;s_{n+1}) = L(...;s_n); \alpha  \quad \text{ when } \action{s_n}{\alpha}{s_{n+1}} \\
    &L(...;s_n;s_{n+1}) = L(...;s_n) \quad \text{ when } \action{s_n}{\epsilon}{s_{n+1}}
\end{align*}
Similarly, we say a trace is maximal (can reach a set of state $\Phi$, resp.) when the underline path does. We denote the set of traces reaching $\Phi$ in a LTS $\mathcal{L}$ as $Tr(\mathcal{L}, \Phi)$, additionally, the set of the terminate traces are denoted as $Tr_{\square}(\mathcal{L}, \Phi)$.
\end{definition}

\begin{example} As the two LTS above share the same $Act$ and $\Theta$, it is obvious that the two LTS above share the same form of traces and $\Phi$. Assume the user want to reach a set of states $\Phi$ such that
\begin{align*}
    \forall s, s \in \Phi \iff (\exists m, lookup(s, m) \land m < 3)
\end{align*}
which means the value saved in the hidden store (in the second LTS, it has a more complicate interpretation, that is the argument of the last $\S{MkPut}$) is less than $3$. Then there are several valid traces
\begin{align*}
    &\emptyset \\ 
    &\S{MkGet}\ ((), 1); \S{MkGet}\ ((), 1); \S{MkGet}\ ((), 1) \\
    &\S{MkPut}\ (7, ()); \S{MkGet}\ ((), 7); \S{MkPut}\ (2, ())
\end{align*}
\end{example}

Before we connect the implementation of test generator $e$ and the LTS defined by the user, we formalized the LTS derived from a term.
\AM{This is same as the second LTS above in Example 1.3? I do not understand the need for this.}\ZZ{to define the soundness and completeness.}
\begin{definition} [LTS of term] For a term $e_I$, the reduction relation $\hookrightarrow$, action $Act$ and predicates $\Theta$, we can define a LST as $(\{ e_0;e_1;e_2... ~|~ \step{e_i}{e_{i+1}}, e_0 = e_I \},Act, \harr {\uparrow}, e_I, \Theta)$, Precisely,
\begin{enumerate}
    \item $\{ e_0;e_1;e_2... ~|~ \step{e_i}{e_{i+1}}, e_0 = e_I \}$ indicates all reduction paths that $e_I$ can reduce to.
    \item $\harr {\uparrow}$ is lift the reduction relation, that is
    \begin{align*}
        &\action{p;e}{\alpha}{p;e;e'} \iff e \hookrightarrow e' \quad \text{ with rule } \S{STPerform} \land \alpha \in Act \\
        &\action{p;e}{\epsilon}{p;e;e'} \iff e \hookrightarrow e' \quad \text{ with other rules }
    \end{align*}
\end{enumerate}
denoted as $\mathcal{L}(e_I, Act, \Theta)$.
\end{definition}

\begin{example}
    The second LTS.
\end{example}

For given ``postcondition'' $\Phi$ that is a first order formula over predicates in $\Theta$, we can define a refinement relation over two LTS, when all traces reaching $\Phi$ in $\mathcal{L}$ is included in the traces reaching $\Phi$ in $\mathcal{L'}$.


\begin{definition} [Soundness and Completeness] For a given LTS $\mathcal{L} = (S, Act, \sarr, s_I, \Theta)$, postcondition $\Phi$ and the term $e$
\begin{enumerate}
    \item term $e$ is a sound (safety) impelementation of the generator iff
    \begin{align*}
    Tr_{\square}(\mathcal{L}(e, Act, \Theta),\Phi) \subseteq Tr(\mathcal{L}, \Phi)
    \end{align*}
    \item term $e$ is a complete (coverage) impelementation of the generator iff     
    \begin{align*}
    Tr(\mathcal{L}, \Phi) \subseteq Tr_{\square}(\mathcal{L}(e, Act, \Theta), \Phi)
    \end{align*}
\end{enumerate}
Notice that, we require the traces in $\mathcal{L}(e, Act, \Theta)$ are terminal traces.
\end{definition}

\subsection{Complete up to Refinement}
\AM{This section makes sense.}
There is a interesting case in the completeness, that is we can weaken the completeness guarantee by defining the refinement relation over the traces.

\begin{definition} [Completeness up to refinement] For a given LTS $\mathcal{L} = (S, Act, \sarr, s_I, \Theta)$, postcondition $\Phi$ and the term $e$, assume $\sqsubseteq$ is a partial order relation over all traces in $\mathcal{L}$ ($Tr(\mathcal{L}, \top)$). Then $e$ is complete up to $\sqsubseteq$ when
\begin{align*}
    \forall tr, tr \in Tr(\mathcal{L}, \Phi) \impl \exists tr', tr' \sqsubseteq tr \land tr' \in Tr_{\square}(\mathcal{L}(e, Act, \Theta), \Phi)
\end{align*}
\end{definition}

To make user define the refinement relation easily, we consider a special form of refinement, that is deriving trace equality from the state equality.

\begin{definition} [refinement of state equality] In a LTS $\mathcal{L} = (S, Act, \sarr, s_I, \Theta)$ and a state equality relation $\simeq$ over $S$, the derived the refinement relation $\sqsubseteq_p$ over paths
\begin{align*}
    &\forall s\ s'\ \pi_1\ \pi_2\ \pi_3, s \simeq s' \iff
    \pi_1;s;\pi_3 \sqsubseteq_p \pi_1;s;\pi_2;s';\pi_3
\end{align*}
Then the refinement relation $\sqsubseteq$ over traces is
\begin{align*}
    \forall \pi\ \pi', \pi \sqsubseteq_p \pi' \iff  L(\pi) \sqsubseteq L(\pi')
\end{align*}
\end{definition}

\begin{example} In the first LTS example above, there is an equality relation over states that is $=_{nat}$. Then a path $0;0;3;4;3$ can be refined as $0;3$. Thus the we can say
\begin{align*}
\S{MkPut}\ (3, ()) \sqsubseteq
    \S{MkGet}\ ((), 0); \S{MkPut}\ (3, ()); \S{MkPut}\ (4, ()); \S{MkPut}\ (3, ())
\end{align*}
\end{example}

Notice that I use the refinement relation instead of equality relation over the traces, because we always expect the generator generate the short trace (e.g., $\S{MkPut}\ ((), 3)$) instead of the longer one.

Dully, the refinement relation may strengthen the soundness requirement.

\begin{definition} [Soundness up to refinement] For a given LTS $\mathcal{L} = (S, Act, \sarr, s_I, \Theta)$, postcondition $\Phi$ and the term $e$, assume $\sqsubseteq$ is a partial order relation over all traces in $\mathcal{L}$ ($Tr(\mathcal{L}, \top)$). Then $e$ is sound up to $\sqsubseteq$ when
\begin{align*}
    \forall tr, tr \in Tr_{\square}(\mathcal{L}(e, Act, \Theta), \Phi) \impl \forall tr', tr' \sqsubseteq tr \land tr' \in Tr(\mathcal{L}, \Phi) \implies tr = tr'
\end{align*}
which indicate all traces $e$ generated are ``minimal''.
\end{definition}

\paragraph{Problem} For given LTS $\mathcal{L}$ and equality relation over states $\simeq$, check if a term $e$ is sound and complete up to the trace refinement relation derived from $\simeq$.

==> draft/meta2.tex <==
\section{Meta Theory}

Now we introduce the formalization and the corresponding soundness and completeness theorems for the ``stateful property-based testing'' and corresponding generator.

From the user perspective, the test generator actually generate traces in the labeled transition system (LTS) from the initial states to the states specified the users.

\begin{definition}[Labeled transition system] A labeled transition system (LTS) is a tuple $\mathcal{L} = (S, Act, \sarr)$ such that
\begin{enumerate}
    \item $S$ is a set of states (the state space).
    \item $Act \cup \{\epsilon\}$ is a set of actions (Act is the label space), where $\epsilon$ indicate a silent action.
    \item $\sarr \subseteq S \times Act \times S$ is a transition relation, $(s, \alpha, s') \in \sarr$ is denoted by $\action{s}{\alpha}{s'}$. Specifically, $\action{s}{\epsilon}{s'}$ indicate a transition with a silent action.
\end{enumerate}
\end{definition}

\begin{definition}[LTS $\mathcal{L}_{\Lambda}$ ] A LTS derived from the operational semantics of the lambda calculus with algebraic effects $\Lambda$ is $\mathcal{L}_{\Lambda} = $ $(\Lambda^0, Act, \harr)$ where
\begin{enumerate}
    \item $\Lambda^0$ indicates all closed terms in the calculus $\Lambda$.
    \item $Act$ is the set of effects calling (name of effects and corresponding arguments).
    \item $\harr$ is based on the reduction relation such that
    \begin{align*}
        &\action{e}{\alpha}{e'} \iff e \hookrightarrow e' \quad \text{ with rule } \S{STPerform} \land \alpha \in E \\
        &\action{e}{\epsilon}{e'} \iff e \hookrightarrow e' \quad \text{ with other rules }
    \end{align*}
\end{enumerate}
\end{definition}

\begin{definition}[Paths and Traces] For given $\mathcal{L} = (S, Act, \sarr)$, a path $\pi$ is a sequence of states $s_0;s_1;s_2;...;s_n$ such that
\begin{enumerate}
    \item The sequence is not empty.
    \item The sequence is finite.
    \item For all $s_i$ and $s_{i+1}$, there is a transition $\action{s_i}{}{s_{i+1}}$ (include unlabelled transition $\epsilon$).
\end{enumerate}
A trace $L(\pi)$ is the labels of a path $\pi$.
If there is path $\pi = s_0;s_1;s_2;...;s_n$, we say $s_0$ can reach $s_n$ via trace $L(\pi)$, denoted as $\maction{s_0}{L(\pi)}{s_n}$.
\end{definition}

\begin{definition}[Free LTS ] The free category of the LTS $\mathcal{L} = (S, Act, \sarr)$ is a LTS $\hat{\mathcal{L}} = (\Pi, Act, \sarr^{\#})$ where
\begin{enumerate}
    \item $\Pi$ indicates the set of the paths in the $\mathcal{L}$.
    \item $\sarr^{\#}$ is lift from $\sarr$ such that
    \begin{align*}
        \action{\pi_1}{\alpha}{\pi_2} \iff \exists \pi_0 \ s_1\ s_2, \pi_1 = \pi_0; s_1 \land \pi_2 = \pi_0; s_1; s_2 \land \action{s_1}{\alpha}{s_2}
    \end{align*}
\end{enumerate}
\end{definition}

\begin{definition}[Weak Bisimulation] For given LTS $\mathcal{L} = (S, Act, \sarr)$, the weak bisimulation is a relation $R\subseteq S \times S$ such that
\begin{align*}
    &\forall s_1\ s_2, (s_1, s_2) \in R \impl \action{s_1}{\epsilon}{s_1'} \impl \exists s_2', \maction{s_2}{\epsilon^*}{s_2'} \land (s_1', s_2') \in R \\
    &\forall s_1\ s_2, (s_1, s_2) \in R \impl \action{s_1}{\alpha}{s_1'} \impl \exists s_2', \maction{s_2}{\epsilon^*\alpha\epsilon^*}{s_2'} \land (s_1', s_2') \in R
\end{align*}
where $\epsilon^*$ indicate traces that only contains the silent actions.
\end{definition}

\begin{definition}[Language Formalization] For the free LTS $\hat{\mathcal{L}}_{\Lambda} = (\Pi, Act, \harr^{\#})$ and a LTS $\mathcal{L} = (S, Act, \sarr)$ that share the same action space, we define the language we consider is the union of them $\hat{\mathcal{L}}_{\Lambda} + \mathcal{L} = (\Pi \cup S, Act, \sarr^{\#\#})$.
\end{definition}

\begin{definition}[Soundness and Completeness] For given $\hat{\mathcal{L}}_{\Lambda} + \mathcal{L} = (\Pi \cup S, Act, \sarr^{\#\#})$, the initial state $s_I \in S$ and a set of terminal states $Q$ in $\mathcal{L}$, the reduction of a term $e$
\begin{enumerate}
    \item (Soundness) only performs traces from $s_I$ to $Q$ in $\mathcal{L}$ iff exists a weak bisimulation $\sim$ such that
    \begin{align*}
        & [e] \sim s_I \\
        & \forall \pi\ v, e;\pi;v \in \hat{\mathcal{L}}_{\Lambda} \impl  \exists s' \in Q, e;\pi;v \sim s'
    \end{align*}
    \item (Completeness) performs all traces from $s_I$ to $Q$ in $\mathcal{L}$ iff exists a weak bisimulation $R$ such that
    \begin{align*}
        & s_I \sim [e] \\
        & \forall s'\in Q, \exists \pi\ v, e;\pi;v \sim s'
    \end{align*}
\end{enumerate}
\end{definition}

\begin{definition} [Type denotation] or given $\hat{\mathcal{L}}_{\Lambda} + \mathcal{L} = (\Pi \cup S, Act, \sarr^{\#\#})$, The formula $\phi$ of the refinement type $\nuut{b}{\phi}$ can describe
\begin{enumerate}
    \item A set of states in $S$.
    \item A set of state in $\hat{\mathcal{L}}_{\Lambda}$ that is a set of path in $\mathcal{L}_{\Lambda}$.
\end{enumerate}
A term $e$ as the
\begin{enumerate}
    \item over type $\nuot{b}{\phi}$, when $\forall \pi, (\exists v, \maction{e}{L(\pi)}{v}) \impl \phi(\pi)$.
    \item under type $\nuut{b}{\phi}$, when $\forall \pi, \phi(\pi) \impl \exists v, \maction{e}{L(\pi)}{v}$.
\end{enumerate}
\end{definition}

==> draft/pldi23.tex <==
\newpage

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=<>, linenos = true]{ocaml}
type 'a tree =
  | Leaf
  | Node of ('a * 'a tree * 'a tree)
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=<>, linenos = true, firstnumber=last]{ocaml}
let rec foo (lo: int) (hi: int) : int tree =
  if lo + 1 >= hi then Leaf else
  let (x: int) = int_range (lo, hi) in
  Node (x, foo lo x, foo x hi)
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=<>, linenos = true, firstnumber=last]{ocaml}
let rec build_bst (lo: int) (hi: int) : int tree =
  if lo + 1 >= hi then Leaf else
  let (x: int) = int_range (lo, hi) in
  Node (x, build_bst lo x, build_bst x hi)
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=&&, linenos = true, firstnumber=last]{ocaml}
let rec bst_gen (lo: int) (hi: int) : int tree =
  if lo + 1 >= hi then Leaf else
  Leaf &$\oplus$&
  let (x: int) = int_range (lo, hi) in
  Node (x, bst_gen lo x, bst_gen x hi)
\end{minted}

\begin{align*}
&\phi(v, lo, hi) \doteq bst(v) \land \forall n{:}int. mem(v, n) \impl lo < n < hi \\
&\forall v{:}int\ tree. \textcolor{blue}{\Code{built\_bst}\ 0\ 3}\Downarrow v \impl \phi(v, 0, 3) \\
&\forall v{:}int\ tree. \phi(v, 0, 3) \impl \textcolor{blue}{\Code{bst\_gen}\ 0\ 3}\Downarrow v \\
\end{align*}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=&&]{ocaml}
if lo + 1 >= hi then Leaf else       : &$\nuut{int\ tree}{lo + 1 \geq hi \land emp(\vnu)}$&
Leaf &$\oplus$&                               : &$\nuut{int\ tree}{lo + 1 < hi \land emp(\vnu)}$&
let (x: int) = int_range (lo, hi) in
Node (x, bst_gen lo x, bst_gen x hi) : &$\nuut{int\ tree}{lo + 1 < hi \land \neg emp(\vnu) \land \phi(\vnu, lo, hi)}$&
: &$\nuut{int\ tree}{\phi(\vnu, lo, hi)}$&
\end{minted}

\begin{align*}
&(lo + 1 \geq hi \land emp(\vnu)) \lor (lo + 1 < hi \land emp(\vnu)) \lor \\
&(lo + 1 < hi \land \neg emp(\vnu) \land \phi(\vnu, lo, hi)) \\
&\impl \phi(\vnu, lo, hi)
\end{align*}

\begin{align*}
& \emptyset \\
&\textcolor{red}{(lo + 1 \geq hi \land \neg emp(\vnu) \land \phi(\vnu, lo, hi))} \lor \\
&(emp(\vnu) \textcolor{orange}{\land \phi(\vnu, lo, hi)} ) \lor \\
&(lo + 1 < hi \land \neg emp(\vnu) \land \phi(\vnu, lo, hi)) \\
&\impl \phi(\vnu, lo, hi)
\end{align*}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, fontsize = \footnotesize, escapeinside=&&]{ocaml}
if lo + 1 >= hi then Leaf else
Leaf &$\oplus$&
let (x: int) = int_range (lo, hi) in
Node (x, bst_gen lo x, bst_gen x hi)
\end{minted}

\begin{align*}
&\Code{bst\_gen}\ 0\ 3 \\
&\Code{bst\_gen}\ 0\ 2 \quad \Code{bst\_gen}\ 2\ 3\\
&\Code{bst\_gen}\ 0\ 1 \quad \Code{bst\_gen}\ 1\ 2
\end{align*}

\begin{align*}
&\Code{lo}{:}?\sarr\Code{hi}{:}?\sarr\nuut{int\ tree}{\phi(\vnu, \Code{lo}, \Code{hi})} \\
&\Code{lo}{:}\nuot{int}{\vnu = 0}\sarr\Code{hi}{:}\nuot{int}{\vnu = 3}\sarr\nuut{int\ tree}{emp(\vnu)} \\
&\Code{lo}{:}\nuot{int}{\vnu = 0}\sarr\Code{hi}{:}\nuot{int}{\vnu = 3}\sarr\nuut{int\ tree}{\phi(\vnu, \Code{lo}, \Code{hi})} \\
&\Code{lo}{:}\nuot{int}{\top}\sarr\Code{hi}{:}\nuot{int}{\Code{lo} \leq \nu}\sarr\nuut{int\ tree}{\phi(\vnu, \Code{lo}, \Code{hi})}
\end{align*}

\begin{flalign*}
 &\text{\textbf{Type Synthesis }} &
 \fbox{$\Gamma \covervdash e \typeinfer \tau$}&&
  &\text{\textbf{Type Check }} &
 \fbox{$\Gamma \covervdash e \typecheck \tau$}
\end{flalign*}

\textbf{Fundamental Theorem}

\textbf{Type Soundness}

\textbf{SMT-based subtyping algorithm}

\begin{align*}
&\Gamma \vdash e : \nuot{t}{\phi} \\
&\Gamma \vdash e : \nuut{t}{\phi} \\
&\otparenth{\,P\,}\; e\; \otparenth{\,Q\,} \\
&\utparenth{\,P\,}\; e\; \utparenth{\,Q\,}
\end{align*}

==> draft/regex-cfg.tex <==
\section{The Language We Used to Express Events}

We can just use the regular language instead of the context-free language in the coverage analysis, which means that it is sound and able to solve most of problems we are interesting in.

The different between the the regular language and the context-free language is that the production rule of the former is either right or left linear, while the context-free language allows to have the following rules:
\begin{align*}
    S \to aSb
\end{align*}
which make the context-free language has a more precise expressive power than the regular expression, e.g., the character ``$($'' and ``$)$'' appeared as pairs in the string. 

The language we use for the events should consider the source code and the user-defined specification (protocols). In general, we can always do approximation of the events can produced by the source code, however, the user-defined specification is more critical that describes the property we want.

From now, we use the motivating example of the paper suggested by Ben: Verifying Correct Usage of Context-Free API Protocols.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* Protocal &$G_S$&, n is some identifiers for a lock. *)
S &$\to$& lock(n) S unlock(n)
S &$\to\ \epsilon$&
(* Generator. *)
let rec gen_G_S () =
    () &$\oplus$& 
    let n = random_lock_id () in
    lock(n);
    gen_G_S ();
    unlock(n)
(* Event Seunece: *)
lock(1); unlock(1)
lock(7); lock(1); unlock(1); unlock(7)
lock(9); lock(2); lock(3); unlock(3); unlock(2); unlock(9)
...
\end{minted}

\subsection{The pairing relation is not the main point of the state readability and coverage analysis}

Our problem setting put the goal as ``enumerate'' all possible events that reach the desirable states. Moreover, to facilitate the generator cover all traces efficiently, we ask the user to provide the equivalence equations to filter out redundant traces. Here, the context-free grammar $G_S$ exactly describes the ``redundant traces'' which is the equivalent class of $\epsilon$ of the following equivalence relation:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* equivalence equations *)
s; lock(n); unlock(n) = s
(* unlock state generator *)
let gen = ()
\end{minted}
In other word, the desirable generator will only generate one (e.g., the empty trace) of the traces listed above, which is sufficient to represent all traces in the $L(G_S)$. The overapproximate analysis care about if all usage of the APIs is the subset of the $L(G_S)$, on the other hand, the underapproximate analysis plus the equivalence equations care about the coverage of the quotient set, where all details and precise specification that can only be expressed by CFG is captured by the equivalent classes.

One better example maybe the complement of the unlock state generator, that is a generator able to enumerate all traces up to the equivalence equation $\Code{s; lock(n); unlock(n) = s}$.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* equivalence equations *)
s; lock(n); unlock(n) = s
(* unlock state generator *)
let rec gen_last_lock n =
    let m = random_lock_id () in
    (lock(m); gen_last_lock m) &$\oplus$&
    (if n == m then Err else unlock(m); gen ())
let gen () =
    let n = random_lock_id () in
    (lock(n); gen_last_lock n) &$\oplus$&
    (unlock(n); gen ())
\end{minted}
The auxiliary function $\Code{gen\_last\_lock}$ records the identifier of the last locked lock, and the conditional expression in its body guarantees the the program never generate $\Code{lock(n); unlock(n)}$. The traces enumerated by the function can be described by the complement of the regular expression ``$\Code{.*lock([a-z]); unlock([a-z]).*}$'' (complement of a regex is also a regex). This regular expression ``product'' with the $G_S$ is able to cover all possible traces.

In high level, the paring relation means we reentry a state we have traversed before, it is another way to say the traces are ``redundent''. The context-free language means there is hidden state need to be capture during ``parsing'' the sequence of events linearly. It is somehow conflict with our goal -- plan a path to reach a desirable state where we explicitly know the this state. Thus, if there indeed has hidden states, like the re-entrant lock here, it should be ``forgetten'' by the quotation that provided by the users.

\subsection{Approximate Protocol Is More Reasonable in the Coverage Analysis}

One question is that, if the user don't provide any (or even don't care about) equivalence equations, is the CFG is necessary? For example, the $\Code{lock(7); lock(1); unlock(1); unlock(7)}$ is just not equal to $\Code{lock(1); unlock(1)}$ because we have to get the lock $\Code{7}$ before lock the lock $\Code{1}$. Thus the users don't believe this equation is valid.

Reconsider the protocol $G_S$ which describes which exactly describe all valid usage of the APIs the re-entrant lock. In the overapproximate (safety) verification, the problem that it is even hard to find a reasonable analogue of $G_S$ in the regular expression. The sound analogue here means a a regular expression $R$ such that $L(R) \subseteq L(G_S)$. There are some trivial examples:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* R1 *)
S &$\to\ \epsilon$&
(* R1 *)
S &$\to$& lock(n);unlock(n)
S &$\to\ \epsilon$&
(* R2 *)
S &$\to$& lock(n);lock(m);unlock(m);unlock(n)
S &$\to$& lock(n);unlock(n)
S &$\to\ \epsilon$&
\end{minted}
where the analogue is simply finite subset of $L(G_S)$, where the worse case is $\emptyset$. It is too strict for any complicate program that has recursion.

On the other hand, in the underapproximate (coverage) verification, the sound analogue means that we should find the regular expression that produce a super set of $L(G_S)$ which also infinite (the worse case is ``$.*$''), it fits the realistic generators that mostly generate infinite outputs.

In order to show that the coverage analysis just avoid to touch the CFG instead of expressing $L(G_S)$ in the regular expression, consider one valid test generator
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
let gen () =
    let n = random_lock_id () in
    (lock(n); gen ()) &$\oplus$& (unlock(n); gen ())
\end{minted}
which is valid in the coverage verification but not valid in the safety verification with the protocol $G_S$.

One may curious about the type of the function $\Code{gen\_G\_S}$ shown in the beginning. If we have the equivalence relation, of course it can only cover ``$\nuut{s}{\epsilon}$'' (the empty sequence, assume the trace type is represented in the regular expression). On the other hand, without the equivalence relation, it can be type checked with ``$\nuut{s}{\epsilon}$'', ``$\nuut{s}{\epsilon {||} lock(n);unlock(n) }$''. These coverage types are trivial finite underapproximation of the behaviours of $\Code{gen\_G\_S}$ (it is similar with $R_1$, $R_2$ and $R_3$). However, it is OK because $\Code{gen\_G\_S}$ itself is not a good test generator at all, it doesn't cover any interesting states for the PBT. In summary, the regular expression aligns with the coverage analysis perfectly that is able to express the events of the generators we are interested in.

==> draft/scracth.tex <==
\section{Introduction}\label{sec:intro}
\section{Overview}\label{sec:overview}
\section{Language}\label{sec:lang}
\section{Type System}\label{sec:rules}
\section{Typing Algorithm}\label{sec:algorithm}
\section{Evaluation}\label{sec:evaluation}
\section{Related Work}\label{sec:related}
\section{Conclusion}\label{sec:conc}


==> draft/st-tr.tex <==
\section{Problem Setting}

\subsection{Input}
Users provide the following types for the effectful operators:

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
val put: nat * int -> unit
val get: nat -> int
\end{minted}

and the following equivalence relations over programs:

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
&$\forall C$& (k: nat) (n: int), put (k, n); get k; &$C$& = put (k, n); &$C$&
\end{minted}

Now the user want a generator to enumerate traces whose terminal states can cover all \emph{distinct} states in the protocol. These states can be the start points of the further testing. Notice that, we are testing client code $C$ and assuming the implementation of library (the interface ``put'' and ``get'') is correct. In other words, our test generator is not generate any datatypes or traces, it generates states. 

\subsection{Monadic Interpretation}
Now we assume there is an \emph{abstract state} $s:S$ indicate the hidden states of the effectful operators. Then the inputs are
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
val put: S -> nat * int -> (S * unit)
val get: S -> nat -> (S * int)
\end{minted}

and the following equivalence relations over \emph{states}:

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
&$\forall (s: S)$& (k: nat) (n: int), 
    (let s, _ = put s (k, n) in let s, _ = get s k in s) = 
    (let s, _ = put s (k, n) in s)
\end{minted}
where the equivalent relation over $s$ is defined over the sequence of events (traces). Or in the form of type class:

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{coq}
Class State (S : Type) :=
  { eq : S -> S -> Prop;
    eqb_coind : forall s1 s2, eq s1 s2 -> forall (k: nat) (n: int), 
        eq (fst (get (fst (put s1 (k, n))) k))
           (fst (put s2 (k, n)))
    }.
\end{minted}

The the user want, for the given generator $gen$ is able to cover all states whatever what instance of $State\ S$ we choose.
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{coq}
forall (S: Type) (_: State S) (s0: S) (s: S), exists (s': S), 
    (s, gen ()) &$\hookrightarrow^*$& (s', v) /\ eq s s'
\end{minted}

\subsection{Compare with the discussion on Wednesday}

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
val put: s&:$\nuot{int\ map}{\top}$& -> k&:$\nuot{nat}{\top}$& * v&:$\nuot{int}{\top}$& -> 
          (&$\nuut{int\ map}{\I{find}(\nu, k, v) \land \forall x\ y, x \not = k \land \I{find}(s, x, y) \impl \I{find}(\nu, x, y) }$& * unit)
val get: s&:$\nuot{int\ map}{\top}$& -> k&:$\nuot{nat}{\exists v, \I{find}(s, \nu, v) }$& -> 
          (&$\nuut{int\ map}{\forall x\ y, \I{find}(s, x, y) \impl \I{find}(\nu, x, y) }$& * &$\nuut{int}{\I{find}(s, k, \nu)}$&)
\end{minted}

The type is very precise, need user efforts. These types actually imply a stronger assumption:
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
&$\forall C$& (k: nat) (n: int) (m: int), put (k, n); put (k, m); &$C$& = put (k, m); put (k, n); &$C$&
\end{minted}
which means a generator that puts keys in decreasing order will be treated as a complete generator while it is actually not.

\subsection{Constructive Abstract State}

What is the form of the abstract state $S$ that satisfies the equivalent relation? The weakest assumption here is the ``history of all previous events'', or the traces (co-inductively, can be all possible future traces, but kind of complicate). We defined the traces as a recursive datatype:
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
type tr = Put of (nat * int) * tr
        | Get of nat * tr
\end{minted}
Indeed, unlike $int\ map$, using $tr$ as an instance of $State$ doesn't require any stronger assumption. However, $tr$ is too weak to be consistent with the equivalent relation. For example,
\begin{align*}
    \S{Get(7, Put ((2, -1), tr))} \not =\S{Put ((2, -1), tr)}
\end{align*}
There are several ways to do it, I am not quite sure.
\begin{enumerate}
    \item Still map $tr$ to some known datatype using a function $A$, but we need to be careful, for example, $int\ map$ is a bad domain. On the other hand, $(int*nat)\ list$ storing all kv-pairs is a valid domain. The question is, how can we infer $(int*nat)\ list$? How can we know $(int*nat)\ list$ doesn't require stronger assumptions?
    \item Using $tr$ directly and using the refinement type to constraint $tr$ to always be ``normal form'' (e.g., the left-hand-side of equation is not the normal form since it can be simplified). However, the equivalent relation has not direction.
    \item \textbf{I prefer this:} Using $tr$ directly and keep the equivalent relation as a new kind of refinement.
\end{enumerate}

\subsection{Richer Inputs and formalization}

We can also add the safety requirement into the inputs by define a special error case of the abstract state. The error state will make the program get stuck.

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
val put: S -> nat * int -> (S * unit)
val clear: S -> nat -> (S * unit)
val get: S -> nat -> (S * int)
\end{minted}

\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
&$\forall (s: S)$& (k: nat),
    (let s, _ = clear s k in let s, _ = get s k in s) = err
\end{minted}

We can also constraint the return value of the operators:
\begin{minted}[fontsize = \small,xleftmargin=10pt, escapeinside=&&]{ocaml}
&$\forall (s: S)$& (k: nat) (v: int),
    (let s, _ = put s (k, v) in let _, v' = get s k in v') = v
\end{minted}

The user can also define the states that the generator need to generate more precisely:

==> draft/tr-example.tex <==
\section{Example: Put and get}

\subsection{Input}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
val[@effect] put: int * int -> unit
val[@effect] get: int -> int

fix (gen: int -> unit) (n: int) =
    let (b: bool) = n == 0 then
    if b then () else
    let (n': int) = n - 1 in
    let () = gen n' in
    let (m: int) = anynot n in
    perform Put (n, m)
\end{minted}

Monadic transformation.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
type s
val[@effect] put: s -> int * int -> (s * unit)
val[@effect] get: s -> int -> (s * int)

fix (gen: int -> unit) (s0: S) (n: int) =
    let (b: bool) = n == 0 then
    if b then (s0, ()) else
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
\end{minted}

User provided equivalence relations:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall$& s n, let s,_ = get s n; s == s
&$\forall$& s n m, let _,v = get s n; v == m &$\impl$& let s,_ = put s (n, m); s == s
&$\forall$& s n m, let s, _ = put s (n, m) in let _, v = get s n in v == m
&$\forall$& s n n' m, &$n \not= n' \impl$& let s, _ = put s (n', m) in let _, v = get s n in v == let _, v = get s n' in v 
\end{minted}

User provided type:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}

&$\vdash$& gen : &$\nuotxarr{s}{s}{\top}\nuotxarr{n}{int}{\vnu \leq 0} \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}$&
&$\phi$&:
&$\forall i, 0 \leq i < n \impl$& let _, j = get s' i in j &$\not= i $&
&$\forall i, n \leq i \impl$& let _, j = get s' i in j == let _, j = get s i in j
\end{minted}

Here we face the same problem with the Incorrectness logic, if we don't add the second line, there is no constraints of what value is stored in the state when the key is greater than $n$. 

\subsection{Pre-processing}

\newcommand{\mptr}{\I{\hat{ret}}}
\newcommand{\mpst}{\I{ret}}
\newcommand{\evappend}{{;;}}

\paragraph{Step one} Define the state type.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
type ev = Put of (int * int)
        | Get of int
        | Err
type s = ev stream 
type evs = ev list
\end{minted}

The type $s$ is defined co-inductively:
\begin{enumerate}
    \item A state (like a process) can be derived from (destructed into) an event ($\Code{Put\ (int * int)}$, $\Code{Get\ int}$ or $\Code{Err}$) and another state.
    \item $a{;;} b ::= Append(a, b)$
\end{enumerate}
For example,
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* A valid trace *)
...&$\evappend$& Put (n, m) &$\evappend$& Get n &$\evappend$& Put (n, m')
(* A trace preform get an uninitialized key (n), which will end up with Err *)
...&$\evappend$& Get n' &$\evappend$& Get n &$\evappend$& Err
\end{minted}

\paragraph{Step two} Define the refinement type of effect operators.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
val[@effect] put: &$\nuotxarr{s}{s}{\top} {\bcol{n}\nuot{int}{\top}}\tprod{\bcol{m}\nuot{int}{\top}}\sarr  \bcol{s'}{\nuut{s}{\vnu = s \evappend \Code{Put (n, m)} }}\tprod{\nuut{unit}{\mpst(s', \vnu)}}$&
val[@effect] get: &$\nuotxarr{s}{s}{\top}\bcol{n}\nuot{int}{\top}\sarr  \bcol{s'}{\nuut{s}{\vnu = s \evappend \Code{Get\ n} }}\tprod{\nuut{int}{\mpst(s', \vnu)}}$&
\end{minted}

The type $\bcol{x}\tau\tprod\tau$ is a dependent product type; $\mpst(s, \vnu)$ is a method predicate indicate the return value the given state $s$ (the history of events) is $\vnu$. Since $s$ captures all previous event and the current one (e.g., the last event of $s'$ in the type of $\Code{get}$ is exactly $\Code{Get\ n}$), this method predicate is sufficient to express the behaviours of effect operators.

\paragraph{Step three} Add the axioms to the equivalence relation $\seq$.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* From Put and Get *)
&$\forall$& s1 s2 n', s1 &$\seq$& s2 &$\impl$& s1 &$\evappend$& Get n &$\seq$& s2
&$\forall$& s1 s2 n', s1 &$\seq$& s2 &$\impl$& put s1 n = m &$\impl$& s1 &$\evappend$& Put (n, m) &$\seq$& s2
(* From Err *)
&$\forall$& s n m, s \evappend Err &$\seq$& s \evappend Err \evappend Put (n, m)
&$\forall$& s n, Err s &$\seq$& Get (Err s, n)
&$\forall$& s n, Err s &$\seq$& Err (Err s)
(* Eq Prop *)
&$\forall$& s, s &$\seq$& s
&$\forall$& s1 s2, s1 &$\seq$& s2 &$\impl$& s2 &$\seq$& s1
&$\forall$& s1 s2 s3, s1 &$\seq$& s2 &$\impl$& s2 &$\seq$& s3 &$\impl$& s1 &$\seq$& s3
\end{minted}

\paragraph{Step four} Definition $\mpst(s, \vnu)$.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\mpst$& (s: state) &$\vnu$& : &$\phi$& =
    match s with
    | s' &$\evappend$& Err -> &$\bot$&
    | s' &$\evappend$& Put (n, m) -> &$\top$&
    | s' &$\evappend$& Get (n) ->
        match s' with
        | s'' &$\evappend$& Err -> &$\bot$&
        | s'' &$\evappend$& Get (n') -> &$\mpst$& (s'' &$\evappend$& Get (n)) &$\vnu$&
        | s'' &$\evappend$& Put (n', m) when n' == n -> &$\vnu = m$&
        | s'' &$\evappend$& Put (_, _) -> &$\mpst$& (s'' &$\evappend$& Get (n)) &$\vnu$&
\end{minted}
which is the maximal specification of all possible $\mpst$.

\paragraph{Step five} Refine the refinement type of target type.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\vdash$& gen : &$\nuotxarr{s}{s}{\top} \nuotxarr{n}{int}{\vnu \leq 0} \nuut{evs}{\phi}\tprod{\nuut{unit}{\top}}$&
&$\phi$&:
&$\forall i\ j, 0 \leq i < n \land i \not=j \impl \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j) \land \forall i\ j, n \leq i \impl \mpst(s \evappend \Code{Get\ i}, j) \impl \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j) $&
\end{minted}

\subsection{To Events Type}
\ZZ{It may not a good idea, it is kind conflict with the induction and exists function}

\newcommand{\evs}{\pi}
\newcommand{\evsor}{{||}}
\newcommand{\trcond}[1]{\langle{#1}\rangle}

The type $s$ is incremental, consider a list of events, which indicates the difference between two state types. The denotation of the events language $\pi$ indicates a set of list of events, where
\small{
\begin{align*}
    \denotation{\pi} &: \Code{ev\ list\ set} \\
    \denotation{\pi} \Code{(s: s)}&::= \{\alpha \in \denotation{\pi} ~|~ s \evappend \alpha\} \\
    \denotation{\pi} \Code{(ss: s\ set)}&::= \{\beta \in ss, \alpha \in \denotation{\pi} ~|~ \beta \evappend \alpha\} \\
\end{align*}
}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\denotation{\emptyset}$& = &$\emptyset$&
&$\denotation{ev}$& = &$\{ [\Code{ev}] \}$&
&$\denotation{.}$& = &$\bigcup_{ev} \{ [\Code{ev}] \}$&
&$\denotation{\evs_1;\evs_2}$& = &$\{ \beta \in \denotation{\evs_2}, \alpha \in \denotation{\evs_1} | \beta \listconcat \alpha \}$&
&$\denotation{\evs_1\evsor\evs_2}$& = &$\{ \alpha | \alpha \in \denotation{\evs_2}, \alpha \in \denotation{\evs_1} \}$&
&$\denotation{\evs^*}$& = &$\bigcup_{n = 0}^{\infty} (\listconcat^n \denotation{\evs})$&
&$\denotation{\trcond{\phi}}$& = &$\{ \alpha | \forall (\beta:s), \denotation{\phi} (\beta \evappend \alpha) \}$&
\end{minted}
where we have an monadic interpretation of the formula $\phi$:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\denotation{\mptr(\pi, x)}$& = fun (s: s) -> &$\forall \alpha, \mpst(s \evappend \alpha, x)$&
&$\denotation{\I{mp}(\overline{x})}$& = fun (s: s) -> &$\I{mp}(\overline{x})$&
&$\denotation{\phi_1 \land \phi_2}$& = fun (s: s) -> &$\denotation{\phi_1}s \land \denotation{\phi_2} s$&
...
\end{minted}

For example,
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\denotation{\trcond{\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mptr(\Code{Get\ i}, j) }}$& = 
&$\{ \alpha | \forall (\beta:s), \denotation{\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mptr(\Code{Get\ i}, j)} (\beta \evappend \alpha) \}$&
&$\{ \alpha | \forall (\beta:s), \forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \denotation{\mptr(\Code{Get\ i}, j)} (\beta \evappend \alpha) \}$&
&$\{ \alpha | \forall (\beta:s), \forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(\beta \evappend \alpha \evappend \Code{Get\ i}, j) \}$&
\end{minted}
which means a list of events $\alpha$ is valid iff $\beta \evappend \alpha \evappend \Code{Get\ i}$ returns a value not equal to $i$ for all $0 \leq i \leq n$.

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\vdash$& gen : &$\nuotxarr{s}{s}{\top} \nuotxarr{n}{int}{\vnu \leq 0} \trcond{\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mptr(\Code{Get\ i}, j)  }\tprod{\nuut{unit}{\top}}$&
\end{minted}

\subsection{Typing Rule}

\newcommand{\purevdash}{\vdash^{\Code{Pure}}}
\newcommand{\trvdash}{\vdash^{\Code{Tr}}}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* TPerform *)
&$\Gamma \vdash v_i : \nuut{b_i}{\phi_i}$&, &$\Gamma \vdash op : \bcol{s}\nuot{s}{\phi_s}\sarr\overline{\bcol{x_i}\nuot{b_i}{\phi_i}}\sarr\bcol{s'}\nuut{evs}{\phi_s}\tprod\nuut{b}{\mpst(s', \nu)}$&
&$\Gamma \vdash$& s : &$\nuut{evs}{\phi_s'}$&, &$\Gamma, \bcol{s}\nuot{s}{\phi_s}, \overline{\bcol{x_i}\nuot{b_i}{\phi_i}} \vdash$& &$\nuut{evs}{\phi_s'} <:_s \nuut{evs}{\phi_s}$&
------------------------------------------------------------------------------------------------
&$\Gamma \vdash$& perform s op v_0 ... v_n : &$\bcol{s'}\nuut{s}{\exists \pi, \phi_s(\pi) \land s \evappend \pi}\tprod\nuut{b}{\mptr(s', \nu)}$&

(* TLetE *)
&$\Gamma \vdash e_1 : \bcol{s}[\pi]\tprod\tau_1$&, &$\Gamma, \bcol{s}[\pi], \bcol{x}\tau_1 \vdash e_2 : \bcol{s'}[\pi_2] \tprod\tau_2$& 
---------------------------------------------------------------
&$\Gamma \vdash$& let (s, x) = e1 in e2 : &$\bcol{s'}[\pi_2] \tprod\tau_2$&
\end{minted}

\subsection{Typing Check}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\phi$&: &$\forall i\ j, 0 \leq i < n \land i \not=j \impl \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j) \land \forall i\ j, n \leq i \impl \mpst(s \evappend \Code{Get\ i}, j) \impl \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j) $&
(* type context; primitives *)
val[@effect] put: &$\nuotxarr{s}{s}{\top} {\bcol{n}\nuot{int}{\top}}\tprod{\bcol{m}\nuot{int}{\top}}\sarr  \bcol{s'}{\nuut{s}{\vnu = \Code{Put (s, (n, m))} }}\tprod{\nuut{unit}{\mptr(s', \vnu)}}$&
val[@effect] get: &$\nuotxarr{s}{s}{\top}\bcol{n}\nuot{int}{\top}\sarr  \bcol{s'}{\nuut{s}{\vnu = \Code{Get (s, n)} }}\tprod{\nuut{int}{\mptr(s', \vnu)}}$&
val (==): &$\bcol{a}\nuot{int}{\top}\sarr \bcol{b}\nuot{int}{\top}\sarr \nuut{int}{\vnu {\iff} a = b}$&
val anynot: &$\bcol{a}\nuot{int}{\top}\sarr \nuut{int}{\vnu \not= a}$&
val (-): &$\bcol{a}\nuot{int}{\top}\sarr \bcol{b}\nuot{int}{\top}\sarr \nuut{int}{\vnu = a - b}$&
\end{minted}

\newcommand{\genrty}{\nuotxarr{s}{s}{\top} \nuotxarr{n}{int}{\vnu \leq 0} \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* type judgement *)
&$\vdash$&
fix (gen: int -> unit) (s0: S) (n: int) =
    let (b: bool) = n == 0 then
    if b then (s0, ()) else
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$: \genrty$&
\end{minted}
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TFix from *)
gen: &$\genrty$& 
&$\vdash$&
fun (s0: S) (n: int) =
    let (b: bool) = n == 0 then
    if b then (s0, ()) else
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$: \genrty$&
\end{minted}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLam from *)
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&
&$\vdash$&
    let (b: bool) = n == 0 then
    if b then (s0, ()) else
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typecheck \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}$&
\end{minted}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TLetE and TApp from *)
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&,
&$\vdash$&
    if b then (s0, ()) else
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typecheck  \nuut{s}{\phi}\tprod{\nuut{unit}{\top}}$&
\end{minted}

The true branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
(* derived by TApp from *)
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&,
&$\vdash$&
    (s0, ())
&$\typeinfer \nuut{s}{\nu = s0}\tprod{\nuut{unit}{\top}}$&
\end{minted}

The false branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&,
&$\vdash$&
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typeinfer ?$&
\end{minted}

The false branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&, &$\bcol{n'}\nuut{int}{\vnu = n - 1}$&,
&$\vdash$&
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typeinfer ?$&
\end{minted}

The false branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&, &$\bcol{n'}\nuut{int}{\vnu = n - 1}$&, &$\bcol{s1}\nuut{s}{\phi[n \mapsto n'][s \mapsto \vnu]}$&, 
&$\vdash$&
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typeinfer ?$&
\end{minted}

The false branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&, &$\bcol{n'}\nuut{int}{\vnu = n - 1}$&, &$\bcol{s1}\nuut{s}{\phi[n \mapsto n'][s \mapsto \vnu]}$&, &$\bcol{m}\nuut{int}{\vnu \not= n}$&,
&$\vdash$&
    perform Put s1 (n, m')
&$\typeinfer \nuut{s}{\vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
\end{minted}

The false branch type inference:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
gen: &$\genrty$&, &$\bcol{s0}\nuot{s}{\top}$&, &$\bcol{n}\nuot{int}{\vnu \leq 0}$&, 
&$\bcol{b}\nuut{bool}{\vnu {\iff} n = 0}$&, &$\bcol{a}\nuut{unit}{b}$&,
&$\vdash$&
    let (n': int) = n - 1 in
    let (s1: S, _) = gen s0 n' in
    let (m: int) = anynot n in
    perform Put s1 (n, m')
&$\typeinfer \nuut{s}{\exists n'\ s1\ m, \neg b \land n' = n - 1 \land m \not=n \land \vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
&$\typeinfer \nuut{s}{\exists n'\ s1\ m, \neg b \land n' = n - 1 \land \phi[n \mapsto n'][s \mapsto s_1 ] \land m \not=n \land \vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
\end{minted}

The type of conditional expression is

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
Merge &$\nuut{s}{b \land \nu = s0}\tprod{\nuut{unit}{\top}}$&
&$\nuut{s}{\exists n'\ s1\ m, \neg b \land n' = n - 1 \land m \not=n \land \vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
&$\typeinfer \nuut{s}{\exists n'\ s1\ m, \neg b \land n' = n - 1 \land \phi[n \mapsto n'][s \mapsto s_1 ] \land m \not=n \land \vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
= 
&$\nuut{s}{b \land \nu = s0 \lor \exists n'\ s1\ m, \neg b \land n' = n - 1 \land \phi[n \mapsto n'][s \mapsto s_1 ] \land m \not=n \land \vnu = s_1 \evappend \Code{Put (n, m)} }\tprod\nuut{unit}{\mpst(s_1 \evappend \Code{Put (n, m)}, \vnu)}$&
\end{minted}
Then

Subtying Query:

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ (\vnu: s), \forall n\ b, n \leq 0 \land b \iff n = 0 \impl$&,
&$\vnu \in \denotation{\nuut{s}{\phi}\tprod{\nuut{unit}{\top}}} \impl$&
&$\vnu \in \denotation{...} $&
\end{minted}
that is
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ (\vnu: s), \forall n, n \geq  \land b \iff n = 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j)) \implies $&
&$s \evappend \vnu \seq s\ \lor $&
&$\exists (\vnu': s), (\forall i\ j, 0 \leq i \leq (n - 1)\land j \not= i {\implies} \mpst(s \evappend \vnu' \evappend \Code{Get\ i}, j)) \land (\forall i\ j, (n - 1) < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j))  \land  $&
&$s \evappend \nu \seq s \evappend \Code{Put (n, m')} \evappend \vnu' $&
\end{minted}

\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\mpst$& (s: state) &$\vnu$& : &$\phi$& =
    match s with
    | s' &$\evappend$& Err -> &$\bot$&
    | s' &$\evappend$& Put (n, m) -> &$\top$&
    | s' &$\evappend$& Get (n) ->
        match s' with
        | s'' &$\evappend$& Err -> &$\bot$&
        | s'' &$\evappend$& Get (n') -> &$\mpst$& (s'' &$\evappend$& Get (n)) &$\vnu$&
        | s'' &$\evappend$& Put (n', m) when n' == n -> &$\vnu = m$&
        | s'' &$\evappend$& Put (_, _) -> &$\mpst$& (s'' &$\evappend$& Get (n)) &$\vnu$&
\end{minted}

Proof by Induction over $\vnu$.
\begin{enumerate}
    \item $\vnu = []$,
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\, \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \Code{Get\ i}, j)) \implies $&
&$s \seq s \lor ...$&
\end{minted}
is valid, because $s \seq s $.
   \item $\vnu = \vnu \evappend Err$,
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \vnu \evappend Err \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \evappend Err \Code{Get\ i}, j)) \implies $&
&$...$&
\end{minted}
Simplified by the definition of $\mpst$:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \bot) \land ...$&
\end{minted}
Exists a counter-example $[i = 0; j = 1]$.
   \item $\vnu = \vnu \evappend \Code{Get\ k}$,
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ k} \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ k} \evappend \Code{Get\ i}, j)) \implies $&
&$s \evappend \vnu \evappend \Code{Get\ k} \seq s \lor $&
&$\exists (\vnu': s), (\forall i\ j, 0 \leq i \leq (n - 1)\land j \not= i {\implies} \mpst(s \evappend \vnu' \evappend \Code{Get\ i}, j)) \land (\forall i\ j, (n - 1) < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j))  \land  $&
&$s \evappend \nu \evappend \Code{Get\ k} \seq s \evappend \Code{Put (n, m')} \evappend \vnu' $&
\end{minted}
Simplified by the definition of $\mpst$ and $\seq$:
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s), \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j)) \implies $&
&$s \evappend \vnu \seq s \lor $&
&$\exists (\vnu': s), (\forall i\ j, 0 \leq i \leq (n - 1)\land j \not= i {\implies} \mpst(s \evappend \vnu' \evappend \Code{Get\ i}, j)) \land (\forall i\ j, (n - 1) < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j))  \land  $&
&$s \evappend \nu \seq s \evappend \Code{Put (n, m')} \evappend \vnu' $&
\end{minted}
proved by induction.
   \item $\vnu = \vnu \evappend \Code{Put\ (p, q)}$.
\begin{minted}[fontsize = \footnotesize, escapeinside=&&]{ocaml}
&$\forall (s:s)\ \forall n, n \geq 0 \impl$&,
&$(\forall i\ j, 0 \leq i \leq n\land j \not= i {\implies} \mpst(s \evappend \vnu \evappend \Code{Put\ (p, q)} \evappend \Code{Get\ i}, j)) \land (\forall i\ j, n < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Put\ (p, q)} \evappend \Code{Get\ i}, j)) \implies $&
&$s \evappend \vnu \evappend \Code{Put\ (p, q)} \seq s \lor $&
&$\exists (\vnu': s), (\forall i\ j, 0 \leq i \leq (n - 1)\land j \not= i {\implies} \mpst(s \evappend \vnu' \evappend \Code{Get\ i}, j)) \land (\forall i\ j, (n - 1) < i \land \mpst(s \evappend \Code{Get\ i}, j) {\implies} \mpst(s \evappend \vnu \evappend \Code{Get\ i}, j))  \land  $&
&$s \evappend \nu \evappend \Code{Put\ (p, q)} \seq s \evappend \Code{Put (n, m')} \evappend \vnu' $&
\end{minted}
\end{enumerate}

==> draft/trace.tex <==
\section{Meta Theory}

\paragraph{How to connect the states and the traces} The users only provide the properties over ``state'', however, our coverage type encodes qualifiers over traces. Here is the key-value store example, and we have the following the properties
\begin{align*}
    &\forall s\ s'\ k\ v, Put (s, (k, v)) = (s', ()) \impl Get(s', k) = v \\
    &\forall s\ s'\ k\ v, Get (s, k) = (s', v) \impl s \simeq s' \\
    &\forall s\ s'\ k_1\ k_2\ v_1, 
    k_1 \not= k_2 \land Put(s, (k_1, v_1)) = (s', ()) \impl Get(s', k_2) = Get(s, k_2)
\end{align*}
where the equality over the abstract state $s$ (i.g., $s \simeq s'$) is defined as ``using the given effects to observe these two states, we cannot distinguish them''. It can be defined (coinductively) as:
\begin{align*}
    s_1 \simeq s_2 \doteq \forall s_1\ s_2\ x\ y_1\ y_2,\forall op \in E, op(s_1, x) = (s_1', y_1) \land op(s_2, x) = (s_2', y_2) \impl s_1' \simeq s_2' \land y_1 = y_2
\end{align*}
where $E$ the set of effects, in the example above, $E$ is $\{Put, Get\}$.

\paragraph{Whats is (the denotation) of the ``abstract states''} Here we should emphasize that how we interpret the ``abstract states'' in the different context.
\begin{enumerate}
    \item The equality over the ``abstract states'' derives the equality over traces that can help us to simplify the redundant traces.
    \item The ``abstract states'' works naturally with the operators (e.g., $\S{Put}$ and $\S{Get}$) just \emph{like} they are the hidden states in the implementation (here we call it ``hidden states'').
    \item In general, ``abstract states'' is not (and not need to be) the hidden states in the implementation of the abstract type libraries. For example, $\S{Put}(a, 2); \S{Put}(b, 3);$ should generate the same hidden states with $\S{Put}(b, 3); \S{Put}(a, 2);$ with respect to the semantics of the key-value store. However, the corresponding ``abstract states'' can and could not be the same. Currently, we believes they are two difference traces, thus they should ends with the different ``abstract states''. On the other hand, if we add the commute property of $\S{Put}$:
    \begin{align*}
    \forall s_1\ s_2\ s_3\ s_2'\ s_3\ k_1\ v_1\ k_2\ v_2,& k_1 \not= k_2 \land\\ 
    &\S{Put}(s_1, (k_1, v_1)) = (s_2, ()) \land \S{Put}(s_2, (k_2, v_2)) = (s_3, ()) \land \\
    &\S{Put}(s_1, (k_2, v_2)) = (s_2', ()) \land \S{Put}(s_2', (k_1, v_1)) = (s_3', ()) \implies s_3 \simeq s_3'
    \end{align*}
    Then these two ``abstract states'' can be equal, and the permutation of $\S{Put}$ will generate the equivalent traces.
\end{enumerate}
In summary, the ``abstract states'' is an more fine-grained than the ``hidden states'', which is sensitive to the traces. In other words, it is an representation of the ``hidden states'' from the perspective of the traces. I get kind of inspired by the Yoneda Lemma, the proper representation of the ``hidden states'' in terms of traces is exactly ``how the hidden states works with the traces''. In fact, the only meaningful operation in the traces is the concatenation, thus I believe the ``abstract states'' is actually a function $\lambda tr. \Code{prefix}\listconcat tr$, or simply say, it a prefix (another understanding is the history) of \emph{valid} trace.

\begin{definition}[Event and Trace] An event is a 3-tuple $(op, args, ret)$, where $op$ is the operator (e.g., $\S{Put}$), $args$ and $ret$ is the arguments and return values of the operator. The trace is a (infinite) sequence of events.
\end{definition}

\begin{definition}[Abstract State] Abstract state is an abstraction of the prefix of traces. Precisely, it consists of $(Tr^{\checkmark}, S, \pi, \simeq)$ where $Tr^{\checkmark}$ indicates the a set of finite length traces, $S$ is the domain of the abstract states, $\pi{:} Tr^{\checkmark}{\to}S$ is mapping maps traces to abstract states, and $\simeq$ is the equivalent relation over the states. Moreover, $\simeq$ can also derive the equivalent relation over traces:
\begin{align*}
    tr_1 = tr_2 \doteq \pi(tr_1) \simeq\pi(tr_2)
\end{align*}
\end{definition}
Notice that, this definition is consistent with our (coinductively) definition above:
\begin{align*}
    s_1 \simeq s_2 \doteq \forall s_1\ s_2\ x\ y_1\ y_2,\forall op \in E, op(s_1, x) = (s_1', y_1) \land op(s_2, x) = (s_2', y_2) \impl s_1' \simeq s_2' \land y_1 = y_2
\end{align*}
because for the prefix $p_1$ and $p_2$ in $\in Tr^{\checkmark}$
\begin{align*}
    \forall x\ y_1\ y_2,\forall op \in E, p_1 \listconcat [(op, x, y_1)] = p_2 \listconcat [(op, x, y_2)] \iff p_1 = p_2 \land y_1 = y_2
\end{align*}

\begin{example} Consider the property 
\begin{align*}
    \forall s\ s'\ k\ v, \S{Put} (s, (k, v)) = (s', ()) \impl \S{Get}(s', k) = v
\end{align*}
where we treat $s$ and $s'$ as two prefix of traces, then it says that
\begin{align*}
    \forall p_1\ p_2 \in Tr^{\checkmark}, \forall k\ v, p_2 = p_1 \listconcat [(\S{Put}, (k, v), ())] \implies (p_2 \listconcat (\S{Get}, k, v') \in Tr^{\checkmark} \iff v = v')
\end{align*}
which describes the constraint over the prefix set $Tr^{\checkmark}$. 
\end{example}

\begin{example} Consider the property 
\begin{align*}
    \forall s\ s'\ k\ v, Get (s, k) = (s', v) \impl s \simeq s'
\end{align*}
where we treat $s$ and $s'$ as two prefix of traces, then it says that
\begin{align*}
    \forall p\ p' \in Tr^{\checkmark}, \forall k\ v, p' = p \listconcat [(\S{Get}, k, v)] \impl
    \pi (p) \simeq \pi (p') 
\end{align*}
which describes the constraint over the equivalent relation $\simeq$. 
\end{example}

\begin{example} The user expect to reach a state $s$:
\begin{align*}
    \forall k_1\ k_2\ v_1\ v_2, k_1 \not= k_2 \land 
    Get(s, k_1) = (\_, v_1) \land Get(s, k_2) = (\_, v_2)  \implies v_1 \not= v_2
\end{align*}
which indicates that the store doesn't contain duplicate values.
If we treat $s$ as the prefix of traces, then it says that we need to enumerate prefix $p$ such that
\begin{align*}
    &p \in Tr^{\checkmark} \land \\
    &(\forall k_1\ k_2\ v_1\ v_2, k_1 \not= k_2 \land p \listconcat [(\S{Get}, k_1, v_1)] \in Tr^{\checkmark} \land p \listconcat [(\S{Get}, k_2, v_2)] \in Tr^{\checkmark} \impl v_1 \not= v_2)
\end{align*}
where our goal is to generate all different valid prefix up to the equivalent relation $\simeq$. 
\end{example}

During the verification, the predicate $\checkmark: Tr{\to}\mathbf{B}$ and relation $\simeq$ are uninterpreted functions.

\paragraph{How it works with the method predicates?} Consider the example of the locks:
\begin{align*}
    \forall s\ s'\ l, Lock (s, l) = (s', ()) \iff unlocked (s, l) \land locked(s', l)
\end{align*}
Here the predicate $unlocked (\_, l)$ will be translate directly into a predicate over traces. The above property means that
\begin{align*}
    \forall p \in Tr^{\checkmark}, p \listconcat [(\S{Lock}, l, ())] \in Tr^{\checkmark} \iff unlocked (p, l) \land unlocked (p \listconcat [(\S{Lock}, l, ())], l)
\end{align*}
Assume the initial ``hidden state'' let the lock $l_1$ is available to be locked. Then we can say
\begin{align*}
    &\models unlocked([], l_1) \\
    &\models unlocked([(\S{Lock}, l_1, ()); (\S{Unlock}, l_1, ())], l_1) \\
    &\models unlocked([(\S{Lock}, l_2, ()), l_1])
\end{align*}
We want to reach a state $s$ such that
\begin{align*}
    \forall l, \neg locked (s, l)
\end{align*}
where all locks are uninitialized or unlocked. Notice that, we doesn't say $Lock l; Unlock l$ is equal to do nothing, thus we need to enumerate all possible traces. This coverage property can be describe as the following type:
\begin{align*}
    \nuut{tr (locks)}{\forall \ev \in \nu, \ev.op = \S{Lock} \land \ev.arg = l \impl \exists \ev', \ev \rightharpoonup^{\nu} \ev' \land \ev'.op = \S{Unlock} \land \ev'.arg = l }
\end{align*}
where $\ev \rightharpoonup^{\nu} \ev'$ indicates that the event $\ev'$ appears after $\ev$ in the trace $\nu$. It can be translate into our new interpretation:
\begin{align*}
    &\nuut{tr (locks)}{\forall p, p \listconcat [(\S{Lock}, l, ())] \sqsubset \nu \impl \exists p', p \sqsubseteq p' \listconcat [(\S{Unlock}, l, ())] \sqsubset \nu }
\end{align*}
where $p \sqsubset \nu$ indicates that $p$ is a true prefix of the trace $\nu$. We unify the operation $\ev \rightharpoonup^{\nu} \ev'$ into $p \sqsubset p' \sqsubset \nu$ and $\ev ;^{\nu} \ev'$ into $p \listconcat [ev; ev'] \sqsubset \nu$.

\begin{example} Consider the maze example, we expect to generate paths in the maze that never reach to the same position. The corresponding type is
\begin{align*}
    &\nuut{tr (maze)}{ \phi } \\
    \phi \equiv& \forall p_1\ p_2\ x_1\ y_1\ x_2\ y_2, p_1 \sqsubset \nu \land p_2 \sqsubset \nu \land \\ 
    &posx(p_1, x_1) \land posy(p_1, y_1) \land posx(p_2, x_2) \land posy(p_2, y_2) \impl \neg (x_1 = x_2 \land y_1 = y_2)
\end{align*}
where $p \sqsubset \nu$ indicates that $p$ is a true prefix of the trace $\nu$.
\end{example}

\paragraph{Compare with the typestate} For a state machine, the typestate would add a lot of constraint (specifications of the fields in the objects, or, in general, specifications of the hidden states) to the states in the state machine. Here we treat the hidden states are truly hidden and add constraint to the traces ends up with this hidden states, that is the prefix, which is the only thing we can obverse.

\paragraph{Logic we use} The ${::}$, $\listconcat{}$ and $\sqsubset$ should be the primitives in this logic, I still want the properties and the method predicates has an inductive interpretation, otherwise I think it is kind of hard to prove.

==> draft/type-st-tr.tex <==
\section{Language}

\begin{figure}[t!]
{\small
    \begin{alignat*}{2}
    \text{\textbf{Variables }}& \quad &\quad& x, f, u, ... \\
    \text{\textbf{Effect Operators}}& \quad &\theta ::= \quad & \in \textit{string} \\
    \text{\textbf{Base Types}}& \quad & b  ::= \quad &  unit ~|~ bool ~|~ nat ~|~ int ~|~  b\ list ~|~ b\ tree ~|~ \ldots \\
    \text{\textbf{Basic Types}}& \quad & t  ::= \quad & b ~|~ t\, {\shortrightarrow}\,t \\
    \text{\textbf{Method Predicates }}& \quad & mp ::= \quad & \I{emp} ~|~ \I{hd} ~|~ \I{mem} ~|~ ...\\
    \text{\textbf{Literals }}& \quad & l ::= \quad & c ~|~ x \\
    \text{\textbf{Propositions}}& \quad & \phi ::= \quad &  l ~|~ \bot ~|~ \top_b  ~|~ op(\overline{l}) ~|~ mp(\overline{x}) ~|~ \neg \phi ~|~ \phi \land \phi ~|~ \phi \lor \phi ~|~ \phi \impl \phi ~|~  \forall u{:}b.\; \phi ~|~ \exists u{:}b.\; \phi \\
    \text{\textbf{Trace Language}}& \quad &tr ::= \quad &  \emptyset ~|~ \theta(\overline{c}) ~|~ \cdot ~|~ tr {||} tr ~|~ tr {;} tr ~|~ \nuut{\textit{b}}{\phi} ~|~ C(\nuot{\textit{b}}{\phi}, tr)\\
    \text{\textbf{Refinement Types}}& \quad &\tau  ::= \quad &  \nuut{\textit{b}}{\phi} ~|~ \nuot{\textit{b}}{\phi} ~|~  x{:}\tau{\shortrightarrow}\tau ~|~ \langle tr \rangle ~|~ x{:}\nuot{\textit{b}}{\phi}{\Rightarrow}\tau  ~|~  \tau \rhd \tau \\
    \text{\textbf{Type Contexts}}& \quad &\Gamma ::= \quad & \emptyset ~|~ \Gamma, x{:}\tau
  \end{alignat*}
}
    \caption{\langname{} syntax.}\label{fig:syntax}
\end{figure}

\paragraph{Consideration} There are several considerations to build the new type system.
\begin{enumerate}
    \item The new adding types should be decomposed from the pure refinement types since there is no traces or states in the source code.
    \item The trace type and the pure refinement type are related to each others. Of course, the new preformed event is dependents on the variables in the type context. On the other hand, the return value of an effectful operator may also depends on the traces (e.g., $\S{get}$, $\S{checkin}$). This ``related'' implies that we should add bindings for both trace types and the pure refinement types in the type context, and they can be arranged with arbitrary order.
    \item The typing rule for ``perform'' should append the event $\theta(\overline{c})$ to the trace directly. The operation happens frequently, and the trace is immutable and incremental, we consider to build a language of traces (like regular expression, but simpler).
    \item For the users to write the specification easily, they should be able to describe the initial states and terminal states easily (implies that we should have state types). For example:
    \begin{align*}
        \vdash \S{unlock\_gen} : \textit{unit}{\shortrightarrow} s{:}\nuot{\textit{bool}}{\top}{\Rightarrow}\nuut{\textit{bool}}{\neg \vnu} \rhd \nuut{\textit{unit}}{\top}
    \end{align*}
    The $\S{unlock\_gen}\ ()$ is a generator that enumerates all possible traces that ends up with ``unlocked'' state from arbitrary states, where the states are represented as a boolean to indicate if the lock is locked.
    \begin{align*}
    &\vdash e : s{:}\nuot{\textit{st}}{p}{\Rightarrow}\nuut{\textit{st}}{q} \rhd \nuut{\textit{b}}{\phi} \\
    &\forall tr\forall s, p(s) \land A(tr) = s \implies \exists tr'\exists s' \exists v, q(s, s') \land A(tr') = s' \land \phi(s, v) \land (<tr, e> \hookrightarrow^* <tr', v>)
    \end{align*}
\end{enumerate}

==> pldi2024/desugar.tex <==
\begin{figure}[t!]
\footnotesize{
{\small\begin{flalign*}
 &\text{\textbf{Desugar}} & \fbox{$\dedep{\tau} \in \mathcal{P}(\tau)$}
\end{flalign*}}
\begin{align*}
    &\dedep{ \rawdat{A}{s}{B} } &&\doteq \{ \rawdat{A}{s}{B} \} \text{ when } B = \topA \text{ or } \botA \text{ or } \epsilon \text{ or } \evop{\effop{}}{\overline{x_i} }{\phi} \text{ or } \evret{ t }
    \\ &\dedep{ \rawdat{A}{s}{X \in B} } &&\doteq \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B} }} 
    \{ \rawdat{A' \landA B'}{s}{\topA}, \rawdat{A' \landA \negA B'}{s}{\botA} \}
    \\ &\dedep{ \rawdat{A}{s}{\alpha \in B} } &&\doteq \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B} }}
    \{ \rawdat{A'}{s}{\alpha \in B'} \}
    \\ &\dedep{ \rawdat{A}{s}{\negA B} } &&\doteq \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B} }} 
    \{ \rawdat{A'}{s}{\negA B'} \}
    \\ &\dedep{ \rawdat{A}{s}{B^*} } &&\doteq \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B} }} 
    \{ \rawdat{A'}{s}{{B'}^*} \}
    \\ &\dedep{ \rawdat{A}{s}{B_1;B_2} } &&\doteq \bigcup_{\rawdat{A_1'}{s}{B_1'} \in \dedep{ \rawdat{A}{s}{B_1} }} \bigcup_{\rawdat{A_2'}{s}{B_2'} \in \dedep{ \rawdat{A}{s}{B_2} }}
    \{ \rawdat{A_1' \landA A_2'}{s}{B_1';B_2'} \}
    \\ &\dedep{ \rawdat{A}{s}{B_1 \landA B_2} } &&\doteq \bigcup_{\rawdat{A_1'}{s}{B_1'} \in \dedep{ \rawdat{A}{s}{B_1} }} \bigcup_{\rawdat{A_2'}{s}{B_2'} \in \dedep{ \rawdat{A}{s}{B_2} }}
    \{ \rawdat{A_1' \landA A_2'}{s}{B_1' \landA B_2'} \}
    \\ &\dedep{ \rawdat{A}{s}{B_1 \lorA B_2} } &&\doteq \bigcup_{\rawdat{A_1'}{s}{B_1'} \in \dedep{ \rawdat{A}{s}{B_1} }} \bigcup_{\rawdat{A_2'}{s}{B_2'} \in \dedep{ \rawdat{A}{s}{B_2} }}
    \{ \rawdat{A_1' \landA A_2'}{s}{B_1' \lorA B_2'} \}
\end{align*}
}
    \caption{\langname{} refinement types desugar.}\label{fig:type-denotation}
\end{figure}

\begin{theorem}[The lemma of the codomain of de-dependent function]\label{lemma:dedep-pre}
{\small\begin{align*}
&\langATr{A} = \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B}  }} \langATr{A'}
\end{align*}}
\end{theorem}

\begin{theorem}[The lemma of the domain of de-dependent function]\label{lemma:dedep-post}
{\small\begin{align*}
\forall \alpha. \alpha \in \langATr{A} \implA \exists \rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}}. \alpha \in \langATr{A'} \landA \langATr{B[X\mapsto \alpha]} = \langATr{B'}
\end{align*}}
\end{theorem}
% \begin{definition}[The lemma of de-dependent function]
% {\small\begin{align*}
% % &\langATr{A} = \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{ \rawdat{A}{s}{B}  }} \langATr{A'}
% % \\
% &\forall \alpha. \alpha \in \langATr{A} \implA \exists \rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}}. \alpha \in \langATr{A'} \landA \langATr{B[X\mapsto \alpha]} = \langATr{B'} \tag{Lemma 1}
% \\&\forall \rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}}. \forall \alpha. \alpha \in \langATr{A'} \implA \langATr{B[X\mapsto \alpha]} = \langATr{B'} \tag{Lemma 2}
% \end{align*}}
% \end{definition}
\paragraph{Proof} For the first lemma, we have
\begin{enumerate}[label=Case]
\item \textsc{Inclusion Check ``$\rawdat{A}{s}{X \in B}$''}:
For all $\alpha \in \langATr{ A }$, according to Lemma~\ref{lemma:dedep-pre}, there exists $A'$ and $B'$ where
{\footnotesize\begin{align*}
\rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}} \landA \alpha \in \langATr{ A' } \landA \langATr{B[X\mapsto \alpha]} = \langATr{B'}
\end{align*}}\noindent
Then, if $\alpha \in \langATr{B' }$, then $\alpha \in \langATr{B[X\mapsto \alpha]}$. There exists a type $\rawdat{A' \landA B'}{s}{\topA} \in \dedep{ \rawdat{A}{s}{X \in B} }$. Moreover
{\footnotesize\begin{align*}
&\alpha \in \langATr{ A' \landA B' } \text{ since } \alpha \in \langATr{ B' } \text{ and } \alpha \in \langATr{A' }
\\&\langATr{(X \in B)[X\mapsto \alpha]} = \langATr{\alpha \in B[X\mapsto \alpha]} = \langATr{\topA} \text{ since } \alpha \in \langATr{B[X\mapsto \alpha]}
\end{align*}}\noindent
Similarly, if $\alpha \not\in \langATr{B' }$, then $\alpha \in \langATr{\negA B' }$. Thus, $\alpha \not\in \langATr{B[X\mapsto \alpha]}$. There exists a type $\rawdat{A' \landA \negA B'}{s}{\botA} \in \dedep{ \rawdat{A}{s}{X \in B} }$. Moreover
{\footnotesize\begin{align*}
&\alpha \in \langATr{ A' \landA \negA B' } \text{ since } \alpha \in \langATr{\negA B' } \text{ and } \alpha \in \langATr{A' }
\\&\langATr{(X \in B)[X\mapsto \alpha]} = \langATr{\alpha \in B[X\mapsto \alpha]} = \langATr{\botA} \text{ since } \alpha \not\in \langATr{B[X\mapsto \alpha]}
\end{align*}}
\item \textsc{Negation ``$\rawdat{A}{s}{\negA B}$''}:
For all $\alpha \in \langATr{ A }$, according to Lemma~\ref{lemma:dedep-pre}, there exists $A'$ and $B'$ where
{\footnotesize\begin{align*}
\rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}} \landA \alpha \in \langATr{ A' } \landA \langATr{B[X\mapsto \alpha]} = \langATr{B'}
\end{align*}}\noindent
There exists a type $\rawdat{A'}{s}{\negA B'} \in \dedep{ \rawdat{A}{s}{\negA B} }$. Moreover
{\footnotesize\begin{align*}
&\alpha \in \langATr{ A'}
\\&\langATr{(\negA B)[X\mapsto \alpha]} = Tr \setminus \langATr{B[X\mapsto \alpha]} = Tr \setminus \langATr{B'} = \langATr{\negA B'}
\end{align*}}\noindent
\item \textsc{Sequence ``$\rawdat{A}{s}{B_1B_2}$''}:
For all $\alpha \in \langATr{ A }$, according to Lemma~\ref{lemma:dedep-pre}, there exists $A'$ and $B'$ where
{\footnotesize\begin{align*}
&\rawdat{A_1'}{s}{B_1'} \in \dedep{\rawdat{A}{s}{B_1}} \landA \alpha \in \langATr{ A_1' } \landA \langATr{B_1[X\mapsto \alpha]} = \langATr{B_1'}
\\&\rawdat{A_2'}{s}{B_2'} \in \dedep{\rawdat{A}{s}{B_2}} \landA \alpha \in \langATr{ A_2' } \landA \langATr{B_2[X\mapsto \alpha]} = \langATr{B_2'}
\end{align*}}\noindent
There exists a type $\rawdat{(A_1' \landA A_2')}{s}{B_1'B_2'} \in \dedep{ \rawdat{A}{s}{B_1B_2} }$. Moreover
{\footnotesize\begin{align*}
&\alpha \in \langATr{ A_1' \landA A_2'}
\\&\langATr{(B_1B_2)[X\mapsto \alpha]} = \langATr{(B_1[X\mapsto \alpha])(B_2[X\mapsto \alpha])} 
\\=&\{\beta_1 \listconcat \beta_2 ~|~ \beta_1 \in \langATr{B_1[X\mapsto \alpha]}, \beta_2 \in \langATr{B_2[X\mapsto \alpha]} \}
\\=&\{\beta_1 \listconcat \beta_2 ~|~ \beta_1 \in \langATr{B_1'}, \beta_2 \in \langATr{B_2'} \}
\\=&\langATr{B_1'B_2'} 
\end{align*}}\noindent
\item \textsc{Union ``$\rawdat{A}{s}{B_1 \lorA B_2}$''}:
For all $\alpha \in \langATr{ A }$, according to Lemma~\ref{lemma:dedep-pre}, there exists $A'$ and $B'$ where
{\footnotesize\begin{align*}
&\rawdat{A_1'}{s}{B_1'} \in \dedep{\rawdat{A}{s}{B_1}} \landA \alpha \in \langATr{ A_1' } \landA \langATr{B_1[X\mapsto \alpha]} = \langATr{B_1'}
\\&\rawdat{A_2'}{s}{B_2'} \in \dedep{\rawdat{A}{s}{B_2}} \landA \alpha \in \langATr{ A_2' } \landA \langATr{B_2[X\mapsto \alpha]} = \langATr{B_2'}
\end{align*}}\noindent
There exists a type $\rawdat{(A_1' \landA A_2')}{s}{B_1' \lorA B_2'} \in \dedep{ \rawdat{A}{s}{B_1 \lorA B_2} }$. Moreover
{\footnotesize\begin{align*}
&\alpha \in \langATr{ A_1' \landA A_2'}
\\&\langATr{(B_1 \lorA B_2)[X\mapsto \alpha]} 
= \langATr{B_1[X\mapsto \alpha] \lorA B_2[X\mapsto \alpha]}
= \langATr{B_1[X\mapsto \alpha]} \lorA \langATr{B_2[X\mapsto \alpha]} 
\\=& \langATr{B_1'} \lorA \langATr{B_2'} = \langATr{B_1' \lorA B_2'} 
\end{align*}}\noindent
\end{enumerate}

\begin{theorem}[soundness of de-dependent function]
{\small\begin{align*}
&\denotation{\rawdat{A}{s}{B}} = \bigcup_{\rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}}} \denotation{\rawdat{A'}{s}{B'}}
\end{align*}}
\end{theorem}

\paragraph{Proof}
{\small\begin{align*}
&\denotation{\rawdat{A}{s}{B}} =
\\=& \{e ~|~ \emptyset \basicvdash e : s \landA \forall \alpha \in \langATr{A}, \forall\alpha'\ v. \msteptr{\alpha}{e}{\alpha'}{v} \implA \alpha \listconcat \alpha' \listconcat [\S{ret}(v)] \in \langATr{B[X\mapsto \alpha]} \}
\end{align*}}\noindent
Then for all term $e$ and for $\alpha \in \langATr{A}$,
According to the Lemma~\ref{lemma:dedep-pre}, there exists $\rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}}$ where
{\footnotesize\begin{align*}
\rawdat{A'}{s}{B'} \in \dedep{\rawdat{A}{s}{B}} \landA \alpha \in \langATr{ A' } \landA \langATr{B[X\mapsto \alpha]} = \langATr{B'}
\end{align*}}\noindent
Then $\alpha \listconcat \alpha' \listconcat [\S{ret}(v)] \in \langATr{B'}$, thus $e\in \denotation{\rawdat{A'}{s}{B'}}$.

\paragraph{Auxiliary Type Judgement} $\Gamma \vdash^{\Code{incr}} e : \rawdat{A}{s}{B} \equiv \Gamma \vdash e : \rawdat{A}{s}{AB}$.


==> pldi2024/new-tech.tex <==
\section{New Typing}

\begin{figure}[t!]
{\small
\begin{flalign*}
 &\text{\textbf{Type Syntax}} &
\end{flalign*}
\begin{alignat*}{2}
    \text{\textbf{Base Types}}& \quad & b  ::= \quad &  \Code{unit} ~|~ \Code{bool} ~|~ \Code{nat} ~|~ \Code{int} ~|~ b\, \Code{option}
    \\ \text{\textbf{Basic Types}}& \quad & s  ::= \quad & b ~|~ s \sarr s
    \\ \text{\textbf{Literals}}& \quad & l ::= \quad & c ~|~ x ~|~ \primop\ \overline{l}
    \\ \text{\textbf{Qualifiers}}& \quad & \phi ::= \quad & l ~|~ \bot ~|~ \top  ~|~ \neg \phi ~|~ \phi \land \phi ~|~ \phi \lor \phi ~|~ \phi \impl \phi ~|~ \forall x{:}b.\, \phi
    \\ \text{\textbf{Refinement Types}}& \quad &t ::= \quad & \nuot{\textit{b}}{\phi} ~|~ x{:}t\sarr\tau
    % ~|~  x{:}b\ghostarr\tau
    % \\ \text{\textbf{Symbolic Event}}& \quad &\pi ::= \quad & \evop{\effop{}}{\overline{x}}{\phi} ~|~ \evret{t }
    \\ \text{\textbf{Symbolic Automata }}& \quad &A,B  ::= \quad & \evop{\effop{}}{\overline{x}}{\phi} ~|~ \evret{t} ~|~ \emptyset ~|~ \empA ~|~ AA ~|~ A \lorA A ~|~ A \setminus A ~|~ A^*
    % ~|~ \compA{A}
    \\ \text{\textbf{Hoare Automata Types}}& \quad &\tau  ::= \quad & \efftp{A}{A}{\text{$s$}}
    \\\text{\textbf{Type Contexts}}& \quad &\Gamma ::= \quad & \emptyset ~|~ x{:}t, \Gamma
  \end{alignat*}
\begin{flalign*}
 &\text{\textbf{Type Aliases}} &
\end{flalign*}
\begin{alignat*}{4}
    \evop{\effop\, \overline{\text{$v_i$}}}{\overline{x}}{\phi} &\doteq \evop{\effop}{\overline{y_i}\ \overline{x}}{\bigwedge \overline{y_i = v_i} \land \phi} \quad&
    \evoponly{\effop} &\doteq \evop{\effop}{\overline{x}}{\top} \quad&
    b &\doteq \rawnuot{b}{\top}
    \quad&
    \anyA &\doteq \lorA \overline{\evoponly{\effop}}
    \\
    \evop{\setminus\, \effop}{\overline{x}}{\phi} &\doteq \anyA \setminus \evop{\effop}{\overline{x}}{\phi}
    % \evop{ret}{\vnu{:}b}{\phi} &\doteq \evret{\rawnuot{b}{\phi}}
    \quad&
   \efftp{A}{t }{\text{$s$}}  &\doteq \efftp{A}{\evret{t}}{\text{$s$}} \quad&
   t &\doteq \efftp{\anyA^*}{\text{$t$}} {\eraserf{\mathit{t}}}
\end{alignat*}
}
    \caption{\langname{} types.}\label{fig:type-syntax}
\end{figure}

==> pldi2024/rebuttal.tex <==
We thank the reviewers for their detailed comments and suggestions.

# Summary of Proposed Changes:
--------------------------------

We propose to implement the following changes in our revision:

1. We will elaborate the discussion in our evaluation to include
additional details about the properties that are checked in our
benchmarks (Reviewers A, C, and D), and will additionally provide
qualitative measures of complexity for the representation invariants
we consider (Reviewer D). We will also add research questions to focus
attention on specific insights gleaned from the experiments (Reviewers
A and D).

2. We will provide additional algorithm details, especially regarding
the bidirectional type system (Reviewer D); properties needed to
perform SFA inclusion checks needed by, e.g., the SubAutomata and
WFHoare rules (Reviewers B and D); and, discussion on the efficiency
and termination conditions of our typing algorithm (Reviewer B).

3. We will incorporate the suggestions made by the referees with
respect to related work and provide a detailed comparison with our
approach.  As noted in Reviewer A's review, the cited prior work
differs significantly from HATs with respect to (a) setting
(verification in the presence of stateful opaque libraries with hidden
state), (b) the degree of automation supported, and (c) the kind and
form of specifications supported.

4. We will expand our discussion of future work as suggested by the
reviewers, i.e., the feasibility of using HATs to address general
verification questions beyond representation invariants (Reviewer B);
verifying quantitative properties and infinite traces (Reviewer D);
and verifying other effectful (instead of merely stateful) libraries
(Reviewer A).

5. We will fix all typos and refine the paper's presentation following
the suggestions from all reviewers.

# Detailed Response:
--------------------------------
# All Reviewers:

## Benchmarks and Checked Properties (All Reviewers):
--------------------------------

The table shown below gives a brief overview of the kinds of
properties checked by our benchmarks. Besides the benchmarks already
discussed in the paper, the stack and queue ADTs require a low-level
safety guarantee - for example, that the underlying linked list
implementation used to implement them is not circular. The set
datatype has a no-duplicate elements property; this ADT is also used
as a library in other benchmarks (e.g., MinSet). The connected graph
benchmark requires that any two nodes are connected, requiring the
need for ghost variables.

| ADT | Safety Property | Library |  Representation Invariant |
|---|---|---|---|
| Stack | Cells in stacks are unique. | LinkedList | No circular linked list. |
|  |  | KVStore | The addresses that store elements are unique. |
| Queue | Cells in queue are unique. | LinkedList | No circular linked list. |
|  |  | Graph | No self-loop in the graph, the degree of nodes in graph are at most 1.  |
| Set | No duplicate elements. | Tree | The tree ADT implements a binary search tree. |
|  |  | KVStore | Every key is associated with a distinct value. |
| Heap | Min-heap property. | Tree | The value of the parent node in the tree is less than the value of  its children nodes. |
|  |  | LinkedList | No circular linked list, and the elements are sorted. |
| MinSet | No duplicate elements, the recorded element is minimal. | Set | The recorded element is less than all inserted elements in the set and has been inserted before. |
|  |  | KVStore | The recorded element is less than all elements put in the store and has been put before. |
| LazySet | No duplicate elements. | Tree | The tree ADT implements a binary search tree. |
|  |  | Set | Never insert the same element twice. |
|  |  | KVStore | Every key is associated with a distinct value. |
| FileSystem | Policy of Unix-like file system paths. | Tree | The parent node must store a path that is a prefix of its children nodes; a non-root parent node stores directories. |
|  |  | KVStore | Any path that is stored as a key in the key-value store (other than the root path) must also have its parent stored as a non-deleted directory in the store. |
| DFA | Determinism of finite automata. | KVStore | All stored transitions are represented as tuples (start, char, end), and any starting state can have at most have one transition over a character. |
|  |  | Graph | Two nodes (indicating states in an FA) can have at most one edge, which is labeled with a character. |
| ConnectedGraph | Connectivity. | Set | The set stores unique pairs (fst, snd), and only elements that have both in and out edges are treated as a value node in the graph. |
|  |  | Graph | All nodes in the graph are connected. |

# Reviewer A:

## State, effects, or simply abstraction?

Currently our implementation focuses on verifying stateful libraries.
While there is no theoretical reason why our type system cannot verify
other kinds of effects, we leave the exploration of this question as
part of future work.

As noted by the reviewer, HATs can constrain traces that record
arbitrary operations (even those that are not effectful), although our
current focus only considers its role in verifying stateful
representation invariants.

# Reviewer B:

## SFA inclusion check

The SFA inclusion check used by the rules SubAutomata, WFHoare, etc.
is similar to the standard SFAs algorithm [7, 12], which is decidable.
More precisely, our SFA inclusion check is decidable (line 751), as
long as the satisfiability check for minterms is decidable. Moreover,
to guarantee the decidability of this check, we limit our qualifiers
to be Effectively Propositional Logic (EPR), as is typical in most
refinement type systems. The full details of our SFA inclusion
algorithm are given in our supplemental materials (Section F,
Algorithm 1). As noted in the changes proposed above, we plan to
highlight the termination guarantees of our algorithm in Section 5 and
discuss its efficiency in Section 6 in the revision.

## Ghost variables inference

We use ghost variables in a fairly limited way, which ameliorates the
problem of automatically inferring them. Ghost variables only appear
in SFAs (instead of in arbitrary refinement types), such that they
only impact our SFA inclusion checks. This is an (implicit)
consequence of the algorithmic typing rules (ChkEOpApp in Fig. 8 and
ChkApp in Fig. 16 in the appendix): the second line in the ChkApp rule
(`Γ ⊢ v_2 ⇐ t_y`), for example, only holds when no free ghost
variables appear in the parameter type `t_y`. We will clarify this
restriction in our revision.

This restriction allows us to perform ghost variable inference in a
similar way to how standard SFA algorithms handle minterms: the
possible instantiations of ghost variables can be reduced to a set of
finite equivalence classes, which avoids the need for complicated Horn
constraint solving, as employed in prior work. The details of how we
infer ghost variables can be found in our supplemental material
(Section F, Algorithm 2).


# Reviewer C:

## General verification besides representation invariants

As we briefly mention on lines 974 - 978, it is certainly conceivable
to use HATs to verify a larger class of safety properties in addition to
representation invariants, leveraging e.g., richer automata classes,
or more expressive effectful abstractions (e.g., algebraic effects).
We leave an investigation of these extensions as a topic for future
work.

# Reviewer D:

## L181-182 (deleteChildren)

The code of deleteChildren can be found in our supplemental material
(line 1749) via the anonymous link
(https://anonymous.4open.science/r/HATs-0C76/data/ri/FileSystem_KVStore/deleteChildren.ml);
we also post it below. It is an internal function that is only used
when deleting a directory from the file system. For the implementation
of this function, the getChildren operation is not necessary; it just
recursively calls ``getChild" to delete all children from given
directory.

```
let rec deleteChildren (path : Path.t) : unit =
  if not (exists path) then ()
  else
    let (bytes : Bytes.t) = get path in
    if hasChild bytes then (
      let (child_path : Path.t) = getChild bytes in
      let (res' : bool) = delete child_path in
      deleteChildren path;
      ())
    else ()
```

## L216-217 (diverging programs)

As is standard in refinement type systems, Marple is silent on the
behavior of diverging programs (lines 703-706). It would be
straightforward to augment our type system with termination checks
(based on a well-founded relation on decreasing arguments) similar to
how this issue is handled in e.g., LiquidHaskell.

## L281-282 (different precondition and postcondition)

Since we focus on the verification of representation invariants, it is
natural for the pre and post-conditions of client code to be the same;
moreover, all interfaces of an effectful library share the same SFA
corresponding to the representation invariant. That said, the reviewer
is correct that the semantics of HATs does not mandate this
constraint: the HAT types of various effectful library operators
(e.g., line 449 - 453) are likely to have different pre- and
post-condition automata, for example. Exploring applications of HATs
to more general verification problems is an interesting direction for
future work.

## L284-285 (understanding the role of ghost variable)

The ``p" here can be understand as a universally quantified variable
that helps HATs constrain all paths stored or that should be stored in
the file system. Note that if ``p" in the invariant on line 240 is not
an arbitrary path, it simply suffices to set ``p" as the root path
(where □⟨isRoot(p)⟩ holds).

## L678-679 (explanation of fundamental theorem)

The fundamental theorem states that the trace of effects produced
during the computation of an effectful term are consistent with its
corresponding HAT, assuming the built-in operator type context is
well-formed. We will add a description of the theorem in english in
our revision.


==> pldi2024/related.tex <==
One complaint I have about this paper is that it fails to mention many other related works. For the start, the paper mentions the Dijkstra monad and F
⋆
⋆ in l.89, but it fails to mention the subsequent work that focuses more on effects. It might be useful to check the following papers:

"SteelCore: An Extensible Concurrent Separation Logic for Effectful Dependently Typed Programs"
"Steel: Proof-oriented Programming in a Dependently Typed Concurrent Separation Logic"
Another line of work that is closely related to this paper is the interaction trees, which is a data structure that represents effects abstractly. Interaction trees are similar to traces because they both specify sequences of operations. Some related papers include:

"Interaction trees: representing recursive and impure programs in Coq"; the paper that discusses interaction trees in detail
"Verifying an HTTP Key-Value Server with Interaction Trees and VST"; the paper also presents a key-value store but based on interaction trees
"Choice Trees: Representing Nondeterministic, Recursive, and Impure Programs in Coq"
"Program Adverbs and Tlön Embeddings"; the paper discusses reasoning about effects using deep embeddings, i.e., abstractly.
Finally, it might also be worth to compare HATs with session types.

I think HATs are still a novel approach compared with all the works mentioned above, but the paper needs to be clear about the differences.


==> pldi2024/timeline.tex <==
\section{Change List}

\paragraph{Syntax, Algorithm, and Implementation}
\begin{enumerate}
    \item \textbf{(Hard)} Remove some type alias; add SFA-level predicates and SFA-level logic.
    \item \textbf{(Hard, but may not needed)} Ghost variable and corresponding typing algorithm, intersection type if necessary.
    \item \textbf{(Easy)} Parametric polymorphism.
    \item \textbf{(Easy - Hard, Depends on performance)} Alphabet Transformation Optimizations: Lori's paper, decision tree.
    \item \textbf{(Easy)} Simplify the put/get operational semantics (remove Get-Get).
\end{enumerate}

\paragraph{Evaluation}
\begin{enumerate}
    \item \textbf{(Easy)} Rephrases benchmarks in terms of representation invariants.
    \item \textbf{(Unknown)} One case study about the smart contract, which involves longer program but relatively simpler protocols.
\end{enumerate}

\paragraph{Presentation}
\begin{enumerate}
    \item \textbf{(Hard)} Rewrite the intro and motivation section in terms of representation invariants; provide mores examples, from easy to advance.
    \item \textbf{(Easy)} Emphasize that we can constraint the result value of events.
    \item \textbf{(Easy)} Explain the representation invariant verified in our benchmarks.
    \item \textbf{(Easy)} Scalability: emphasize the framing condition, which can help we omit the effects we don't care about; maybe justify this by our smart contract case study.
    \item \textbf{(Easy)} Related works (reviewer B).
    \item \textbf{(Easy)} Expressivity and Limitations, maybe emphasize that our alphabet transformation approach combine the refinement subtyping and the SFA inclusion, which makes our system more expressible. Clarify the relation/limitation with respect to OCaml features and typing.
\end{enumerate}

\paragraph{Typos}
\begin{enumerate}
    \item Fix $e\ v$.
    \item State that we assume typed recursive function always halt.
\end{enumerate}

\section{Timeline}

\begin{enumerate}
    \item \textbf{09/20 - 09/26} Refine syntax and add SFA-level predicates (also try to implement new features on the old benchmarks.). Find a case study, refine current benchmarks. These two are relevant, what specification we can/need to express. \emph{Others:} I need to prepare the slides for upenn talk.
    \item \textbf{09/27 - 10/03} Implement the new changes, add parametric polymorphism, run experiments. \emph{Others:} I will travel to UPenn (Thursday and Friday) and prepare the Midwest PL poster.
    \item \textbf{10/04 - 10/10} Finish the experiments, optimize the code if we need, try to finish the evaluation section. \emph{Others:} I will travel to UMich (Thursday and Friday).
    \item \textbf{10/11 - 11/16} It's better to take about one week to focus on the Incorrectness workshop and a month to rewrite the PLDI submission.
    \item Dues. PLDI submission deadline \textbf{11/16}; Incorrectness Workshop submission deadline \textbf{10/30}; POPL notification \textbf{10/02}; POPL artifact submission deadline \textbf{10/09}; POPL 2nd submission deadline \textbf{10/26}.
\end{enumerate}

==> sections/SFA.tex <==

\subsection{Symbolic Automata}\label{sec:SFA}
Unlike standard finite automata that work over a \emph{finite} domain
of input characters, symbolic finite automata (SFAs or, alternatively,
just symbolic automata) work over an \emph{infinite} set of
characters. This allows us to represent the potentially infinite set
of events that may appear in the trace of an effectful
computation. The symbolic \zget{} event {\small$\evop{get}{\Code{auth\_tab}\, \Code{id}}{\vnu>0}$}, for example,
captures the infinite set of successful authorization events {\small
  \{$\, \evapp{get}{auth\_tab\, id}{1}, \evapp{get}{auth\_tab\,id}{2},
  \ldots$ \}} that can occur during the execution of our motivating
example. A \emph{string} accepted by a SFA is a finite sequence of characters; and the \emph{language} of a SFA is a set of accepted strings.
% A \emph{string} is a finite sequence of characters; and a
% \emph{language} is a set of strings.
SFAs are finite state automata
(FAs) whose transitions carry \emph{predicates} instead of characters.
The domain of these predicates constitute the automata's
\emph{symbolic alphabet}. As with FAs, a string is accepted by SFA
{\small {\small$A$} } iff each character satisfies the corresponding
predicates carried by {\small$A$'s} transitions. The recognized
language of {\small$A$} is the set of all strings accepted by it,
denoted as {\small$\langA{A}$}.

As shown in \autoref{fig:type-syntax}, the symbolic alphabet of our
SFAs consists of a set of \emph{symbolic effect events}
{\small$\evop{\effop}{\overline{x}}{\phi}$} and a \emph{symbolic
  return event} {\small$\evopret{t }$}, per the definition of events
and traces in \autoref{fig:selected-semantics}.  A symbolic effect event
is similar to a refinement
type {\small$\rawnuot{b}{\phi}$}, and contains the name of an effect
operator {\small$\effop$}, argument variables {\small$\overline{x}$}
and the result variable {\small$\vnu$} that record the arguments and the result
value of applying {\small$\effop$} to {\small$\overline{x}$}, as well
as a qualifier {\small$\phi$} that constrains the assignment of
{\small$\overline{x}$} and {\small$\vnu$}.  A symbolic return event
{\small$\evret{t}$}, on the other hand, qualifies the result of a
trace (e.g., {\small$[\evappret{\lambda x{:}unit.1}]$}) and
thus has a pure refinement type {\small$t$}.  Symbolic automata
{\small$A$} are expressed as regular expressions over symbolic
alphabets and include standard constructions: the automaton that
accepts no trace ({\small$\emptyset$}), the automaton that only accepts the
empty trace ({\small$\epsilon$}), concatenation ({\small$AA$}), union ({\small$A \lorA A$}),
difference ({\small$A \setminus A$}), Kleene star ({\small$A^*$}), and wildcard
({\small$\anyA$}), which is defined as the union of all symbolic effect
events.

\begin{figure}[thp]
\begin{minipage}{.5\textwidth}
\centering
\begin{tikzpicture}[scale=0.115]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (28.1,-2.4) circle (2.2);
\draw [black] (7.9,-2.4) circle (2.2);
\draw [black] (48.5,-2.4) circle (2.2);
\draw [black] (48.5,-2.4) circle (1.6);
\draw [black] (48.5,-10.6) circle (2.2);
\draw [black] (48.5,-10.6) circle (1.6);
% \draw [black] (2.4,-2.4) circle (2.2);
\draw [black] (10.1,-2.4) -- (25.9,-2.4);
\fill [black] (25.9,-2.4) -- (25.1,-1.9) -- (25.1,-2.9);
\draw (18.0,-1.5) node [above] {\tiny$\evopa{put}{3}{k\, z}{z \leq 2 }$};
\draw [black] (30.3,-2.4) -- (46.3,-2.4);
\fill [black] (46.3,-2.4) -- (45.5,-1.9) -- (45.5,-2.9);
\draw (38.3,-1.5) node [above] {\tiny$\evopa{get}{2\,3}{}{\vnu > 0}$};
\draw [black] (30.14,-3.22) -- (46.46,-9.78);
\fill [black] (46.46,-9.78) -- (45.9,-9.02) -- (45.53,-9.95);
\draw (29.1,-7.6) node [below] {\tiny$\evop{put}{tab\,k\,z}{k \opmod{} 3 > z}$};
\draw [black] (3.6,-2.4) -- (5.7,-2.4);
\fill [black] (5.7,-2.4) -- (4.9,-1.9) -- (4.9,-2.9);
\end{tikzpicture}
\vspace*{-.1in}
\caption{Symbolic automaton {\small$A$} .}\label{fig:sfa-A}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\centering
\begin{tikzpicture}[scale=0.115]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (23,-2.4) circle (2.2);
\draw [black] (8.9,-2.4) circle (2.2);
\draw [black] (48.5,-2.4) circle (2.2);
\draw [black] (48.5,-2.4) circle (1.6);
% \draw [black] (2.4,-2.4) circle (2.2);
\draw [black] (11.1,-2.4) -- (20.8,-2.4);
\fill [black] (20.8,-2.4) -- (20,-1.9) -- (20,-2.9);
\draw (15.95,-0.7) node [above] {\tiny$\evoponly{get}$};
\draw [black] (25.2,-2.4) -- (46.3,-2.4);
\fill [black] (46.3,-2.4) -- (45.5,-1.9) -- (45.5,-2.9);
\draw (35.75,-0.7) node [above] {\tiny$\evopret{\Code{x{:}int}\sarr\nuot{int}{\vnu \,{>}\, x}}$};
\draw [black] (4.6,-2.4) -- (6.7,-2.4);
\fill [black] (6.7,-2.4) -- (5.9,-1.9) -- (5.9,-2.9);
\end{tikzpicture}
% \vspace*{-.1in}
\caption{Symbolic automaton {\small$B$}.}\label{fig:sfa-B}
\end{minipage}
\vspace*{-.1in}
\end{figure}

\begin{example}[Symbolic automata]
  Consider the symbolic automata {\small$A$} and {\small$B$} over
  effect operators \zput{} and \zget{} shown in \autoref{fig:sfa-A}
  and \autoref{fig:sfa-B}. {\small$A$} consists of four states where
  two are final (labeled with a double circle); the first event
  {\small$\evopa{put}{3}{k\, z}{z \leq 2 }$} whose desugared
  representation (\autoref{fig:type-syntax} lists our type aliases) is
  {\small$\evop{put}{tab\,k\,z}{tab = 3 \land z \leq 2 }$}, requires the
  first argument of \zput{} to be {\small$3$}, its third argument to be less
  than or equal to {\small$2$}, and imposes no constraint on the second
  argument.  {\small$A$} accepts the following two effect traces %
  {\small
    \begin{align*}
      &\alpha_1 \doteq [\evapp{put}{3\ \minus 19\
        1}{()};\ \evapp{get}{2\ 3}{17}] \quad
      &\alpha_2 \doteq
        [\evapp{put}{3\ \minus 6\ \minus 1}{()};\ \evapp{put}{\minus 99\
        8\, 0}{()}]
    \end{align*}}\noindent
  where the first trace {\small$\alpha_1$} halts on the upper final state
  in the figure since it ends with a \zget{} event that satisfies {\small$2 = 2 \land
    3 = 3 \land 17 > 0$}; the second trace {\small$\alpha_2$} halts on the
  lower final state, whose last event is a \zput{} event that satisfies
  {\small$8 \opmod{} 3 > 0$}. On the other hand, the automata
  {\small$B$} has a return event containing  a function
  type, and accepts the computation trace {\small$\beta_1$} but rejects
  {\small$\beta_2$}: %
  {\small
    \begin{align*}
      &\beta_1 \doteq
        [\evapp{get}{0\ 0}{0};\ \evappret{\text{$\lambda x.x+1$}}] \quad
      &\beta_2
        \doteq [\evapp{get}{0\ 0}{0};\ \evappret{\text{$\lambda x.2$}}]
    \end{align*}}\noindent
  {\small$B$} accepts the trace {\small$\beta_1$} because {\small$\beta_1$}'s first
  event is consistent with the symbolic event on the first transition of
  {\small$B$} (after
  desugaring {\small$\evop{get}{tab\,k\,z}{\top}$}); the last event in
  {\small$\beta_1$} returns a function {\small$\lambda x.x+1$}, which is
  an inhabitant of the pure refinement type
  {\small$\Code{x{:}int}\sarr\nuot{int}{\vnu > x}$}. On the other hand,
  because the return event of trace {\small$\beta_2$} holds a function
  {\small$\lambda x.2$} that may output a value less than its input (e.g.,
  {\small$x=3$}),  it will be rejected by  {\small$B$}.
\end{example}

==> sections/changes.tex <==
\newpage
\section{Summary of Revisions}

We have attached three files: (a) marple.pdf is the revised version of
the paper, (b) marple-diff.pdf highlights the text corresponding to
major changes in \textcolor{blue}{blue} (typo fixes and minor edits
are not highlighted), and (c) marple-sm.pdf contains our supplementary
material.

The major changes are:
\begin{enumerate}

\item We have expanded \autoref{sec:evaluation} to include:
  \begin{enumerate}
  \item A table (\autoref{tab:evaluation-prop}) that provides
    additional details about the properties we consider in our
    evaluation (lines $883$-$907$, Reviewers A, C, and D),

  \item Specific research questions that focus the reader's attention
    on specific insights gleaned from the experiments (lines
    $909$-$913$, Reviewers A and D), and

  \item A discussion of qualitative measures of complexity for the
    representation invariants used in our evaluation (lines
    $934$-$940$, Reviewer D).
  \end{enumerate}

\item We have fleshed out \autoref{sec:algo} with additional
  details about our algorithm, including:
  \begin{enumerate}
  \item Additional details of our SFA inclusion check procedure,
    (lines $723$-$724$, $728$-$730$, $759$-$762$, $774$-$775$,
    Reviewers B and D),

  \item Expanded discussion of our algorithm's treatment of ghost
    variables (lines $806$-$813$, $825$-$830$, Reviewer D), and

  \item Added emphasis on the conditions that ensure our
    algorithmic type system is efficiently decidable, as
    well as an accompanying decidability theorem,
    \autoref{theorem:algo-decidable}
    (lines $462$-$464$, $723$-$724$, $728$-$730$, $860$-$861$, Reviewer B).
  \end{enumerate}

\item We have expanded our discussion of future work in
  \autoref{sec:conclusion} to incorporate the reviewers' suggestions,
  including more general verification
  questions (lines $1070$-$1073$, Reviewer B),
  richer properties (lines $1075$-$1076$, Reviewer D), and reasoning
  about effects beyond state (lines $1076$-$1077$, Reviewer A).

\item We have revised the body of our paper to more consistently use
  the terms ``stateful'' and ``effectful''; our introduction and
  overview emphasize that we are focused on clients that interact with
  library with hidden state (lines $94-97$, Reviewer A), while our
  formal treatment adopts the phrase effectful to emphasize that our
  type system is not intrinsically limited to stateful programs (lines
  $341$-$342$).

\item Our related work section now cites the additional papers on the
  Djiktstra Monad, F*, and session types, and includes a comparison with verification
  approaches based on interaction trees (lines $997$-$1005$, Reviewer A).

\item We have added an informal description of our fundamental theorem
  (lines $688$-$689$, Reviewer D).

%\item We have clarified the sources of our benchmarks on lines
%  $884$-$885$ (Reviewer A).

\end{enumerate}


==> sections/new-typing.tex <==
\section{New Typing}

\begin{enumerate}
    \item Shall we add a real test event? or it is too complicate
    \item Typing and algorithm, recursive function problem.
\end{enumerate}

\begin{figure}[t!]
{\footnotesize
{\small\begin{flalign*}
 &\text{\textbf{Type Syntax}} &
\end{flalign*}}
\begin{alignat*}{2}
    \text{\textbf{Base Types}}& \quad & b  ::= \quad &  \Code{unit} ~|~ \Code{bool} ~|~ \Code{nat} ~|~ \Code{int} ~|~ \Code{char} ~|~ \Code{string} ~|~ b\, \Code{option}
    \\ \text{\textbf{Basic Types}}& \quad & s  ::= \quad & b ~|~ s \sarr s
    \\ \text{\textbf{Value Literals}}& \quad & l ::= \quad & c ~|~ x ~|~ \primop\ \overline{l}
    \\ \text{\textbf{Qualifiers}}& \quad & \phi ::= \quad & l ~|~ \bot ~|~ \top  ~|~ \neg \phi ~|~ \phi \land \phi ~|~ \phi \lor \phi ~|~ \phi \impl \phi ~|~ \forall x{:}b.\, \phi 
    \\ \text{\textbf{Refinement Types}}& \quad &t ::= \quad & \nuot{\textit{b}}{\phi} ~|~ x{:}t\sarr\tau  ~|~ x{:}b\garr t
    \\ \text{\textbf{Symbolic Automata}}& \quad &A,B  ::= \quad &  \evop{\effop{}}{\overline{x}}{\phi} ~|~ \evret{t} ~|~ \evparenth{\phi} ~|~ \botA ~|~ \topA ~|~ \negA A ~|~ A \landA A ~|~ A \lorA A ~|~ \empA ~|~ AA ~|~ A^*
    \\ \text{\textbf{Guarded Automata Types}}& \quad &\tau  ::= \quad & t ~|~ \rawgatLR{s}{\overline{A \effarr B\gatbar}}
    \\\text{\textbf{Type Contexts}}& \quad &\Gamma ::= \quad & \emptyset ~|~ x{:}t, \Gamma
  \end{alignat*}
{\small\begin{flalign*}
 &\text{\textbf{Automata Aliases}} &
\end{flalign*}}
\begin{alignat*}{3}
    \evop{\effop}{... {\sim}{x_i}{:}{v_i} ...}{\phi} &\doteq \evop{\effop}{... x_i ...}{x_i = v_i \land \phi}
    \quad& A \implA B &\doteq \negA A \lorA B
    \quad& A \iffA B &\doteq  A \implA B \landA B \implA A
    \\ \existsA A &\doteq \topA A \topA
    \quad& A \mustAfter B &\doteq \existsA (AB) \lorA \negA (\existsA B) 
    \quad& A \mustBefore B &\doteq \existsA (AB) \lorA \negA (\existsA A)
\end{alignat*}
{\small\begin{flalign*}
 &\text{\textbf{Type Aliases}} &
\end{flalign*}}
\begin{alignat*}{3}
    \rawgatLR{s}{ ... \gatbar A \increffarr B \gatbar ...  } &\doteq \rawgatLR{s}{... \gatbar A \effarr AB \gatbar ...  } 
    \quad& b &\doteq \rawnuot{b}{\top} 
    % \quad& t &\doteq \rawgat{\eraserf{t}}{\topA}{\topA  \evopret{t}}
\end{alignat*}
}
    \caption{\langname{} types.}\label{fig:type-syntax}
\end{figure}

\paragraph{Syntax} Similar with the FOL logic used in the value qualifiers, the language of trace qualifiers is an regular language that has logic connectives (negation, conjunction, and disjunction) as well as all primitives in SFAs (symbolic events, empty trace, concatenation, Kleene star). Moreover, to fit the dependency in the DATs, we also extend it will trace-level variable $X$ and inclusion test $\alpha \in A$.

\section{Example}

\paragraph{Built-in operator} The built-in operators:
{\footnotesize\begin{align*}
    \predA{KVStore}{saved}(\Code{tab,key,value}) &\doteq \topA \evop{put}{\df{x}{tab}\,\df{y}{key}\,\df{z}{value}}{\phi}(\negA \existsA \evop{put}{\df{x}{tab}\,\df{y}{key}\,z}{\top})
    \\\S{get} : &\gv{value}{\Code{int}} \Code{tab}{:}\Code{int} \sarr \Code{key}{:}\Code{int} \sarr 
    \\ \effL \Code{int\ option} ~|~ &\predA{KVStore}{saved}(\Code{tab}, \Code{key}, \Code{value}) \increffarr
    \evopret{\nuot{int}{\vnu = \Code{Some\ value}}} \gatbar
    \\&\negA \existsA \evop{put}{\df{x}{tab}\,\df{y}{key}\,z}{\top} \increffarr
    \evopret{\nuot{int}{\vnu = \Code{None}}} \effR
    \\\S{put} : &\Code{tab}{:}\Code{int} \sarr \Code{k}{:}\Code{int} \sarr \Code{data}{:}\Code{int} \sarr \incrgat{unit}{\topA}{\evopret{\Code{unit}}}
    % \\\S{member} : &\Code{tab}{:}\Code{int} \sarr \Code{k}{:}\Code{int} \sarr \effL \Code{bool} ~|~ P_{\Code{exists}} \increffarr\evopret{\nuot{bool}{\vnu = \Code{true}}} \gatbar \negA P_{\Code{exists}} \increffarr\evopret{\nuot{bool}{\vnu = \Code{false}}}
    % \effR
\end{align*}}

\paragraph{File system} File system, Consider following interface:
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=@@]{ocaml}
let add (path: string) (data: string): unit =
    match get (prefix path) with
    | Some DIR -> put path data
    | _ -> ()
\end{minted}

{\footnotesize\begin{align*}
    R_{\Code{FS}}(\Code{p}) \doteq & \evparenth{\Code{p}= \text{""}} \lorA (\evop{put}{\df{x}{{prefix}(\Code{p})}\,\df{y}{DIR}}{\top} \topA) \Lleftarrow (\evop{put}{\df{x}{p}\,y}{\top})
    \\\Code{add} :& \Code{p}{:}\Code{string} \garr \Code{path}{:}\nuot{string}{\vnu \not= \text{""}} \sarr \Code{data}{:}\Code{data} \sarr \gat{unit}{R_{\Code{FS}}(\Code{p})}{R_{\Code{FS}}(\Code{p})}
    % \\P_{\Code{stored}}(\Code{p}, \Code{data}) \doteq& \topA\evop{put}{\df{x}{p}\,\df{y}{data}}{\top}\topA
    % \\P_{\Code{stored}}(x\,y~|~\phi) \doteq& \topA\evop{put}{x\,y}{\phi}\topA
    \\\Code{case_1}:& R_{\Code{FS}}(\Code{p}) \landA (\existsA \evop{put}{\df{x}{{prefix}(\Code{path})}\,\df{y}{DIR}}{\top}) \increffarr
    \\&\evop{get}{\df{x}{prefix(path)}}{\vnu = \Code{Some\ DIR}}\evop{put}{\df{x}{path}\,\df{y}{data}}{\top}\evopret{\Code{unit}}
    \\\Code{case_2}:& R_{\Code{FS}}(\Code{p}) \landA \negA (\existsA \evop{put}{\df{x}{{prefix}(\Code{path})}\,\df{y}{DIR}}{\top}) \increffarr
    \\&\evop{get}{\df{x}{prefix(path)}}{\vnu \not= \Code{Some\ DIR}}\evopret{\Code{unit}}
    \\&\gatLR{unit}{\Code{case_1} \gatbar \Code{case_2}} <: \gat{unit}{R_{\Code{FS}}(\Code{p})}{R_{\Code{FS}}(\Code{p})}
\end{align*}}
\ZZ{Why not condition? (a) Condition always requires you to talk about both cases of an automata, however, all the thing out from $R_{\Code{FS}}$ is undefined; We can put the $\botA$ on the false branch, however, it is kind of complicate. (b) We have pattern matching that has arbitrary many cases, it is wired that can have conditional expression in type (c) To define a nested conditional expression in the type will change our type denotation a lot. }

\paragraph{MinSet}Represent the MinSet consists of a set plus mutable cell. Consider following interface:
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=@@]{ocaml}
let minset_insert (elem : int) : unit =
  if not (inited ()) then (
    write elem;
    insert elem)
  else if mem elem then ()
  else (
    insert elem;
    let (min : int) = read () in
    if min <= elem then () else write elem)
\end{minted}

{\footnotesize\begin{align*}
    \predA{WR}{stored}(\Code{elem}) &\doteq \topA \evop{write}{\df{x}{elem}}{\top} \negA \existsA \evop{write}{x}{\top}
    \\R_{\Code{minset}}(\Code{min}) \doteq&
    \predA{WR}{stored}(\Code{min}) \iff \existsA \evop{write}{\df{x}{min}}{\top} \landA \negA \existsA \evop{write}{x}{x < \Code{min}}
    \\\Code{minset\_insert}:& \gvn{min}{int} \Code{elem:int}\sarr \gat{unit}{R_{\Code{minset}}(\Code{min})}{R_{\Code{minset}}(\Code{min})}
    \\\Code{case_1}:& R_{\Code{minset}}(\Code{min}) \landA \negA \existsA \evop{write}{x}{\top}
    \\&\increffarr \evop{inited}{x}{\vnu = \Code{false}}\evop{write}{\df{x}{elem}}{\top}\evop{insert}{\df{x}{elem}}{\top}\evopret{\Code{unit}}
    \\\Code{case_2}:& R_{\Code{minset}}(\Code{min}) \landA \existsA \evop{write}{x}{\top} \landA \existsA \evop{insert}{\df{x}{elem}}{\top}
    \\&\increffarr \evop{inited}{x}{\vnu = \Code{true}}\evop{mem}{\df{x}{elem}}{\vnu = \Code{true}}\evopret{\Code{unit}}
    \\\Code{case_3}:& R_{\Code{minset}}(\Code{min}) \landA \existsA \evop{write}{x}{\top} \landA \negA \existsA \evop{insert}{\df{x}{elem}}{\top} \landA \existsA \evop{insert}{x}{x \leq \Code{elem}}
    \\&\increffarr \evop{inited}{x}{\vnu =\Code{true}}\evop{mem}{\df{x}{elem}}{\vnu = \Code{false}}
    \\&\quad\evop{insert}{\df{x}{elem}}{\top}\evop{read}{x}{\vnu \leq \Code{elem}}\evopret{\Code{unit}}
    \\\Code{case_4}:& R_{\Code{minset}}(\Code{min}) \landA \existsA \evop{write}{x}{\top} \landA \negA \existsA \evop{insert}{\df{x}{elem}}{\top} \landA \negA \existsA \evop{insert}{x}{x \leq \Code{elem}}
    \\&\increffarr \evop{inited}{x}{\vnu =\Code{true}}\evop{mem}{\df{x}{elem}}{\vnu = \Code{false}}
    \\&\quad\evop{insert}{\df{x}{elem}}{\top}\evop{read}{x}{\Code{elem} < \vnu}\evop{write}{\df{x}{elem}}{\top}
    \evopret{\Code{unit}}
\end{align*}}

\paragraph{LazySet} Here is the one of the most interesting case, consider that our \Code{Set} operation (e.g., insert) is time-comsuming, thus the \Code{LazySet} want to (1) avoid duplicate insert (2) delay the actually insert. Thus it will preserve the following invaraiant:
{\footnotesize\begin{align*}
    R_{\Code{LazySet}}(\Code{elem}) \doteq \negA \existsA (\evop{insert}{\df{x}{elem}}{\top}\topA \evop{insert}{\df{x}{elem}}{\top})
\end{align*}}\noindent
Then consider following two interfaces:
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=@@]{ocaml}
let lazy_insert (thunk: unit -> unit) (a: int): unit -> unit =
    fun () => thunk (); (if (mem a) then insert a else ())

let force_thunk (thunk: unit -> unit) : unit = thunk ()
\end{minted}
The type of $\Code{lazy\_insert}$ is interesting
{\footnotesize \begin{align*}
    \Code{lazy\_insert}:&\gvn{elem}{int}\normalv{thunk}{(\Code{unit}\sarr \gat{unit}{R_{\Code{LazySet}}(\Code{elem})}{R_{\Code{LazySet}}(\Code{elem})})} \normalv{a}{\Code{int}}
    \\&\Code{unit}\sarr \gat{unit}{R_{\Code{LazySet}}(\Code{elem})}{R_{\Code{LazySet}}(\Code{elem})}
\end{align*}}\noindent
where both input thunk and output thunk preserves the representation invariant. There are two branch's in the implementation:
{\footnotesize\begin{align*}
    \Code{case1}:& R_{\Code{LazySet}}(\Code{elem}) \landA \existsA (\topA \evop{insert}{\df{x}{elem}}{\top} \topA) \increffarr \evopret{\Code{unit}}
    \\\Code{case2}:& R_{\Code{LazySet}}(\Code{elem}) \landA \negA \existsA (\topA \evop{insert}{\df{x}{elem}}{\top} \topA) \increffarr \evop{insert}{\df{x}{elem}}{\top}\evopret{\Code{unit}}
    \\& \gat{unit}{\Code{case1}\gatbar\Code{case2}} <: \gat{unit}{R_{\Code{LazySet}}(\Code{elem})}{R_{\Code{LazySet}}(\Code{elem})}
\end{align*}}\noindent



\paragraph{BST} Represent the BSTs in the tree library.
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=@@]{ocaml}
type node = int

type effect =
  | NewNode of ('a -> node) (* unique node id *)
  | GetLabel of (node -> 'a)(* read a value from node; independent from tree *)
  | MemNode of (node -> bool) (* check membership *)
  | IsLeft of (node -> node -> bool) (* is left child *)
  | IsRight of (node -> node -> bool) (* is left child *)
  | GetLeft of (node -> node option) (* return left child *)
  | GetRight of (node -> node option) (* return right child *)
  | GetPrarent of (node -> node option) (* return parent *)
  | AddLeft of (node -> node -> unit) (* add left into tree *)
  | AddRight of (node -> node -> unit) (* add right into tree *)
  | RemoveLeft of (node -> unit) (* remove left child from tree *)
  | RemoveRight of (node -> unit) (* remove left child from tree *)
\end{minted}

Then the representation of BST is 
{\footnotesize \begin{align*}
    \predA{Tree}{node}(\Code{i}, \Code{v_i}) \doteq& \topA \evop{NewNode}{\df{x}{v_i}}{\vnu = \Code{i}} \negA (\existsA  \evop{RemoveNode}{\df{x}{i}}{\top})
    \\\predA{Tree}{left}(\Code{i},\Code{j}) \doteq&
    \topA \evop{addLeft}{\df{x}{i}\,\df{y}{j}}{\top} \negA (\topA \evop{removeLeft}{\df{x}{g}\,\df{y}{i}}{\top} \topA)
    \\\predA{Tree}{right}(\Code{i},\Code{j}) \doteq&
    \topA \evop{addRight}{\df{x}{i}\,\df{y}{j}}{\top} \negA (\topA \evop{removeRight}{\df{x}{g}\,\df{y}{i}}{\top} \topA)
    \\R_{\Code{BST}}(\Code{i}, \Code{v_i}, \Code{j}, \Code{v_j}) \doteq&
    \predA{Tree}{node}(\Code{i}, \Code{v_i}) \landA \predA{Tree}{node}(\Code{j}, \Code{v_j}) \Rrightarrow 
    (\predA{Tree}{left}(\Code{g},\Code{i},\Code{j}) \lorA \predA{Tree}{right}(\Code{g},\Code{j},\Code{i})) \implA \evparenth{ \Code{v_i} < \Code{v_j}}
    \\\Code{bst\_insert} :& \Code{i}{:}\Code{node} \garr \Code{v_i}{:}\Code{int} \garr
    \Code{j}{:}\Code{node} \garr \Code{v_j}{:}\Code{int} \garr
    \Code{root}{:}\Code{node} \sarr \Code{data}{:}\Code{int} \sarr \gat{unit}{R_{\Code{BST}(\Code{i, v_i, j,v_j})}}{R_{\Code{BST}(\Code{i, v_i, j,v_j})}}
\end{align*}}

\paragraph{DFA} Represent the DFA in the graph library -- the interfaces comes from the ``OCamlGraph'' library (marked mutable graph).
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=@@]{ocaml}
type node = int

type effect =
  | NewNode of (unit -> node) (* unique node id *)
  | RemoveNode of (node -> unit) (* unique node id *)
  | MemNode of (node -> bool) (* check membership *)
  | GetEdge of (node -> node -> 'b option) (* is connected *)
  | Connect of (node -> node -> 'b -> unit) (* connect *)
  | DisConnect of (node -> node -> unit) (* disconnect *)
\end{minted}

Then the representation of DFA is 
 {\footnotesize
    \begin{align*}
      \predA{Graph}{node}(\Code{s}) \doteq \
      &\topA \evop{newNode}{x}{\vnu = \Code{s}} \negA (\topA  \evop{removeNode}{\df{x}{s}}{\top}; \topA) \\
       \predA{Graph}{connected}(\Code{s_1, c, s_2}) \doteq \
      &\topA \evop{connect}{\df{x}{s_1}\,\df{y}{c}\,\df{z}{s_2}}{\top} \negA (\topA  \evop{disconnect}{\df{x}{s_1}\,\df{y}{c}\,\df{z}{s_2}}{\top}; \topA) 
      \\R_{\Code{DFA}}(\Code{s_1}, \Code{c}, \Code{s_2}, \Code{s_3}) \doteq \
      &(\predA{Tree}{node}(\Code{s_1}) \landA \predA{Tree}{node}(\Code{s_2})  \Lleftarrow \evop{connect}{\df{x}{s_1}\,\df{y}{s_1}\,\df{z}{c}}{\top})  \landA 
      \\&(\predA{Graph}{connected}(\Code{s_1, c, s_2}) \landA \predA{Graph}{connected}(\Code{s_1, c, s_3}) \implA \evparenth{\Code{s_2} = \Code{s_3}})
      \\\Code{add\_trans} :& \Code{s_1}{:}\Code{node} \garr \Code{c}{:}\Code{char} \garr
    \Code{s_2}{:}\Code{node} \garr \Code{s_3}{:}\Code{node} \garr
    \\&\Code{start}{:}\Code{node} \sarr \Code{ch}{:}\Code{char} \sarr \Code{end}{:}\Code{node} \sarr 
    \gat{unit}{R_{\Code{DFA}(\Code{s_1, c, s_2, s_3})}}{R_{\Code{DFA}(\Code{s_1, c, s_2, s_3})}}
    \end{align*}}\noindent

\subsection{Type Soundness}

\begin{figure}[t!]
\footnotesize{
{\small\begin{flalign*}
 &\text{\textbf{SFA Language}} & \fbox{$\langATr{A} \in \mathcal{P}(\alpha)$}
\end{flalign*}}
\begin{align*}
    \langATr{ \evop{\effop{}}{\overline{x_i} }{\phi} } &\doteq \{ \pevapp{\effop}{\overline{v_i}}{v} ~|~ \emptyset \basicvdash \effop : \overline{b_i}\sarr b \landA (\forall i.\emptyset \basicvdash v_i : b_i) \landA \emptyset \basicvdash v : b \landA \phi\overline{[x_i\mapsto v_i][\vnu \mapsto v]} \}
\end{align*}
\begin{alignat*}{2}
    \langATr{ \evret{ t }} &\doteq \{ \pevappret{v} ~|~ v \in \denotation{t} \}\quad&
    \langATr{\empA} &\doteq \{ \emptr \}
    \qquad \langATr{\topA} \doteq Tr
    \qquad \langATr{\botA} \doteq \emptyset
    \\ 
    \langATr{\negA A} &\doteq Tr \setminus \langATr{A}
    \quad& \langATr{A \lorA A' } &\doteq \langATr{A} \cup \langATr{A'}
    \qquad \langATr{A \landA A' } \doteq \langATr{A} \cap \langATr{A'}
    \\ \langATr{A^*} &\doteq \bigcup^{\infty}_{i = 0} \langA{\underbrace{\epsilon AA...A}_\text{repeat $A$ for $i$ times} }
    \quad& \langATr{A;A'} &\doteq \{ \alpha \listconcat \alpha' ~|~ \alpha \in \langATr{A}, \alpha' \in  \langATr{A'} \} 
    \\ \langATr{\evparenth{\phi}} &\doteq \begin{cases}
      Tr, & \text{if}\ \phi \iff \top\\
      \emptyset, & \text{otherwise}
    \end{cases}
\end{alignat*}
% {\small\begin{flalign*}
%  &\text{\textbf{Guarded SFA Language}} & \fbox{$\langATr{\alpha, G} \in \mathcal{P}(\alpha)$}
% \end{flalign*}}
% \begin{alignat*}{2}
%     \langATr{ \evret{ t }} &\doteq \{ \pevappret{v} ~|~ v \in \denotation{t} \}\quad&
%     \langATr{\empA} &\doteq \{ \emptr \}
%     \qquad \langATr{\topA} \doteq Tr
%     \qquad \langATr{\botA} \doteq \emptyset
% \end{alignat*}
{\small\begin{flalign*}
  &\text{\textbf{Type Denotation}}
  & \fbox{$\denotation{t} \in \mathcal{P}(e)
    \quad \denotation{\tau} \in \mathcal{P}(e)$}
\end{flalign*}}
\begin{align*}
    &\denotation{ \rawnuot{b}{\phi} } &&\doteq \{ e ~|~ \emptyset \basicvdash e : b \land \forall \alpha\ \alpha'\ v. \msteptr{\alpha}{e}{\alpha'}{v} \impl \alpha' = \emptr \land \phi[\nu\mapsto v] \}
    \\ &\denotation{ x{:}t_x\sarr{}\tau } &&\doteq \{ e ~|~ \emptyset \basicvdash e : \eraserf{x{:}t_x\sarr{}\tau} \land
    \forall v_x \in \denotation{ t_x }.\, e\ v_x \in  \denotation{ \tau[x\mapsto v_x ] } \}
    \\ &\denotation{ x{:}s_x\garr{}\tau } &&\doteq \{ e ~|~ \emptyset \basicvdash e : \eraserf{\tau} \land
    \forall v_x. \emptyset \basicvdash v_x : s_x \impl e \in  \denotation{ \tau[x\mapsto v_x ] } \}
    \\ &\denotation{ \overline{\rawgat{s}{A}{B} \gatbar} } &&\doteq \{e ~|~ \emptyset \basicvdash e : s \land \forall \alpha\ \alpha'\ v. \msteptr{\alpha}{e}{\alpha'}{v} \impl \bigwedge \alpha \in \langATr{A_i} \impl \alpha \listconcat \alpha' \listconcat \evret{v} \in \langATr{B_i} \}
\end{align*}
{\small\begin{flalign*}
  &\text{\textbf{Type Context Denotation}}
  & \fbox{$\denotation{\Gamma} \in \mathcal{P}(\sigma)$}
\end{flalign*}}
\begin{alignat*}{2}
    \denotation{ \emptyset } &\doteq \{ \emptyset \} \qquad\qquad\qquad\qquad&
    \denotation{ x{:}t, \Gamma } &\doteq \{ \sigma[x\mapsto v] ~|~ v\in \denotation{t}, \sigma \in \denotation{\Gamma[x\mapsto v]} \}
\end{alignat*}
}
    \caption{\langname{} refinement types denotation.}\label{fig:type-denotation}
\end{figure}

The denotation of a symbolic automaton {\small$\langA{A}$}, as shown in \autoref{fig:type-denotation}, is the set of traces
accepted by the automata (i.e., the recognized language in the
automata literature); the denotation of pure refinement types
{\small$\denotation{t}$} and HATs {\small$\denotation{\tau}$} are sets of terms; these functions are defined mutually-recursively. Analogy: {\small
\begin{alignat*}{3}
\text{STLC:}&& \quad \mstep{e}{v} &\impl e \in \denotation{\rawnuot{b}{\phi}} \quad &&\text{ where } \phi[\vnu \mapsto v] \text{ is valid} \\
\text{\langname:}&& \quad \msteptr{\alpha}{e}{\alpha'}{v} &\impl e \in \denotation{\rawgat{b}{A}{B\evopret{\rawnuot{b}{\phi}}}}  \quad &&\text{ where }
\alpha \in \langA{A}, \alpha \listconcat \alpha' \in \langA{B}, \phi[\vnu \mapsto v] \text{ is valid}
\end{alignat*}}\noindent

\begin{definition}[Well-formed built-in operator typing context]\label{lemma:built-in-typing}
  The built-in operator typing context {\small$\Delta$} is well-formed iff for
  any (pure or effectful) operator {\small$\theta$} that has basic type {\small$\overline{b_i}\sarr b$},
  the pure refinement type {\small {\small$t$}} where {\small$ (\theta, t) \in \Delta$} is
  of the form
  {\small$\overline{x{:}b}\garr \overline{y{:}t_y}\sarr\basegat{b}{\overline{A_k \increffarr \evopret{t_k}}}$}
  such that {\small
\begin{align*}
    &\forall \sigma \in \denotation{\Gamma}.\overline{\forall x{:}b}. \overline{\forall v_y \in \denotation{\sigma(t_y)}}. \forall \alpha\ v. \alpha \vDash \theta\ \overline{v_y} \Downarrow v \impl \bigwedge 
    \alpha \in \langA{\sigma(A_k\overline{[y \mapsto v_y]})} \impl v \in \denotation{\sigma(t_k\overline{[y \mapsto v_y]})}
\end{align*}}\noindent
Since both pure and effectful operators in \langname{} are atomic,
the postcondition automaton of the operator is always a pure
refinement type consistent with the primitive relation
{\small$\Downarrow$}.
Moreover, if {\small$\theta$} is pure, {\small$A$}  can always be {\small$\topA$} indicating that {\small$\theta$} can be applied in an arbitrary context.
\end{definition}

\begin{theorem}\label{theorem:fundamental}[Fundamental Theorem] If the built-in operator type context {\small$\Delta$} is well-formed, for all type contexts
  {\small$\Gamma$}, terms {\small$e$} and GAT {\small$\tau$},
  {\small$\Gamma \vdash e : \tau \implies \forall \sigma, \sigma \in \denotation{\Gamma} \impl \sigma(e) \in \denotation{\sigma(\tau)}$}.\footnote{A Coq mechanization of this theorem and the type soundness corollary are provided in the \techreport{}.}
\end{theorem}

\begin{corollary}\label{theorem:postautomata}[Type Soundness] If the built-in operator type context {\small$\Delta$} is well-formed, for all terms {\small$e$} and representation invariant $R(\overline{x})$\footnote{The type judgement is actually under a stronger assumption, where $x$ in the two sides of implication are the same.},
{\small\begin{align*}
&\emptyset \vdash e : \overline{x{:}b}\garr \rawgat{s}{R(\overline{x})}{R(\overline{x})\evopret{\Code{unit}}} \implies 
\\&\quad \forall \alpha\ \alpha'.\msteptr{\alpha}{e}{\alpha'}{()} \impl 
(\overline{\forall x{:}b}. \alpha \in \langATr{R(\overline{x})}) \impl (\overline{\forall x{:}b}. \alpha \listconcat \alpha'\in \langA{R(\overline{x})})
\end{align*}}
\end{corollary}


\begin{figure}[th]
{\footnotesize
{\normalsize
\begin{flalign*}
 &\text{\textbf{Type Synthesis }} &
 \fbox{$\Gamma \infervdash{A} e \typeinfer B$}&&
  &\text{\textbf{Type Check }} &
 \fbox{$\Gamma \checkvdash{A} e \typecheck B$}
\end{flalign*}
}
\\ \
\begin{prooftree}
\hypo{
\emptyset \basicvdash c : b
}
\infer1[\textsc{SynConst}]{
\Gamma \infervdash{A} c \typeinfer A\evopret{\rawnuot{b}{\vnu = c}}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{(x, \rawnuot{b}{\phi}) \in \Gamma}
\infer1[\textsc{SynBVar}]{
\Gamma \infervdash{A} x \typeinfer A\evopret{\rawnuot{b}{\vnu = x}}
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{(x, \overline{x{:}b}\garr y{:}t\sarr\tau) \in \Gamma}
\infer1[\textsc{SynFVar}]{
\Gamma \infervdash{A} x \typeinfer A\evopret{ \overline{x{:}b}\garr y{:}t\sarr\tau }
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{35mm}{\center
  $\Gamma \infervdash{A} e_x \typeinfer \lorA\overline{A_i\evopret{t_i}} $\quad 
  $\forall i. \Gamma, x{:}t_i \checkvdash{A_i} e \typecheck B$
}
}
\infer1[\textsc{ChkLet}]{
\Gamma \checkvdash{A} \zlet{x}{e_x}{e} \typecheck B
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{40mm}{\center
  $\Gamma \infervdash{A} e \typeinfer B'$\\ 
  $\Gamma \vdash ((A\topA) \landA B') \subseteq ((A\topA) \landA B)$
}
}
\infer1[\textsc{ChkSub}]{
\Gamma \checkvdash{A} e \typecheck B
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{70mm}{\center
  $\Gamma \infervdash{A} v_1 \typeinfer A_x\evopret{\overline{y{:}b_{y}} \garr z{:}t\sarr \fullnormalgat{s}{A_i}{B_{ij}}{t_{ij}}}$\\
  $\Gamma, y{:}b_{y} \checkvdash{A_x} v_2 \typecheck A_x\evopret{t}$ \\
  $\forall i. \Code{AbductiveInfer}(\overline{y{:}b_{y}}, A_x \landA A_i) = \overline{y{:}t_{y_i}}$\\
  $\forall i\ j. \Gamma, \overline{y{:}t_{y_i}}, x{:}t_{ij} \checkvdash{((A_x \landA A_i)\topA) \landA B_{ij}} e \typecheck B$
}
}x
\infer1[\textsc{ChkApp}]{
  \Gamma \checkvdash{A} \zlet{x}{v_1\ v_2}{e} \typecheck B
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{60mm}{\center
  $(\effop, \overline{y{:}b_{y}} \garr \overline{z_i{:}t_i}\sarr \fullnormalgat{s}{A_j}{B_{jk}}{t_{jk}}) \in \Delta$\\
  $\forall i. \Gamma, \overline{y{:}t_{y}} \checkvdash{A} v_i \typecheck A\evopret{t_i}$\\
  $\forall i. \Code{AbductiveInfer}(\overline{y{:}b_{y}}, A \landA A_j) = \overline{y{:}t_{y_j}}$\\
  $\forall j\ k. \Gamma, \overline{y{:}t_{y_j}}, x{:}t_{jk} \checkvdash{((A \landA A_j)\topA) \landA B_{jk}} e \typecheck B$
}
}x
\infer1[\textsc{ChkEffOp}]{
  \Gamma \checkvdash{A} \zlet{x}{v_1\ v_2}{e} \typecheck B
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{58mm}{\center
  $(\primop, \overline{z_i{:}t_i}\sarr t_x) \in \Delta$\\
  $\forall i. \Gamma \infervdash{A} v_i \typecheck A\evopret{t_i}$ \\
  $\Gamma, x{:}(t_x\overline{[z_i \mapsto v_i]}) \checkvdash{A} e \typecheck B$
}}
\infer1[\textsc{ChkPureOp}]{
\Gamma \checkvdash{A} \perform{x}{\primop}{\overline{v_i}}{e} \typecheck B
}
\end{prooftree}
% \quad
% \begin{prooftree}
% \hypo{
% \parbox{30mm}{\center
%   $B = \evopret{x{:}t_x \garr t}$\\
%   $\Gamma, x{:}t_x \checkvdash{A} e \typecheck B$
% }
% }
% \infer1[\textsc{ChkGhost}]{
% \Gamma \checkvdash{A} e \typecheck B
% }
% \end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{60mm}{\center
  $B = \evopret{\overline{y{:}b}\garr x{:}t_x \sarr \rawdat{A_x}{s}{B_x}}$ \quad
  $\Gamma, \overline{y{:}b} \vdash t_x <: t$ \\ 
  $\Gamma, \overline{y{:}b}, x{:}t_x \checkvdash{A_x} e \typecheck B_x$
}
}
\infer1[\textsc{ChkFunc}]{
\Gamma \checkvdash{A} \zlam{x}{t}{e} \typecheck B
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{45mm}{\center
  $B = \evopret{t_f'}$ \quad
  $\Gamma \vdash t_f' <: t_f$ \quad 
  $\Gamma, f{:}t_f' \checkvdash{A} \zlam{x}{t_x}{e} \typecheck B$
}
}
\infer1[\textsc{ChkFix}]{
\Gamma \checkvdash{A} \zfix{f}{\text{$t_f$}}{x}{\text{$t_x$}}{e} \typecheck B
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{80mm}{\center
  $\forall i. (d_i, \overline{{y_{j}}{:}t_{j}}\sarr\rawnuot{b}{\phi_i}) \in \Delta$ \\
  $\Gamma, \overline{{y_{j}}{:}t_{j}}, z{:}\rawnuot{b}{\vnu = v \land \phi_i} \checkvdash{A} e_i \typecheck B$ \quad \text{ where $z$ is fresh}
}
}
\infer1[\textsc{ChkMatch}]{
\Gamma \checkvdash{A} \match{v} \overline{d_i\, \overline{y_{j}} \to e_i} \typecheck B
}
\end{prooftree}
}
\caption{Bidirectional Typing Rules}\label{fig:full-bi-type-rules}
\end{figure}

\section{Declarative Typing Rules}

\begin{figure}[!ht]
{\small
{\normalsize
\begin{flalign*}
 &\text{\textbf{Well-Formed Types }} & % \fbox{$\Gamma \vdashover \tau$} \text{ and }
 \fbox{$\Gamma \wellfoundedvdash t  \quad \Gamma \wellfoundedvdash A \quad \Gamma \wellfoundedvdash \tau$}
\end{flalign*}}
 \\ \
\begin{prooftree}
\hypo{
\eraserf{\Gamma}, \vnu{:}b \basicvdash \phi : \Code{bool}
}
\infer1[\textsc{WfBase}]{
\Gamma \wellfoundedvdash \rawnuot{b}{\phi}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash t_x
}
\hypo{
\Gamma, x{:}t_x \wellfoundedvdash t
}
\infer2[\textsc{WfArr}]{
\Gamma \wellfoundedvdash x{:}t_x \sarr t
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash t_x
}
\hypo{
\Gamma, x{:}t_x \wellfoundedvdash t
}
\infer2[\textsc{WfGArr}]{
\Gamma \wellfoundedvdash x{:}t_x \garr t
}
\end{prooftree}
 \\ \ \\ \ \\
\begin{prooftree}
\hypo{
\S{Ty}(\effop) = \overline{x_i{:}b_i}\sarr b \quad  \eraserf{\Gamma}, \overline{x_i{:}b_i}, \vnu{:}b \basicvdash \phi : \Code{bool}
}
\infer1[\textsc{WfOpEvent}]{
\Gamma \wellfoundedvdash \evop{\effop{}}{\overline{x_i}}{\phi}
}
\end{prooftree}
 \\ \ \\ \ \\
\begin{prooftree}
\hypo{}
\infer1[\textsc{WfBotA}]{
\Gamma \wellfoundedvdash \botA
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{}
\infer1[\textsc{WfTopA}]{
\Gamma \wellfoundedvdash \topA
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{}
\infer1[\textsc{WfEpsilon}]{
\Gamma \wellfoundedvdash \epsilon
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash A_1 \quad \Gamma \wellfoundedvdash A_2
}
\infer1[\textsc{WfConcat}]{
\Gamma \wellfoundedvdash A_1A_2
}
\end{prooftree}
 \\ \ \\ \ \\
 \begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash A_1 \quad \Gamma \wellfoundedvdash A_2
}
\infer1[\textsc{WfOrA}]{
\Gamma \wellfoundedvdash A_1 \lorA A_2
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash A_1 \quad \Gamma \wellfoundedvdash A_2
}
\infer1[\textsc{WfAndA}]{
\Gamma \wellfoundedvdash A_1 \landA A_2
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\Gamma \wellfoundedvdash A
}
\infer1[\textsc{WfStar}]{
\Gamma \wellfoundedvdash A^*
}
\end{prooftree}
\ \\ \ \\ \ \\
\begin{prooftree}
\hypo{
\parbox{100mm}{\center
  $\forall i\ j. \Gamma \wellfoundedvdash A_i \land
  \Gamma \wellfoundedvdash B_{ij} \land \Gamma \wellfoundedvdash t_{ij} \land \eraserf{t_{ij}} = s$ \\ $\overline{A_i}$ and $\overline{B_{ij}}$ cannot be empty set
}}
\infer1[\textsc{WfGAT}]{
\Gamma \wellfoundedvdash \basegat{s}{\overline{A_i \effarr (\lorA \overline{B_{ij}\evopret{t_{ij}}})}}
}
\end{prooftree}
 \\ \
{\normalsize
\begin{flalign*}
 &\text{\textbf{Subtyping }} & \fbox{$\Gamma \vdash \tau <: \tau$}&&
  &\text{\textbf{Automata Inclusion }} &
 \fbox{$\Gamma \vdash A \subseteq A$}
\end{flalign*}
}
\\ \
\begin{prooftree}
\hypo{
\parbox{55mm}{\raggedright
$\forall \sigma \in \denotation{\Gamma}, \denotation{\sigma(\rawnuot{b}{\phi_1})} \subseteq \denotation{\sigma(\rawnuot{b}{\phi_2})}$
}}
\infer1[\textsc{SubBase}]{
\Gamma \vdash \rawnuot{b}{\phi_1} <: \rawnuot{b}{\phi_2}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{47mm}{\raggedright
$\Gamma \vdash \tau_{21} <: \tau_{11}$ \quad
$\Gamma, x{:}\tau_{21} \vdash \tau_{12} <: \tau_{22}$
}
}
\infer1[\textsc{SubArr}]{
\Gamma \vdash x{:}\tau_{11}\sarr{}\tau_{12} <: x{:}\tau_{21}\sarr{}\tau_{22}
}
\end{prooftree}
 \\ \ \\ \ \\
 \begin{prooftree}
\hypo{
\forall \sigma \in \denotation{\Gamma}, \langATr{\sigma(A)} \subseteq \langATr{\sigma(A')}
}
\infer1[\textsc{SubA}]{
\Gamma \vdash A \subseteq A'
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\forall i\ j. \Gamma \vdash ((A_i \land A_j')\topA) \landA B_i \subseteq ((A_i \land A_j')\topA) \landA B_j'
}
\infer1[\textsc{SubGAT}]{
\Gamma \vdash \basegat{s}{ \overline{A_i \effarr B_i} } <: \basegat{s}{ \overline{A_j' \effarr B_j'} }
}
\end{prooftree}
 \\ \ \\ \ \\
\begin{prooftree}
\hypo{
\Gamma, x{:}b \vdash \tau_{1} <: \tau_{22}
}
\infer1[\textsc{SubGArr1}]{
\Gamma \vdash \tau_1 <: x{:}b \garr\tau_{22}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\exists t. \Gamma \not\vdash t <: \rawnuot{b}{\bot} \land \Gamma, x{:}t \vdash \tau <: \tau'
}
\infer1[\textsc{SubGArr2}]{
\Gamma \vdash x{:}b \garr\tau <: \tau'
}
\end{prooftree}
}
\caption{Full auxiliary typing rules.}\label{fig:aux-rules-full}
\end{figure}

\begin{figure}[!ht]
{\footnotesize
{\normalsize
\begin{flalign*}
 &\text{\textbf{Typing}} & \fbox{$\Gamma \vdash \effop : \tau \quad \Gamma \vdash \primop : \tau \quad \Gamma \vdash e : \tau$}
\end{flalign*}
}
\\ \
\begin{prooftree}
\hypo{(x, \rawnuot{b}{\phi}) \in \Gamma}
\infer1[\textsc{\footnotesize TBaseVar}]{
\Gamma \vdash x : \rawnuot{b}{\vnu = x}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{(x, z{:}t\sarr\tau) \in \Gamma}
\infer1[\textsc{\footnotesize TFuncVar}]{
\Gamma \vdash x : z{:}t\sarr\tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{\emptyset \basicvdash c : b}
\infer1[\textsc{\footnotesize TConst}]{
\Gamma \vdash c : \rawnuot{b}{\vnu = c}
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{\Gamma, x{:}t_x \vdash e :  \tau}
\infer1[\textsc{\footnotesize TGhost}]{
\Gamma \vdash e : x{:}t_x\garr \tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{\Gamma, x{:}t_x \vdash e :  \tau}
\infer1[\textsc{\footnotesize TFun}]{
\Gamma \vdash \zlam{x}{t_x}{e} : x{:}t_x\sarr \tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{\Gamma, f{:}\tau \vdash \zlam{x}{\text{$s$}}{e} : \tau }
\infer1[\textsc{\footnotesize TFix}]{
\Gamma \vdash \zfix{f}{\text{$s$}}{x}{\text{$s$}}{e} : \tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{15mm}{\center
$\Gamma \vdash \tau_1 <: \tau_2$\quad
$\Gamma \vdash e : \tau_1$
}}
\infer1[\textsc{\footnotesize TSub}]{
\Gamma \vdash e : \tau_2
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\forall i. \Gamma \vdash e : \rawgat{s}{A_i}{B_i}
}
\infer1[\textsc{\footnotesize TSplit}]{
\Gamma \vdash e : \basegat{s}{\overline{A_i \effarr B_i}}
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{15mm}{\center
$(\primop, \tau) \in \Delta$
}}
\infer1[\textsc{\footnotesize TBuiltIn1}]{
\Gamma \vdash \primop : \tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{15mm}{\center
$(\effop, \tau) \in \Delta$
}}
\infer1[\textsc{\footnotesize TBuiltIn2}]{
\Gamma \vdash \effop : \tau
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{48mm}{\center
$\Gamma \vdash \primop : \overline{z_i{:}t_i}\sarr t$ \quad 
$\forall i. \Gamma, \overline{y{:}t_y} \vdash v_i : t_i$\\
$t\overline{[z_i \mapsto v_i]} = t_x$ \\
$\Gamma, x{:}t_x \vdash{} e : \tau$
}}
\infer1[\textsc{\footnotesize TPureOp}]{
\Gamma \vdash{} \zlet{x}{\primop\ \overline{v_i}}{e} : \tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{
\parbox{55mm}{\center
$\Gamma \vdash \effop : \overline{z_i{:}t_i}\sarr \tau$ \quad 
$\forall i. \Gamma, \overline{y{:}t_y} \vdash v_i : t_i$ \\
$\tau\overline{[z_i \mapsto v_i]} = \rawgat{b}{A}{A_x\evopret{t_x}}$ \\
$\Gamma, x{:}t_x \vdash{} e : \rawgat{s}{A_x\evop{\effop}{\rawdf{x_i}{v_i}}{\vnu = x}}{B}$
}}
\infer1[\textsc{\footnotesize TEffOp}]{
\Gamma \vdash{} \perform{x}{\effop{}}{\overline{v_i}}{e} : \rawgat{s}{A}{B}
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{58mm}{\center
$\Gamma \vdash v_1 : z{:}t \sarr \tau_x$\quad
$\Gamma \vdash v_2 : t$\\
$\tau_x[z\mapsto v_2] = \rawgat{s_x}{A}{\bigvee \overline{A_i\evopret{t_i}}}$\\
$\forall i. \Gamma, x{:}t_i \vdash e :  \rawgat{s}{A_i}{B_i}$
}}
\infer1[\textsc{\footnotesize TApp}]{
\Gamma \vdash \zlet{x}{v_1\ v_2}{e} :  \rawgat{b}{A}{\bigvee \overline{B_i}}
}
\end{prooftree}
% \\ \ \\ \ \\ \
\quad
\begin{prooftree}
\hypo{
\parbox{40mm}{\center
$\Gamma \vdash e_x : \rawgat{s}{A}{\bigvee \overline{A_i\evopret{t_i}}}$ \\
$\forall i. \Gamma, x{:}t_i \vdash e : \rawgat{s}{A_i}{B_i}$
}}
\infer1[\textsc{\footnotesize TLetE}]{
\Gamma \vdash \zlet{x}{e_x}{e} : \rawgat{s}{A}{\bigvee \overline{B_i}}
}
\end{prooftree}
\\ \ \\ \ \\ \
\begin{prooftree}
\hypo{
\parbox{45mm}{\center
% $\Gamma \vdash v : \rawnuot{b}{\phi}$\quad
$\forall i. (d_i, \overline{{y_{j}}{:}t_{j}}\sarr\rawnuot{b}{\phi_i}) \in \Delta$ \\
$\Gamma, \overline{{y_{j}}{:}t_{j}}, z{:}\rawnuot{b}{\vnu = v \land \phi_i} \vdash e_i : \tau$ \quad \text{ where $z$ is fresh}
% $\Gamma \wellfoundedvdash \tau$\quad
% $\Gamma, \overline{{y}{:}\tau_y} \vdash d_i\, \overline{{y}} : \tau_v$\quad
% $\Gamma, \overline{{y_{j}}{:}\tau_{j}} \vdash e_i : \tau$
}}
\infer1[\textsc{\footnotesize TMatch}]{
\Gamma \vdash (\match{v} \overline{d_i\, \overline{y_{j}} \to e_i}) :
\tau }
\end{prooftree}
}
\caption{Type rules.}\label{fig:full-typing-rules}
\end{figure}

==> tech/outlines.tex <==
\section{Outlines of Supplemental Materials}

The supplemental material is organized as follows. The full set  of rules for our operational semantics, basic typing, and declarative typing judgements are provided in \autoref{sec:tech:semantics}, \autoref{sec:tech:basic-typing}, and \autoref{sec:tech:typing}. The syntax and denotation of symbolic regular languages (SRL) that is used in our typing algorithm and implementation is presented in \autoref{sec:tech:srl}. The details of our typing algorithm is provided in \autoref{sec:tech:algo}. The Coq formalization and proof of theorems in our paper are presented in \autoref{sec:tech:proof}. ~\autoref{sec:tech:evaluation} provides a full table of our experimental results, as well as the source code of our tools and our benchmarks.

==> tech/srl.tex <==
\newpage
\section{Symbolic Regular Language}\label{sec:tech:srl}

\begin{figure}[t!]
{\footnotesize
{\small
\begin{alignat*}{2}
    \text{\textbf{Symbolic Regular Language}}& \quad &A,B  ::= \quad & \evop{\effop{}}{\overline{x}}{\phi} ~|~ \evparenth{\phi} ~|~ \anyA ~|~ \emptyset ~|~ \epsilon ~|~ A \landA A ~|~ A \lorA A ~|~ A ; A ~|~ A \setminus A ~|~ A^*
  \end{alignat*}}}
\caption{Symbolic Regular Language.}
\label{fig:srl}
\end{figure}

\begin{figure}[t!]
{\footnotesize
{\small\begin{flalign*}
 &\text{\textbf{SRL Language}} & \fbox{$\langA{A} \in \mathcal{P}(\alpha)$}
\end{flalign*}}
\begin{flalign*}
    \langA{ \evop{\effop{}}{\overline{x_i} }{\phi} } &\doteq \{ [\pevapp{\effop}{\overline{v_i}}{v}]  \in \mathit{Tr}^\textbf{WF} ~|~ \phi\overline{[x_i\mapsto v_i][\vnu \mapsto v]} \}
     \quad&
    \langA{ \evparenth{\phi} } &\doteq \{ [\pevapp{\effop}{\overline{v_i}}{v}]  \in \mathit{Tr}^\textbf{WF} ~|~ \phi \}\\
    \langA{\emptyset} &\doteq \emptyset
    \quad&
    \langA{\empA} &\doteq \{ \emptr \}\\
    \langA{A; A'} &\doteq \{ \alpha \listconcat \alpha' ~|~ \alpha \in \langA{A}, \alpha' \in  \langA{A'} \}
    \quad&
    \langA{\anyA} &\doteq \{ \alpha \in \mathit{Tr}^\textbf{WF} ~|~ \I{len}(\alpha) = 1 \}\\ 
    \langA{A \lorA A' } &\doteq \langA{A} \cup \langA{A'}
    \quad&
    \langA{A \land A' } &\doteq \langA{A} \cap \langA{A'}\\
    \langA{A^*} &\doteq \bigcup^{\infty}_{i = 0} \langA{\underbrace{\epsilon AA...A}_\text{repeat $A$ for $i$ times} }
     \quad& 
     \langA{A \setminus A'} &\doteq \langA{A} \setminus \langA{A'}
\end{flalign*}}
\caption{Symbolic Regular Language.}
\label{fig:srl-denoration}
\end{figure}

We post the syntax of Symbolic Regular Languages (SRL) and corresponding denotation in \autoref{fig:srl} and  \autoref{fig:srl-denoration}, which is strictly more expressive than LTL$_f$. Our desugaring procedure converts all SFAs encoded in LTL$_f$ formulae into SRL terms by adapting the standard  LTL$_f$ translation algorithm \cite{LTLf}.

==> tech/thoerom.tex <==
\begin{theorem}\label{theorem:preservation}[Preservation] If the built-in operator type context $\Delta$ is well-formed, for terms $e$ and Hoare automata types $\efftp{A}{\beta B}{s}$,
\begin{align*}
    \emptyset \vdash e : \efftp{A}{\beta B}{s} \land (\forall \alpha \in \langA{A} . \steptr{\alpha}{e}{\beta}{e'}) \impl \emptyset \vdash e' : \efftp{A\beta}{B}{s}
\end{align*}
\end{theorem}

\begin{theorem}\label{theorem:progress}[Progress] If the built-in operator type context $\Delta$ is well-formed, for a non-value computation $e$, 
\begin{align*}
    \emptyset \vdash e : \efftp{A}{B}{s} \impl \forall \alpha \in \langA{A} \exists \beta\ e'.\steptr{\alpha}{e}{\beta}{e'}
\end{align*}
\end{theorem}

Notice that the basic typing doesn't guarantee the progress, because even $\Code{Read}\,()$ is well typed in the basic type system, it still may get stuck when the context trace is an empty trace.


==> tech/type-syntax.tex <==
\begin{figure}[t!]
{\footnotesize
{\small\begin{flalign*}
 &\text{\textbf{Type Syntax}} &
\end{flalign*}}
\vspace{-1.8em}
{\small
\begin{alignat*}{2}
    \text{\textbf{Symbolic Regular Language}}& \quad &A,B  ::= \quad & \evop{\effop{}}{\overline{x}}{\phi} ~|~ \evparenth{\phi} ~|~ \anyA ~|~ \emptyset ~|~ \epsilon ~|~ A \landA A ~|~ A \lorA A ~|~ A ; A ~|~ A \setminus A ~|~ A^*
  \end{alignat*}}
\caption{Symbolic Regular Language.}
\label{fig:srl}}
\end{figure}

We post the syntax of Symbolic Regular Language (SRL) as above, which is similar with the symbolic LTL$_f$.
